Towards Corruption-Agnostic Robust Domain Adaptation

Big progress has been achieved in domain adaptation in decades. Existing works are always based on an ideal assumption that testing target domain are i.i.d. with training target domains. However, due to unpredictable corruptions (e.g., noise and blur) in real data like web images, domain adaptation methods are increasingly required to be corruption robust on target domains. In this paper, we investigate a new task, Corruption-agnostic Robust Domain Adaptation (CRDA): to be accurate on original data and robust against unavailable-for-training corruptions on target domains. This task is non-trivial due to large domain discrepancy and unsupervised target domains. We observe that simple combinations of popular methods of domain adaptation and corruption robustness have sub-optimal CRDA results. We propose a new approach based on two technical insights into CRDA: 1) an easy-to-plug module called Domain Discrepancy Generator (DDG) that generates samples that enlarge domain discrepancy to mimic unpredictable corruptions; 2) a simple but effective teacher-student scheme with contrastive loss to enhance the constraints on target domains. Experiments verify that DDG keeps or even improves performance on original data and achieves better corruption robustness that baselines.

==> CRDA (TOMM)/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> CRDA (TOMM)/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle


==> CRDA (TOMM)/latex/Supplementary_Section/DetailsOfCorruptions.tex <==
\section{Details of corruptions}
\label{sec:sup_DetailsOfCorruptions}

We follow the same types of corruptions as Hendrycks~\etal~\cite{hendrycks2019benchmarking} proposed to investigate how neural networks are robust against to common corruptions and perturbations.
The $15$ types of corruptions are: Gaussian Noise, Shot Noise, Impluse Noise, Defocus Blur, Motion Blur, Zoom Blur, Fog, Frost, Snow, Elastic Transform, Contrast, Brightness, JPEG Compression, Pixelate, and Glass Blur.
Fig.~\ref{fig:15corruption} illustrates examples of all the $15$ kinds of corruptions. For each kind, there are $5$ levels of severity as shown in Fig.~\ref{fig:6severity}.

% \input{latex/Supplementary_Section/imgs/15corruptions}

% \input{latex/Supplementary_Section/imgs/6severity}

==> CRDA (TOMM)/latex/Supplementary_Section/Full_TSCL_results.tex <==
\section{Full results for trade-off in TSCL}
\label{sec:full_TSCL_result}
\input{latex/Supplementary_Section/tabs/err_TSCL}
Table~\ref{tab:err_TSCL_full} reports the full results (mCE) of methods on each type of visual corruption.

==> CRDA (TOMM)/latex/Supplementary_Section/Further_Explanation.tex <==
\section{Further Explanation}
\label{sec:further_explanation}
% corruption robustness一直都很重要
% 以往研究不care这件事情是因为它在有监督的情境下已经解决的很好了
% 在DA中的corruption远远没有达到upper bound，还有非常大的工作空间
\input{latex/Supplementary_Section/imgs/mCE_precise-sup}

In this section, we emphasize the challenge and importance of CRDA through the lower bound. 

Corruption robustness is always an important subject. Previous works do not pay much care for corruptions because it has been addressed enough well in the setting of supervised learning. However, \textbf{corruption robustness in domain adaptation is far from satisfactory}.
% Corruption robustness has been tackled enough well in the setting of supervised learning, which is the reason why more attention are paid on challenging adversarial robustness rather than corruption robustness. However, corruption robustness in domain adaptation is far from satisfactory. 

As shown in Fig.~\ref{fig:mCE-precise-sup}, to estimate the status of current study, we further set an empirical lower bound for CRDA calculated by mCE of TSCL applied on CDAN+TN, which assumes testing corruptions are available while training. Models that reach the lower bound can be robust against unseen corruptions as if they are already known beforehand.

It is shown that current methods for CRDA still hold a large distance to the lower bound. In a word, instead of enough good progress in supervised learning, \textbf{there is still a long way to go for CRDA.}


==> CRDA (TOMM)/latex/Supplementary_Section/More_Ablation.tex <==
\section{More ablation on $\delta$, $\eta$, and $n$}
\label{sec:more_ablation}
\input{latex/Supplementary_Section/tabs/tab-ablation}
Table \ref{tab:Ablation-delta2} reports the mCE on different settings of hyper-parameter of DDG in Algorithm 2. Besides the conclusion of $\eta$ in the main text, it is shown that the final corruption robustness improves as the increase of shift range $\delta$ and decrease of the update step $n$. For stability, we set $\delta=60/255$, $\eta>2\delta$ and $n=2$ in this paper.

==> CRDA (TOMM)/latex/Supplementary_Section/Other_Details.tex <==
\section{Other details}
\label{sec:other_details}
% \paragraph{Clean error rate in Table 3 of Section 5.2.}
% The error rate of clean data in Table 3 is computed by the average of TSCL on total 15 corruptions (TSCL is trained for a specific corruption).

\paragraph{Training details of Fig.5 of Section 5.3 in the main manuscript}
All models are trained on a single domain (Real World of Office-Home).
Given Gaussian Noise corruption set with five levels of severity $T=\{t_{i}\}_{1}^{5}$ ($t_{0}$ denotes clean images) and inputs $x$, the training details of the models are as follows.
\begin{itemize}
    \item \textbf{Clean:} Supervised training on clean data.
    \item \textbf{All levels:} At the begining of each iteration, we randomly select a corruption from $\{t_{i}\}_{0}^{5}$ to corrupt the inputs $x$. All corrupted inputs $t(x)$ are aligned with the original clean inputs $x$ in feature space by contrastive loss.
    \item \textbf{Clean + Level 5:}  At the begining of each iteration, we randomly select a corruption from $\{t_{0},t_{5}\}$ to corrupt the inputs $x$. All corrupted inputs $t(x)$ are aligned with the original clean inputs $x$ in feature space by contrastive loss.
    \item \textbf{Level 5:} At the beginning of each iteration, we use level 5 corruption $t_{5}$ to corrupt the inputs $x$.
\end{itemize}


==> CRDA (TOMM)/latex/Supplementary_Section/Proof_Assumptions.tex <==
\section{Proof for three assumptions in Section 4.1 of the main manuscript}
\label{sec:sup_ProofFor3Assumptions}

% \begin{assumption}
% \label{assum:assum1}
% The corrupted versions are within the $\delta$-range neighborhood of the original clean image in sample space ($\boldsymbol{\delta}$ \textbf{cycle} for precise) and distance in sample space $d_{s}(t(x),x)$ becomes larger with increase of the severity level of corruption $T$.
% \end{assumption}
% \begin{assumption}
% \label{assum:assum2}
% Within the $\delta$ cycle, the severity level $t$ of a corruption  $T$ is positively correlated to distance in feature space  $d_{f}(f(t(x)) ,f(x))$.
% \end{assumption}
% \begin{assumption}
% \label{assum:assum3}
% Within the $\delta$ cycle, the severity level $t$ of a corruption $T$ is positively correlated to the value of transfer loss $\ell_{trans}(t(x))$.
% \end{assumption}

%--------------------------------------------------------------------------
\subsection{Proof for Assumption 1}
We give the empirical proof for Assumption 1 via Average Shift. Given a clean image $x\in \mathbb{R}^{c \times w \times h}$ and a corruption $t$, the Average Shift is calculated by:
\begin{equation}
    \begin{split}
    avg&=\frac{\|x-t(x)\|_{1}}{cwh} \\
    &=\frac{1}{cwh}\sum_{i=1}^{c} \sum_{j=1}^{w} \sum_{k=1}^{h} \left|(x-t(x))_{i j k}\right|.
    \end{split}
\end{equation}

Table \ref{tab:shift} shows the Average Shift of an image under 15 corruptions with the most severe level. It is shown that most corruptions are within the shift range $\delta=0.26 \approx 60/255$.

Fig.~\ref{fig:shift-6severity} verifies that the Average Shift in sample space increases with the increase of the severity level of most corruptions.



\input{latex/Supplementary_Section/tabs/tab-shift}
\input{latex/Supplementary_Section/imgs/shift_6severity}
%--------------------------------------------------------------------------
\subsection{Proof for Assumption 2}
It is shown in Section 5.4 of the main manuscript.

%------------------------------------------------------------------------
\subsection{Proof for Assumption 3}
Given input target domain $D_{t}=\{(\mathcal{X}_{t},\mathcal{Y}_{t})\}$, source domain $D_{s}=\{(\mathcal{X}_{s},\mathcal{Y}_{s})\}$, a corruption with 5 severity levels $T={\{t_{i}\}}_{1}^{5}$, an ideal transfer loss function $\ell_{trans}$ and a DA model $m=f \circ c$, we first make some notions for precise:

\begin{equation}
    \begin{split}
        \ell_{trans}(t_{i})&=\mathbb{E}_{x_t \sim \mathcal{X}_{t}} \left[\ell_{trans}(f(t_{i}(x_t)),f(\mathcal{X}_{s}))\right],\\
        Acc({t_{i}})&=\mathbb{P}_{(x_{t},y_{t}) \sim D_{t}}(m(t_{i}(x_{t}))=y_{t}),\\
        \ell_{total}(t_{i})&=\ell_{trans}(t_{i})+\ell_{cls}(\mathcal{X}_s,\mathcal{Y}_s), 
    \end{split}
\end{equation}
where $\ell_{trans}(t_{i})$ denotes the average transfer loss of corrupted target domain samples. $Acc({t_{i}})$ denotes the classification accuracy of corrupted target domain samples. $\ell_{cls}(\mathcal{X}_s)$ denotes the classifier loss of source domain samples; $\ell_{total}(t_{i})$ denotes the total loss of a classic DA models, which usually correlated to $Acc({t_{i}})$.

It is observed that the classification accuracy decreases as the increase of the severity level, as:
\begin{equation}
    i<j \Rightarrow Acc({t_{i}}) > Acc({t_{j}}).
    \label{observe}
\end{equation}

We make the proof by contradiction.
If
\begin{equation}
    \begin{split}
        i<j &\Rightarrow \ell_{trans}({t_{i}}) > \ell_{trans}({t_{j}})\\
        &\Rightarrow \ell_{total}(t_{i}) > \ell_{total}(t_{j}), 
    \end{split}
\end{equation}
the final classification accuracy should be $Acc({t_{i}}) < Acc({t_{j}})$. Conflict with Equation (\ref{observe}).




==> CRDA (TOMM)/latex/Supplementary_Section/Proof_Equation6.tex <==
\section{Proof for Equation (3) in the main manuscript}
\label{sec:sup_ProofForEq6}
% \begin{equation}
%     \begin{split}
%     x_{t}^{(DDG)}&=\mathop{\arg\max}_{\left\|x_{t}^{(DDG)}-x_{t}\right\| \leq \delta} \ell_{trans}\left(f(x_{t}^{(DDG)}), f(D_{s})\right)
%     \\&\Rightarrow \mathop{\arg\max}_{t \in T} \ell_{trans}\left(f(t\left(x_{t})\right), f(D_{s})\right)=t_{\max }(x_{t}).
%     \end{split}
%     \label{construction_x_adv}
% \end{equation}

According to Assumption 1, $x_{t}^{(DDG)}$ and $t(x_{t})$ are within the $\delta$ neighborhood $\{x | \left\|x-x_{t}\right\| \leq \delta\}$. 

Suppose $t_{max}$ as the most severe corruption in corruption set $T$. According to Assumption 3, 

\begin{equation}
   t_{max}=\mathop{\arg\max}_{t \in T} \ell_{trans}\left(f(t\left(x_{t})\right), f(D_{s})\right).
\end{equation}

Due to the uncertainty of $T$, the corrupted versions $t(x_{t})$ can be everywhere in $\delta$ neighborhood.
Thus, 
% $\mathop{\max}_{\left\|x_{t}^{(DDG)}-x_{t}\right\| \leq \delta} \ell_{trans}\left(f(x_{t}^{(DDG)}), f(D_{s})\right) = \mathop{\max}_{t \in T} \ell_{trans}\left(f(t\left(x_{t})\right), f(D_{s})\right)$
% 
% , as : 
\begin{equation}
    \begin{split}
    & \ell_{trans}\left(f(x_{t}^{(DDG)}), f(D_{s})\right)
    \\
    &=\ell_{trans}\left(f(t_{max}\left(x_{t})\right), f(D_{s})\right)=\ell_{max}.
    \end{split}
\end{equation}

Suppose that

\begin{equation}
    \begin{split}
     X^{(DDG)}&=\left \{x_{t}^{(DDG)}| \ell_{trans}\left(f(x_{t}^{(DDG)}), f(D_{s})\right)= \ell_{max} \right\}
    \\X^{(tm)}&=\left\{t_{max}(x_{t}) | \ell_{trans}\left(f(t_{max}(x_{t})), f(D_{s})\right) = \ell_{max} \right\}.
    \end{split}
\end{equation}
We get
\begin{equation}
    X^{(DDG)}=X^{(tm)}.
\end{equation}
Thus, $x_{t}^{(DDG)} \in X^{(wc)}$ can represent $t_{max}(x_{t}) \in X^{(tm)}$, as:

\begin{equation}
    x_{t}^{(DDG)} \Rightarrow t_{max}(x_{t}).
\end{equation}

==> CRDA (TOMM)/latex/Supplementary_Section/Worst-Corruption_Sample.tex <==
\section{Instance of worst-corruption sample}
\label{sec:wc_sample}
% \input{latex/Supplementary_Section/imgs/wc_sample}
We show several examples of worse-corruption sample generated by our method, as well as its corresponding clean image, in Figure \ref{fig:wc_sample}.

==> CRDA (TOMM)/latex/Supplementary_Section/imgs/15corruptions.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.85\textwidth]{latex/figs/15corruptions.pdf}
    \caption{Examples of 15 kinds of corruptions.}
    \label{fig:15corruption}
\end{figure*}

==> CRDA (TOMM)/latex/Supplementary_Section/imgs/6severity.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.85\textwidth]{latex/figs/6severity.pdf}
    \caption{Examples of 5 levels of severity.}
    \label{fig:6severity}
\end{figure*}

==> CRDA (TOMM)/latex/Supplementary_Section/imgs/mCE_office-sup.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{latex/figs/mCE-office-supplementary.pdf}
    \caption{mCE ($\%$) on all cross-domain settings of Office-31 under CRDA (ResNet-50).}
    \label{fig:mCE-office-sup}
\end{figure}

==> CRDA (TOMM)/latex/Supplementary_Section/imgs/mCE_officehome-sup.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.96\textwidth]{latex/figs/mCE-officehome-supplementary.pdf}
    \caption{mCE ($\%$) on all cross-domain settings of Office-Home under CRDA (ResNet-50).}
    \label{fig:mCE-officehome-sup}
\end{figure*}

==> CRDA (TOMM)/latex/Supplementary_Section/imgs/mCE_precise-sup.tex <==
\begin{figure}[!h]
    \centering
    % \includegraphics[width=\linewidth]{latex/figs/mCE-precise-supplementary.pdf}
    \includegraphics[width=0.6\linewidth]{latex/figs/mCE-supplementary.pdf}
    \caption{mCE ($\%$) on Office-Home and Office-31 datasets.}
    \label{fig:mCE-precise-sup}
\end{figure}

==> CRDA (TOMM)/latex/Supplementary_Section/imgs/shift_6severity.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{latex/figs/proof_ass1e.pdf}
    \caption{Average Shift of different corruptions with $6$ severity levels.}
    \label{fig:shift-6severity}
\end{figure}

==> CRDA (TOMM)/latex/Supplementary_Section/imgs/wc_sample.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.88\textwidth]{latex/figs/WC_samplee.pdf}
    \caption{Worst-corruption samples of different iterations.}
    \label{fig:wc_sample}
\end{figure*}

==> CRDA (TOMM)/latex/Supplementary_Section/tabs/err_TSCL.tex <==
\begin{table}
    \centering
    \caption{Error rate ($\%$) under a specific known corruption on the Ar$\to$Rw setting of Office-Home dataset for teacher-student warm-up shceme.}
    \label{tab:err_TSCL_full}
    \setlength{\tabcolsep}{3mm}{
    % \small{
    \begin{tabular}{c|ccc}
        \toprule
        \multirow{2}{*}{Corruption} & \multicolumn{3}{c}{CDAN+TN} \\
        \cline{2-4}
         & -  & DataAug & Ours \\
        \hline
        Clean & 22.1 & 24.6 & 21.2\\
        Gaussian Noise & 78.4 & 33.4 & 27.8\\
        Shot Noise & 78.3 & 34.9 & 26.9\\
        Impulse Noise & 83.4 & 33.4 & 24.4\\
        Defocus Blur & 70.4 & 34.9 & 26.7\\
        Motion Blur & 69.5 & 28.4 & 24.3\\
        Zoom Blur & 53.6 & 29.4 & 23.1\\
        Fog & 47.3 & 24.6 & 23.6\\
        Frost & 55.7 & 30.6 & 25.5\\
        Snow & 60.0 & 31.2 & 23.9\\
        Elastic Transform & 84.2 & 30.0 & 23.3\\
        Contrast & 66.4 & 24.6 & 23.0\\
        Brightness & 29.7 & 26.5 & 23.6\\
        JPEG Compression & 37.6 & 29.0 & 23.2\\
        Pixelate & 45.7 & 26.9 & 22.6\\
        Glass Blur & 86.4 & 37.0 & 27.8\\
        \bottomrule
    \end{tabular}
    % }
    }
    \vspace{-1.5mm}
\end{table}

==> CRDA (TOMM)/latex/Supplementary_Section/tabs/tab-ablation.tex <==
% \begin{table}[t]
%     \centering
%     \caption{mCE ($\%$) on Ar$\to$Rw for different parameters in TSCL-WC}
%     \label{tab:Ablation-delta2}
%     \small{
%     \setlength{\tabcolsep}{4mm}{
%     \begin{tabular}{c|ccc|c|c}
%         \toprule
%         object&$\delta$&$\eta$&$n$&mCE ($\downarrow$)&convergence\\
%         \hline
%         \multirow{4}{*}{$\eta$} & $60/255$ & $> 2\delta$ & 2 & 48.0 & 2000\\ 
%         &$60/255$ & $> 2\delta$ & 10 & 49.6 & 3500\\ 
%         &$60/255$ & $15/255$ & 10 & 51.6 & 4000\\ 
%         &$60/255$ & $6/255$ & 10 & 52.8 & 4000\\ 
%         \hline
%         \multirow{7}{*}{$\delta$}&$20/255$ & $> 2\delta$ & 2 & 49.5 & 2000\\ 
%         &$40/255$ & $> 2\delta$ & 2 & 48.6 & 2000\\ 
%         &$60/255$ & $> 2\delta$ & 2 & 48.0 & 2000\\ 
%         &$80/255$ & $> 2\delta$ & 2 & 47.3 & 2500\\
%         &$100/255$ & $> 2\delta$ & 2 & 48.1 & 2500\\
%         &$120/255$ & $> 2\delta$ & 2 & 46.9 & 3000\\
%         &$140/255$ & $> 2\delta$ & 2 & 46.4 & 3000\\
%         \hline
%         \multirow{4}{*}{$n$}&$60/255$ & $> 2\delta$ & 1 & 47.4 & 2000\\
%         &$60/255$ & $> 2\delta$ & 2 & 48.0 & 2000\\
%         &$60/255$ & $> 2\delta$ & 5 & 49.9 & 2000\\
%         &$60/255$ & $> 2\delta$ & 10 & 49.6 & 3500\\
%         \bottomrule
%     \end{tabular}
%     }
%     }
%     \vspace{-3mm}
% \end{table}

\begin{table}[t]
    \centering
    \caption{mCE ($\%$) for different parameters in TSCL-WC on the UDA task of Ar$\to$Rw from Office-Home dataset.}
    \label{tab:Ablation-delta2}
    % \small{
    \setlength{\tabcolsep}{3mm}{
    \begin{tabular}{c|ccc|c}
        \toprule
        object&$\delta$&$\eta$&$n$&mCE ($\downarrow$)\\
        \hline
        \multirow{4}{*}{$\eta$} & $60/255$ & $> 2\delta$ & 2 & 48.0\\ 
        &$60/255$ & $> 2\delta$ & 10 & 49.6\\ 
        &$60/255$ & $15/255$ & 10 & 51.6\\ 
        &$60/255$ & $6/255$ & 10 & 52.8\\ 
        \hline
        \multirow{7}{*}{$\delta$}&$20/255$ & $> 2\delta$ & 2 & 49.5\\ 
        &$40/255$ & $> 2\delta$ & 2 & 48.6\\ 
        &$60/255$ & $> 2\delta$ & 2 & 48.0\\ 
        &$80/255$ & $> 2\delta$ & 2 & 47.3\\
        &$100/255$ & $> 2\delta$ & 2 & 47.2\\
        &$120/255$ & $> 2\delta$ & 2 & 46.9\\
        &$140/255$ & $> 2\delta$ & 2 & 46.4\\
        \hline
        \multirow{4}{*}{$n$}&$60/255$ & $> 2\delta$ & 1 & 47.4\\
        &$60/255$ & $> 2\delta$ & 2 & 48.0\\
        &$60/255$ & $> 2\delta$ & 5 & 49.9\\
        &$60/255$ & $> 2\delta$ & 10 & 49.6\\
        \bottomrule
    \end{tabular}
    % }
    }
    % \vspace{-3mm}
\end{table}

==> CRDA (TOMM)/latex/Supplementary_Section/tabs/tab-shift.tex <==
\begin{table}[t]
    \centering
    \caption{Average Shift of different corruptions}
    \label{tab:shift}
    \setlength{\tabcolsep}{1.2mm}{
    \small{
    \begin{tabular}{c|c||c|c}
        \toprule
         Corruption & Avg shift & Corruption & Avg shift \\
         \hline
         Gaussian Noise & 0.22 & Snow & 0.25\\
         Shot Noise & 0.25 & Elastic Transform & 0.19\\
         Impulse Noise & 0.14 & Contrast & 0.26\\
         Defocus Blur & 0.08 & Brightness & 0.25\\
         Motion Blur & 0.13 & JPEG Compression & 0.04\\
         Zoom Blur & 0.12 & Pixelate & 0.05\\
         Fog & 0.24 & Glass Blur & 0.08\\
         Frost & 0.21 & & \\
         \bottomrule
    \end{tabular}
    }
    }
\end{table}

% \begin{table}
%     \centering
%     \caption{mCE ($\%$) on all cross-domain settings of Office-Home dataset under CRDA (ResNet-50).}
%     \label{tab:mCE_OfficeHome}
%     \setlength{\tabcolsep}{1.2mm}{
%     \small{
%     \begin{tabular}{c|ccc|ccc|c}
%         \toprule
%         \multirow{2}{*}{Settings} & \multicolumn{3}{c|}{CDAN+TN} &\multicolumn{3}{c|}{DCAN} & Lower \\
%         \cline{2-7}
%          & - & AugMix & Ours & - & AugMix & Ours & Bound \\
%         \hline
%         Ar$\to$Cl & 69.7 & 69.3 & 59.8 & 61.4 & 63.2 & 58.3 & 52.2 \\
%         Ar$\to$Pr & 62.2 & 52.8 & 52.2 & 51.0 & 49.3 & 48.0 & 37.7 \\
%         Ar$\to$Rw & 59.2 & 56.0 & 48.0 & 47.9 & 46.0 & 44.6 & 30.8 \\
%         Cl$\to$Ar & 65.4 & 73.7 & 66.0 & 58.6 & 57.4 & 55.2 & 45.8 \\
%         Cl$\to$Pr & 58.7 & 56.6 & 51.9 & 58.0 & 57.3 & 51.6 & 34.6 \\
%         Cl$\to$Rw & 57.6 & 61.3 & 56.2 & 52.0 & 53.8 & 47.5 & 34.7 \\
%         Pr$\to$Ar & 65.5 & 72.2 & 63.6 & 61.1 & 58.9 & 55.1 & 44.7 \\
%         Pr$\to$Cl & 70.9 & 71.4 & 63.6 & 66.2 & 65.3 & 62.2 & 54.9 \\
%         Pr$\to$Rw & 55.0 & 55.3 & 48.8 & 53.7 & 48.5 & 49.4 & 25.7 \\
%         Rw$\to$Ar & 63.2 & 62.4 & 57.8 & 63.0 & 59.2 & 57.7 & 36.0 \\
%         Rw$\to$Cl & 70.4 & 61.4 & 64.4 & 64.0 & 64.2 & 59.9 & 52.9 \\
%         Rw$\to$Pr & 60.9 & 52.6 & 47.9 & 58.4 & 52.5 & 52.6 & 26.8 \\
%         \hline
%         Avg ($\downarrow$) & 63.2 & 62.1 & \textbf{56.7} & 57.9 & 56.3 & \textbf{53.5} & 39.7 \\
%         \bottomrule
%     \end{tabular}
%     }
%     }
%     \vspace{-1.5mm}
% \end{table}
 	 	 	 	 	 	 	 		 	 	 	 
 	 	 	 	 	 	 	 	 	 	 	 	


 	  	 	 	 	 	 	 	 	 	 	 	 	 
	 	 	 	 	 	 	 	 	 	 	 


==> CRDA (TOMM)/latex/algorithm/algorithm-AdvTL.tex <==
\begin{algorithm}[t]
\caption{Overall process for AdvTL}
\begin{algorithmic}[1]
\Require The original DA model $f+c$, source and target domain samples $X=X_s\cup X_t$, source domain labels $Y_s$. Parameters for AdvTL: threshold $\delta$, update stride $\eta > 2\delta$ and update steps $n$.
\State Train the original DA model as the teacher model $f^{(tea)}+c^{(tea)}$. Fix the parameters.
\State 	Construct a student network $f^{(stu)}+c^{(stu)}$ with same structure of $f+c$. 
\Repeat :
\State Get a batch of source and target domain samples $x=\{x_{s},x_{t}\}$ from $X$ and the corresponding labels of source domain samples $y_s$.
\State Construct worst-transformation-case samples $x_{t}^{(adv)}$ by Algorithm \ref{algorithm-PGD}:

$x_{t}^{(adv)}=\text{PGD}(x_{t},x_{s},f^{(stu)},\delta, \eta, n)$
\State  Calculate features representations of target domain samples:

$z_{t}^{(adv)}=f^{(stu)}\left(x_{t}^{(adv)}\right)$


$z_{t}^{(stu)}=f^{(stu)}\left(x_{t}\right)$

$z_{t}^{(tea)}=f^{(tea)}\left(x_{t}\right)$

\State  Calculate features representations of source domain samples:

$z_{s}^{(stu)}=f^{(stu)}\left(x_{s}\right)$

$z_{s}^{(tea)}=f^{(tea)}\left(x_{s}\right)$

\State Calculate classification predict result:

$z_{stu}=z_{t}^{(stu)} \cup z_{s}^{(stu)}$

$y_{stu}=c_{stu}\left(z_{stu}\right)$
\State 	Calculate the loss introduced by the original DA model:

$\ell_{ori}\left(z_{stu},\ y_{stu},\ y_s\right)$
\State Calculate the contrastive loss by \textcolor{red}{Equation (\ref{CL-AdvTL})}: 

$\ell_{contrast}^{(adv)}=\ell_{contrast}\left(z_{t}^{(adv)},z_{t}^{(tea)}\right)$
\State Calculate the total loss $\ell_{total}=\ell_{ori}+\lambda\ell_{contrast}^{(adv)}$
\State Backward grad and update parameters of $f_{stu}+c_{stu}$
\Until Converge
\State \Return $f_{stu}+c_{stu}$

\end{algorithmic}
\label{algorithm-AdvTL}
\end{algorithm}

==> CRDA (TOMM)/latex/algorithm/algorithm-AdvTL_v2.tex <==
\begin{algorithm}[t]
    \caption{Overall process for TSCL-WC}
    \label{algorithm-AdvTL}
    \small{
    \textbf{Input:} 
    \begin{minipage}[t]{0.87\linewidth}
    Data and source labels: $\mathcal{X}_{s}$, $\mathcal{X}_{t}$, $\mathcal{Y}_{s}$; Original DA model $f+c$; Parameters: $\delta=60/255$, $\eta > 2\delta$, $n=2$
    \end{minipage}
    
    \textbf{Output:} 
    \begin{minipage}[t]{0.86\linewidth}
    Robust student model $f^{(stu)}+c^{(stu)}$
    \end{minipage}
    
    \begin{algorithmic}[1]
    \State Train the original model as a teacher model $f^{(tea)}+c^{(tea)}$. Fix the parameters.
    \State 	Construct a student network $f^{(stu)}+c^{(stu)}$ with same structure of $f+c$. 
    \Repeat :
    \State Draw $x_{s}, x_{t}, y_s$ from $\mathcal{X}_{s}, \mathcal{X}_{t}, \mathcal{Y}_{s}$.
    \State 
    \begin{minipage}[t]{0.9\linewidth}
    Construct worst-corruption samples according to Equation (\ref{construction_x_adv}) and Algorithm \ref{algorithm-PGD}:
    
    $\qquad x_{t}^{(wc)}=\text{PGD}\left(x_{t},x_{s},f^{(stu)},\delta, \eta, n\right)$
    \end{minipage}
    
    \State
    Update $f^{(stu)}+c^{(stu)}$ according to Equation (\ref{CL-AdvTL})
    
    and (\ref{total_loss}).
    
    \Until Convergence
    \State \Return $f^{(stu)}+c^{(stu)}$
    
    \end{algorithmic}
    }
\end{algorithm}

==> CRDA (TOMM)/latex/algorithm/algorithm-DDG.tex <==
\begin{algorithm}[t]
    \caption{Overall process for Domain Discrepancy Generator}
    \label{algorithm-DDG}
    \small{
    \textbf{Input:} 
    \begin{minipage}[t]{0.87\linewidth}
    Data and source labels: $\mathcal{X}_{s}$, $\mathcal{X}_{t}$, $\mathcal{Y}_{s}$; Original DA model $f+c$; Parameters: $\delta=60/255$, $\eta > 2\delta$, $n=2$
    \end{minipage}
    
    \textbf{Output:} 
    \begin{minipage}[t]{0.86\linewidth}
    Robust student model $f^{(stu)}+c^{(stu)}$
    \end{minipage}
    
    \begin{algorithmic}[1]
    \State Train the original model as a teacher model $f^{(tea)}+c^{(tea)}$. Fix the parameters.
    \State 	Construct a student network $f^{(stu)}+c^{(stu)}$ with same structure of $f+c$. 
    \Repeat :
    \State Draw $x_{s}, x_{t}, y_s$ from $\mathcal{X}_{s}, \mathcal{X}_{t}, \mathcal{Y}_{s}$.
    \State 
    \begin{minipage}[t]{0.9\linewidth}
    Generate augmentation samples according to Equation (\ref{construction_x_adv}) and Algorithm \ref{algorithm-PGD}:
    
    $\qquad x_{t}^{(DDG)}=\text{PGD}\left(x_{t},x_{s},f^{(stu)},\delta, \eta, n\right)$
    \end{minipage}
    
    \State
    Update $f^{(stu)}+c^{(stu)}$ according to Equation (\ref{total_loss}).
    
    \Until Convergence
    \State \Return $f^{(stu)}+c^{(stu)}$
    
    \end{algorithmic}
    }
\end{algorithm}

==> CRDA (TOMM)/latex/algorithm/algorithm-PGD.tex <==
\begin{algorithm}[t]
    \caption{PGD: Projected Gradient Descent}
    \small{
    \textbf{Input:} 
    \begin{minipage}[t]{0.87\linewidth}
    Target and source doamin data $x_{t},x_{s}$; Feature  extractor $f$;Parameters: shift range $\delta$, update stride $\eta$, update step number $n$.
    \end{minipage}
    
    \textbf{Output:}
    \begin{minipage}[t]{0.86\linewidth}
    augmented target samples by DDG $x_{t}^{(DDG)}$
    \end{minipage}
    
    \begin{algorithmic}[1]
    
    \State $i=0$, $x_{t}^{(DDG)}=x_t$
    \Repeat :
    \State Transfer loss:
    
    $\ell=\ell_{trans}(f(x_{t}^{(DDG)}),f(x_{s}))$
    
    
    \State Update $x_{t}^{(DDG)}$ by the gradients of transfer loss:
    
    $x_{t}^{(DDG)} \leftarrow x_{t}^{(DDG)} + \eta \cdot \text{sign} \left(\frac{\partial {\ell}}{\partial x_{t}^{(DDG)}}\right)$
    
    \State Clamp $x_{t}^{(DDG)}$ within $\left\|x_{t}^{(DDG)}-x_{t}\right\| \leq \delta$
    \State $i \leftarrow i+1$
    \Until $i=n$
    \State \Return $x_{t}^{(DDG)}$
    
    \end{algorithmic}
    \label{algorithm-PGD}
    }
\end{algorithm}

==> CRDA (TOMM)/latex/algorithm/algorithm-TSCL.tex <==
\begin{algorithm}[t]
\caption{Overall process for TSCL}
\begin{algorithmic}[1]
\Require The original DA model $f+c$, source and target domain samples $X=X_s\cup X_t$, source domain labels $Y_s$ and a transformation $T \equiv {\{t_{i}\}}_{0}^{5}$ with six levels of severity during testing ($t_{0}$ denotes clean data).
\State Train the original DA model as the teacher model $f^{(tea)}+c^{(tea)}$. Fix the parameters.
\State 	Construct a student network $f^{(stu)}+c^{(stu)}$ with same structure of $f+c$. 
\Repeat :
\State Get a batch of samples $x$ from $X$ and the corresponding labels of source samples $y_s$.
\State Randomly select a transformation $t$ from $\{t_{0},t_{5}\}$
\State  Calculate features representations:

$z^{(stu)}=f^{(stu)}\left(t(x)\right)$, $z^{(tea)}=f^{(tea)}\left(x\right)$
\State Calculate classification predict result:

$y^{(stu)}=c^{(stu)}\left(z^{(stu)}\right)$
\State 	Calculate the loss introduced by the original DA model:

$\ell_{ori}\left(z^{(stu)},\ y^{(stu)},\ y_s\right)$
\State Calculate the contrastive loss in Equation (\ref{CL}):

$\ell_{contrast}\left(z^{(stu)},z^{(tea)}\right)$
\State Calculate the total loss: $\ell_{total}=\ell_{ori}+\lambda\ell_{contrast}$
\State Backward gradients and update parameters of $f^{(stu)}+c^{(stu)}$
\Until Converge
\State \Return $f^{(stu)}+c^{(stu)}$

\end{algorithmic}
\label{algorithm-TSCL}
\end{algorithm}

==> CRDA (TOMM)/latex/algorithm/algorithm-TSCL_v2.tex <==
\begin{algorithm}[t]
\caption{Overall process for TSCL}
\textbf{Input:} 
\begin{minipage}[t]{0.87\linewidth}
Data and source labels: $\mathcal{X}_{s}$, $\mathcal{X}_{t}$, $\mathcal{Y}_{s}$; Original DA model $f+c$; A corruption with six levels of severity  $T = {\{t_{i}\}}_{0}^{5}$  ($\mathrm t_{0}$ denotes clean data).
\end{minipage}

\textbf{Output:} 
\begin{minipage}[t]{0.86\linewidth}
Robust student model $f^{(stu)}+c^{(stu)}$
\end{minipage}
\begin{algorithmic}[1]
\State Train the original model as a teacher model $f^{(tea)}+c^{(tea)}$. Fix the parameters.
\State 	Construct a student network $f^{(stu)}+c^{(stu)}$ with same structure of $f+c$. 
\Repeat :
\State Draw $x_{s}, x_{t}, y_s$ from $\mathcal{X}_{s}, \mathcal{X}_{t}, \mathcal{Y}_{s}$. $x=\{x_{s}, x_{t}\}$.
\State Randomly draw a corruption $t$ from $\{t_{0},t_{5}\}$
\State  
\begin{minipage}[t]{0.9\linewidth}
\begin{spacing}{1.4}
Update $f^{(stu)}+c^{(stu)}$ according to (\ref{CL}):

    $\qquad \ell_{ori}\left(t(x_{s}),t(x_{t}),y_{s}\right)$

    $\qquad \ell_{con}\left(f^{(stu)}(t(x)),f^{(tea)}(x)\right)$
\end{spacing}
\begin{spacing}{0.5}
    $\qquad \ell_{total}=\ell_{ori}+\lambda\ell_{con}$
\end{spacing}
\end{minipage}
% \begin{minipage}[t]{0.9\linewidth}
% \begin{spacing}{1.4}
% Update $f^{(stu)}+c^{(stu)}$ according to (\ref{CL}):

%     $\qquad \ell_{ori}\left(x_{s},x_{t},y_{s}\right)$

%     $\qquad \ell_{con}\left(f^{(stu)}(x_{t}^{(wc)}),f^{(tea)}(x_{t})\right)$
% \end{spacing}
% \begin{spacing}{0.5}
%     $\qquad \ell_{total}=\ell_{ori}+\lambda\ell_{con}$
% \end{spacing}
% \end{minipage}
\Until Convergence
\State \Return $f^{(stu)}+c^{(stu)}$

\end{algorithmic}
\label{algorithm-TSCL}
\end{algorithm}

==> CRDA (TOMM)/latex/imgs/15corruptions.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.7\textwidth]{latex/figs/15corruptions.pdf}
    \caption{Examples of $15$ kinds of corruptions.}
    \label{fig:15corruption1}
\end{figure*}

==> CRDA (TOMM)/latex/imgs/Error_MostLevel_stage2b_A2R.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.92\textwidth,height=5.4cm]{latex/figs/A2R_mCE_DDG.pdf}
    \caption{Error rate ($\%$) on Ar$\to$Rw of Office-Home for different corruptions with the most severe level under CRDA (ResNet-50).}
    \label{fig:exp3}
    \vspace{-3mm}
\end{figure*}

==> CRDA (TOMM)/latex/imgs/Fig1.tex <==
\begin{figure*}
    \begin{center}
    \includegraphics[width=0.96\textwidth]{latex/figs/figure_stage2be.pdf}
    \end{center}
    \caption{Instances of corruption robust domain adaptation (CRDA).
    %Here labeled clean source domain (art) and unlabeled clean target domain (real world) samples are available while training.
    Existing domain adaptation method (CDAN+TN \cite{wang2019TransNorm}) and corruption robust method (AugMix \cite{hendrycks2019augmix}), even their combination, suffer from unseen corruptions on target domain.}
    \label{fig:illustration}
    \vspace{-3mm}
\end{figure*}

==> CRDA (TOMM)/latex/imgs/ObservationsOfOrder.tex <==
\begin{figure}
    \subfloat[Cosine distance ($\uparrow$)]{
    \begin{minipage}[c][0.4\textwidth]{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{latex/figs/figure_ordere.pdf}
    \end{minipage}}
    % 	\hfill
    \subfloat[Euclidean distance ($\downarrow$)]{
    \begin{minipage}[c][0.4\textwidth]{0.45\textwidth}
    \centering
    \includegraphics[width=\linewidth]{latex/figs/figure_order_eue.pdf}
    \end{minipage}}
    \caption{Feature distance between a clean image and the versions corrupted by five severity levels of Gaussian Noise on the basis of different models: \textbf{Clean} (a ResNet-50 trained on clean data), \textbf{All levels} (trained on all severity levels of Gaussian Noise), \textbf{Clean + Level 5} (trained on clean data and severity level 5 Gaussian Noise), \textbf{Level 5} (trained on data only corrupted by severity level 5).}
    \vspace{-3mm}
    \label{fig:order}
\end{figure}

==> CRDA (TOMM)/latex/imgs/StructureOfAdvTLe.tex <==
\begin{figure}
    \begin{center}
    \includegraphics[width=0.6\textwidth]{latex/figs/DDG.pdf}
    \end{center}
    \caption{Overall structure of DDG. The yellow part is the classic structure of DA, while the green part is DDG. The gradient of transfer loss is inversely added to the target domain inputs by Projected Gradient Descent (PGD)~\cite{madry2017PGD} in Algorithm \ref{algorithm-PGD} to generate augmentation samples $x_{t}^{(DDG)}$ which is aligned with the original domain-invariant feature extracted by a pretrained teacher model with contrastive loss.}
    \label{fig:AdvTL}
    \vspace{-3mm}
\end{figure}

==> CRDA (TOMM)/latex/imgs/illustration.tex <==
\begin{figure*}
    \begin{center}
    \centering
    \includegraphics[width=\textwidth]{latex/figs/figure1_CRDA_tomm.pdf}
    \captionof{figure}{Instances of corruption-agnostic robust domain adaptation (CRDA).
    %Here labeled clean source domain (art) and unlabeled clean target domain (real world) samples are available while training.
    To our surprise, existing domain adaptation method (CDAN+TN \cite{wang2019TransNorm}) and corruption robust method (AugMix \cite{hendrycks2019augmix}), even their combination, suffer from unseen corruptions on target domain.}
    \label{fig:illustration}
    \vspace{-3mm}
    \end{center}
\end{figure*}



==> CRDA (TOMM)/latex/sections/Abstract_v6.tex <==
\begin{abstract}
% 1. DA 目前的发展（套话）
% 2. 更真实且通用的场景——Corruption Robust Domain Adaptation (CRDA): 定义
% 3. 目前方法直接组合在CRDA上效果不好
% 4. 我们的思考：CRDA问题可以分解为两个子问题：
%     (1) domain invariance 和 Corruption 之间的协调 <-- 以往方法组合不好的原因
%     (2) 如何考虑unseen corruption的问题 
% 5. 由此，我们提出了 xxxxx 的方法：
%     (1) 针对问题(1), 我们先不考虑unseen corruption的问题，假设可以得到测试corruption，基于已有DA模型框架，提出TSCL --> 一个基础框架
%     (2) 针对问题(2), 我们采用基于inverting domain discrepency的方式构造worst-corruption sample 来隐式地表示unseen corruption; 并且将TSCL中的随机数据增广替换成worst-corruption sample。
% 6. 实验上看，我们的方法优于现有解决方案
% 7. 有趣的一点是：我们理论证明了只需要考虑最严重的severity就可以handle所有level severity，提升了方法效果和效率。
Big progress has been achieved in domain adaptation in decades. Given unseen corruptions (\eg, noise and blur) in real data, domain adaptation methods are increasingly required to be corruption robust on target domain.
In this paper, we investigate a new task, corruption robust domain adaptation (CRDA): 
% models are required 
to be accurate on clean data and robust against unseen corruptions on target domain.
We observe that popular methods of domain adaptation, corruption robustness, and their combinations, have sub-optimal CRDA results.
% The challenges are two-fold: 1) trade-off between domain invariance and corruption robustness; 2) data augmentation for robustness contributes little to domain adaptation.
The challenges are two-fold: 1) trade-off between domain invariance and corruption robustness; 2) generalization to unseen corruptions via domain information.
% For better results, we present TSCL-WP.
For better results, we present TSCL-WC.
Specifically, we propose a simple but effective teacher-student scheme (TSCL) to balance domain invariance and corruption robustness. %suitable to most DA models on the basis of random data augmentation.
% Besides, we generate worse perturbation (WP) by inverting domain discrepancy to mimic unseen corruptions.
Besides, we generate worst-corruption (WC) samples that most enlarge domain discrepancy to mimic unseen corruptions.
Experiments verify that TSCL-WC keeps performance on clean data and achieves better corruption robustness than baselines.
% Interestingly, \textcolor{red}{we empirically find that networks always learn order-invariant representations for different severity levels of corruptions.} Based on this finding, we theoretically show only considering the most severe corruptions is enough for our framework to gain robustness on all levels of severity.
\end{abstract}

==> CRDA (TOMM)/latex/sections/Abstract_v7.tex <==
\begin{abstract}
% 1. DA 目前的发展（套话）
% 2. 更真实且通用的场景——Corruption Robust Domain Adaptation (CRDA): 定义
% 3. 目前方法直接组合在CRDA上效果不好
% 4. 我们的思考：CRDA的两个挑战：
%     (1) 无标签的目标域
%     (2) 域差异损失约束力较弱
% 5. 由此，我们提出了 xxxxx 的方法：
%     (1) 我们采用基于inverting domain discrepency的方式构造worst-corruption sample 来隐式地表示unseen corruption; 并且将TSCL中的随机数据增广替换成worst-corruption sample。
%     (2) 为了解决训练早期特征不稳定的问题，我们采用teacher-student结构
% 6. 实验上看，我们的方法优于现有解决方案
% 7. 有趣的一点是：我们理论证明了只需要考虑最严重的severity就可以handle所有level severity，提升了方法效果和效率。
Big progress has been achieved in domain adaptation in decades. Existing works are always based on an ideal assumption that testing target domains are i.i.d. with training target domains. However, due to unpredictable corruptions (\eg, noise and blur) in real data like web images, domain adaptation methods are increasingly required to be corruption robust on target domains.
In this paper, we investigate a new task, Corruption-agnostic Robust Domain Adaptation (CRDA): 
% models are required 
to be accurate on original data and robust against unavailable-for-training corruptions on target domains. This task is non-trivial due to large domain discrepancy and unsupervised target domains.
We observe that simple combinations of popular methods of domain adaptation and corruption robustness have sub-optimal CRDA results.
% The challenges are two-fold: 1) unpredictable corruptions with large domain discrepancy; 2) weak constraints for robustness on unlabeled target domain.
We propose a new approach based on two technical insights into CRDA: 1) an easy-to-plug module called Domain Discrepancy Generator (DDG) that generates samples that enlarge domain discrepancy to mimic unpredictable corruptions; 
2) a simple but effective teacher-student scheme with contrastive loss to enhance the constraints on target domains. 
Experiments verify that DDG keeps or even improves performance on original data and achieves better corruption robustness than baselines.
% Interestingly, \textcolor{red}{we empirically find that networks always learn order-invariant representations for different severity levels of corruptions.} Based on this finding, we theoretically show only considering the most severe corruptions is enough for our framework to gain robustness on all levels of severity.
\end{abstract}



==> CRDA (TOMM)/latex/sections/Conclusion_Future_Work_v2.tex <==
\section{Conclusion}
% In this paper, we propose TSCL-WC to investigate a more realistic new task, corruption robustness domain adaptation (CRDA) in the aspect of two key challenges: 1) trade-off between domain invariance and corruption robustness; 2) generalization to unseen domains via domain information. For the first challenge, we propose a Teacher-Student scheme via Contrastive Loss (TSCL) to show that it is better to consider domain invariance and corruption robustness step by step instead of simultaneous training. For the second challenge, taking the particularity of DA into consideration, we present a new idea for corruption robustness that mimic unseen corruptions via worst-corruption samples most enlarging domain discrepancy. Empirical results justify that TSCL-WC outperforms existing baselines on domain invariance and achieves better corruption robustness.
% 
% Future work include a more general scenario, where target domains are unavailable while training. This is in the category of domain generalization. 
In this paper, we propose TSCL-WC to investigate a more realistic new task, corruption robust domain adaptation (CRDA). We propose a Teacher-Student scheme via Contrastive Loss (TSCL) to show that it is better to consider domain invariance and corruption robustness step by step rather than simultaneous learning. Besides, taking domain information into consideration, we present a new idea for corruption robustness that mimic unseen corruptions via worst-corruption samples most enlarging domain discrepancy. Empirical results justify that TSCL-WC outperforms existing baselines on domain invariance and achieves better corruption robustness.

==> CRDA (TOMM)/latex/sections/Conclusion_Future_Work_v3.tex <==
\section{Conclusion}
In this paper, we throw a new sight to domain adaptation to investigate a more realistic new task, Corruption-agnostic Robust Domain Adaptation (CRDA). Taking domain information into consideration, we present a new idea for corruption robustness called Domain Discrepancy Generator (DDG) that mimic unpredictable corruptions via generating samples most enlarging domain discrepancy. Besides, we propose a teacher-student warm-up scheme via contrastive loss to enhance the constraints on unlabelled target domains and stabilize the early training stage feature. Empirical results justify that DDG outperforms existing baselines on original accuracy and achieves better corruption robustness.


==> CRDA (TOMM)/latex/sections/Experiments_v3.tex <==
\section{Experiments}
%------------------------------------------------------------------------------------
\subsection{Setups}
\paragraph{Datasets.} Office-Home and Office-31 are two benchmark datasets widely adopted for visual domain adaptation algorithms. Experiments are mainly conducted on Office-Home, a relatively challenging dataset. 
% Office is an easier dataset to validate generalization of our methods. 
\textit{Office-Home}~\cite{venkateswara2017officehome} is a challenging medium sized benchmark, which contains 15588 images from 4 domains (Artistic images (Ar), Clip Art (Cl), Product images (Pr), and Real-World images (Rw)). Each domain consists of 65 object classes under daily life environment.
\textit{Office-31}~\cite{saenko2010office31} is a standard benchmark with 4110 images and 31 classes under office environment. There are totally three domains: Amazon (A), Webcam (W) and DSLR (D).

\paragraph{Corruption.} To check the corruption robust of one given DA model, we create the corrupted version of Office-31 and Office-Home by using the corruption types defined by ImageNet-C \cite{hendrycks2019benchmarking}, a widely used benchmark for corruption robustness. For each image, there exists $15$ corruption types with $5$ levels of severity as partially illustrated in Figure\ref{fig:illustration} and detailed described in SM. 
% We further test on these two datasets with spatial transformation and the implementation details can be seen in corresponding experiments.

%------------------------------------------------------------------------------------
\paragraph{Baselines} To illustrate the improvement on CRDA, we apply our method on \textbf{CDAN+TN} \cite{long2018conditional,wang2019TransNorm}, a classic baseline model for domain adaptation. We further apply our method to a SOTA DA model \textbf{DCAN} \cite{Li20DCAN}. 
% In addition, our methods can further maintain or improve models' original accuracy. To validate this, another SOTA model \textbf{SHOT} \cite{liang2020shot} is adopted together with CDAN+TN and DCAN.
Note that the domain discrepancies of CDAN+TN and DCAN are respectively measured by adversarial methods~\cite{goodfellow2014GAN} and MMD~\cite{borgwardt2006integrating}. 
We compare our TSCL-WC method with \textbf{AugMix} \cite{hendrycks2019augmix}, a SOTA method for corruption robustness, which aggregates several general transformations such as contrast, equalization and posterization for data augmentation. 
 
 %-----------------------------------------------------------------------------------
 \paragraph{Implementation details}
 For contrastive loss in Equations (\ref{CL}) and (\ref{CL-AdvTL}), the trade-off $\lambda$ is set to $0.5$. For TSCL-WC, we conduct Algorithm \ref{algorithm-DDG} with $\delta=60/255$, $\eta=6$, $n=2$. Network structures and other hyper-parameters are the same as the original DA models. The structure and parameter details of CDAN+TN and DCAN can be seen in SM. 
 
 %-----------------------------------------------------------------------------------
\subsection{Experiments of Trade-off in TSCL}
\input{latex/tabs/acc_rawOfficeHome}
% In this section, we evaluate our TSCL framework method for stage 2-(a). Table \ref{tab:err_TSCL_home} precisely reports the error rate on clean data and some corruptions with the most severe severity. The full results can be seen in SM. Results show that our TSCL can significantly improve the model’s robustness against a specific corruption. Furthermore, TSCL can further improves the model’s original performance instead of negative effect brought by pure data augmentation. In another word, TSCL does not conduct trade-off over robustness and accuracy. 
Assuming testing corruptions available while training, we precisely report the error rate of TSCL on clean data and some corruptions with the most severe severity in Table \ref{tab:err_TSCL_home}. The full results can be seen in SM. Results show that our TSCL can significantly improve the model’s robustness against a specific known corruption. Furthermore, instead of the negative effect brought by simultaneous learning of pure data augmentation, TSCL further improves the model’s average clean accuracy that reflects domain invariance. In another word, the step-by-step learning scheme of TSCL balances the trade-off between domain invariance and corruption robustness well. 

\input{latex/tabs/err_TSCL_OfficeHome_full}

\input{latex/imgs/Error_MostLevel_stage2b_A2R}

%-----------------------------------------------------------------------------------
\subsection{Experiments in CRDA}
We compare TSCL-WC with AugMix and the original DA models on both corruption robustness and original performance which reflects domain invariance. In addition, we further set an empirical lower bound for CRDA calculated by mCE of TSCL applied on CDAN+TN, which assumes testing corruptions are available while training. Models that reach the lower bound can be robust against unseen corruptions as if they are already known beforehand.
 
Figure \ref{fig:exp3} shows the error rate on clean data and 15 different corruptions with the most severe severity in a single setting. It is reported that TSCL-WC achieves improvement over most kinds of corruptions with about 10 percentages in average than the original model and 3 percentages than AugMix.  We observe that AugMix only achieves relatively high robustness on several corruptions such as Fog and Contrast. The reason possibly is that these corruptions can be implied by the aggregation of the general transformations defined by AugMix, however, corruptions like Pixelate may lie out of the implied set. Instead, our TSCL-WC achieves a much more generalizable implied set thanks to reasonable utilization of domain discrepancy information. It is worthy of noting that same like TSCL, TSCL-WC can also improve the original accuracy which reflects domain invariance.

\input{latex/tabs/mCE_OfficeHome}
\input{latex/tabs/mCE_Office}
 
Figure \ref{fig:exp3} also shows that TSCL-WC gains no improvement over the Contrast corruption. We argue the reason probably is that this corruption conducts too much shift in sample space which goes beyond the scope of Assumption~\ref{assum:assum1}. Possible solutions include loosening the constraint in Assumption~\ref{assum:assum1} and considering the invariant order of pixel values (Contrast does not change the order of pixel values). We leave them for future work.

We report the overall robustness under the whole Office-Home and Office-31 datasets in Table \ref{tab:mCE_OfficeHome} and Table \ref{tab:mCE_Office} with the standard robustness metric mCE. Results show that even the SOTA model AugMix has sub-optimal results or even worse  performance in some settings, which indicates the challenge of CRDA. Despite the challenging task, TSCL-WC still gains improvement with obvious margins. Meanwhile, there is still a long way for further study to reach the lower bound in CRDA.
Besides robustness, TSCL-WC also maintains or improves the original accuracy of DA models. Results are shown in Table \ref{tab:acc_OfficeHome}. 

%-----------------------------------------------------------------------------------
% \subsection{Improvement on original accuracy}

% In \textcolor{red}{Experiments xxx}, both TSCL and TSCL-Adv are found beneficial to the original performance. In this section, we respectively apply our methods on \textcolor{red}{classic} model CDAN+TN and two SOTA model DCAN and SHOT. \textcolor{red}{For TSCL, it is found that replacing the random data augmentation with random translation gains stable improvement over all kinds of methods. Random translation randomly translate the input images with at most 1/4 of the image width, which is realized by affine transformation \cite{jaderberg2015STN,shen2016TICNN}. Details about Random Translation and affine transformation can be seen in Appendix. }. \textcolor{red}{Table \ref{tab:acc_OfficeHome}} shows that our methods achieve improvement over all three kinds of DA models. Results shows that SHOT with TSCL-translation can overperform the current SOTA. In summary, TSCL and TSCL-Adv gains improve over both robustness and accuracy \textcolor{red}{instead of trade-off}, which is what most current methods on transformation robustness lack.

% \textcolor{red}{\textbf{Analysis for improvement of TSCL with translation}}

% % \begin{figure*}
% % \begin{center}
% % % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
% % %   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
% % \includegraphics[width=0.9\textwidth]{latex/figs/exp5.png}
% % \end{center}
% %   \caption{accuracy on clean Office-Home data}
% % \label{fig:exp5}
% % \end{figure*}
% \input{latex/tabs/acc_rawOfficeHome}

%-----------------------------------------------------------------------------------
\subsection{Empirical analysis}
\label{sec:empirical}

\paragraph{Ablation.}
\input{latex/tabs/mCE_Ablation-delta}

In Section~\ref{sec:theory}, we theoretically show only considering the edge points on the $\delta$ cycle is enough for TSCL-WC, which is realized by setting stride $\eta > 2\delta$ in Algorithm \ref{algorithm-DDG}. Table \ref{tab:Ablation-delta} reports the mCE under CRDA with different strides $\eta$. Results show that the setting $\eta > 2\delta$, which results in only considering the edge points, gains best performance. We conclude the reason why settings $\eta \ll \delta$ perform relatively poorer is that they may wander in the $\delta$ cycle instead of reaching the large-shift points on the edge, which causes a lack of consideration on large-shift corruptions like contrast and blurs. Table \ref{tab:Ablation-delta} also shows that only 2 update steps is enough for TSCL-WC to gain corruption robustness.
More ablation results can be seen in SM.
\input{latex/imgs/ObservationsOfOrder}

\paragraph{Order-invariant representations of corruptions.}
We empirically observe that the distance between the corrupted versions and the corresponding clean image in feature space (\textbf{feature distance} for precise) is always positively correlated to the severity of corruptions. Training details are shown in SM. Figure \ref{fig:order} shows that even only trained on clean and corrupted samples with a single severity, models still learn the positive correlation instead of relatively nearer feature distance on a specific severity. In a word, networks always learn order-invariant representations in feature space for different levels of severity, which contributes to Assumption~\ref{assum:assum2} in Section~\ref{sec:wc}.


==> CRDA (TOMM)/latex/sections/Experiments_v4.tex <==
\section{Experiments}
%------------------------------------------------------------------------------------
\subsection{Setups}
\paragraph{Datasets.} Office-Home and Office-31 are two benchmark datasets widely adopted for visual domain adaptation algorithms. Experiments are mainly conducted on Office-Home, a relatively challenging dataset. 
% Office is an easier dataset to validate generalization of our methods. 
\textit{Office-Home}~\cite{venkateswara2017officehome} is a challenging medium sized benchmark, which contains 15588 images from 4 domains (Artistic images (Ar), Clip Art (Cl), Product images (Pr), and Real-World images (Rw)). Each domain consists of 65 object classes under daily life environment.
\textit{Office-31}~\cite{saenko2010office31} is a standard benchmark with 4110 images and 31 classes under office environment. There are totally three domains: Amazon (A), Webcam (W) and DSLR (D).

\paragraph{Corruption.} To check the corruption robust of one given DA model, we create the corrupted version of Office-31 and Office-Home by using the corruption types defined by ImageNet-C \cite{hendrycks2019benchmarking}, a widely used benchmark for corruption robustness. For each image, there exists $15$ corruption types with $5$ levels of severity as illustrated in Fig.~\ref{fig:15corruption1}. 
% We further test on these two datasets with spatial transformation and the implementation details can be seen in corresponding experiments.

%------------------------------------------------------------------------------------
\paragraph{Baselines} To illustrate the improvement on CRDA, we apply our method to \textbf{CDAN+TN} \cite{long2018conditional,wang2019TransNorm}, a classic baseline model for domain adaptation. We further apply our method to a SOTA DA model \textbf{DCAN} \cite{Li20DCAN}. 
% In addition, our methods can further maintain or improve models' original accuracy. To validate this, another SOTA model \textbf{SHOT} \cite{liang2020shot} is adopted together with CDAN+TN and DCAN.
Note that the domain discrepancies of CDAN+TN and DCAN are respectively measured by adversarial methods~\cite{goodfellow2014GAN} and MMD~\cite{borgwardt2006integrating}. 
We compare our DDG method with \textbf{AugMix} \cite{hendrycks2019augmix}, a SOTA method for corruption robustness, which aggregates several general transformations such as contrast, equalization and posterization for data augmentation. 
 
 %-----------------------------------------------------------------------------------
 \paragraph{Implementation details}
 For contrastive loss in Equations (\ref{total_loss}), the trade-off $\lambda$ is set to $0.5$. For DDG, we conduct Algorithm \ref{algorithm-DDG} with $\delta=60/255$, $\eta=6$, $n=2$. Network structures and other hyper-parameters are the same as the original DA models.
 
 %-----------------------------------------------------------------------------------
% \subsection{Experiments of Trade-off in TSCL}
\input{latex/tabs/acc_rawOfficeHome}
% % In this section, we evaluate our TSCL framework method for stage 2-(a). Table \ref{tab:err_TSCL_home} precisely reports the error rate on clean data and some corruptions with the most severe severity. The full results can be seen in SM. Results show that our TSCL can significantly improve the model’s robustness against a specific corruption. Furthermore, TSCL can further improves the model’s original performance instead of negative effect brought by pure data augmentation. In another word, TSCL does not conduct trade-off over robustness and accuracy. 
% Assuming testing corruptions available while training, we precisely report the error rate of TSCL on clean data and some corruptions with the most severe severity in Table \ref{tab:err_TSCL_home}. The full results can be seen in SM. Results show that our TSCL can significantly improve the model’s robustness against a specific known corruption. Furthermore, instead of the negative effect brought by simultaneous learning of pure data augmentation, TSCL further improves the model’s average clean accuracy that reflects domain invariance. In another word, the step-by-step learning scheme of TSCL balances the trade-off between domain invariance and corruption robustness well. 

% 

\input{latex/imgs/Error_MostLevel_stage2b_A2R}

%-----------------------------------------------------------------------------------
\subsection{Experiments in CRDA}
We compare DDG with AugMix and the original DA models on both corruption robustness and original performance. In addition, we further set an empirical lower bound for CRDA calculated by simply replacing DDG-generated samples in Algorithm \ref{algorithm-DDG} with corresponding corrupted samples,which means models that reach the lower bound can be robust against unpredictable corruptions as if they are already known beforehand.
 
Fig.~\ref{fig:exp3} shows the error rate on clean data and 15 different corruptions with the most severe severity in a single setting. It is reported that DDG achieves improvement over most kinds of corruptions with about 10 percentages in average than the original model and 3 percentages than AugMix.  We observe that AugMix only achieves relatively high robustness on several corruptions such as Fog and Contrast. The reason possibly is that these corruptions can be implied by the aggregation of the general transformations defined by AugMix, however, corruptions like Pixelate may lie out of the implied set. Instead, our DDG achieves a much more generalizable implied set thanks to reasonable utilization of domain discrepancy information. It is worthy of noting that DDG can also improve the original accuracy, which is detailedly reported in Table \ref{tab:acc_OfficeHome}.

\input{latex/tabs/mCE_OfficeHome}
\input{latex/tabs/mCE_Office}
 
Fig.~\ref{fig:exp3} also shows that DDG gains no improvement over the Contrast corruption. We argue the reason probably is that this corruption conducts too much shift in sample space which goes beyond the scope of Assumption~\ref{assum:assum1}. Possible solutions include loosening the constraint in Assumption~\ref{assum:assum1} and considering the invariant order of pixel values (Contrast does not change the order of pixel values). We leave them for future work.

We report the overall robustness under the whole Office-Home and Office-31 datasets in Table \ref{tab:mCE_OfficeHome} and Table \ref{tab:mCE_Office} with the standard robustness metric mCE. Results show that even the SOTA model AugMix has sub-optimal results or even worse  performance in some settings, which indicates the challenge of CRDA. Despite the challenging task, DDG still gains improvement with obvious margins. Meanwhile, there is still a long way for further study to reach the lower bound in CRDA.
Besides robustness, DDG also maintains or improves the original accuracy of DA models. Results are shown in Table \ref{tab:acc_OfficeHome}. 

%-----------------------------------------------------------------------------------
% \subsection{Improvement on original accuracy}

% In \textcolor{red}{Experiments xxx}, both TSCL and TSCL-Adv are found beneficial to the original performance. In this section, we respectively apply our methods on \textcolor{red}{classic} model CDAN+TN and two SOTA model DCAN and SHOT. \textcolor{red}{For TSCL, it is found that replacing the random data augmentation with random translation gains stable improvement over all kinds of methods. Random translation randomly translate the input images with at most 1/4 of the image width, which is realized by affine transformation \cite{jaderberg2015STN,shen2016TICNN}. Details about Random Translation and affine transformation can be seen in Appendix. }. \textcolor{red}{Table \ref{tab:acc_OfficeHome}} shows that our methods achieve improvement over all three kinds of DA models. Results shows that SHOT with TSCL-translation can overperform the current SOTA. In summary, TSCL and TSCL-Adv gains improve over both robustness and accuracy \textcolor{red}{instead of trade-off}, which is what most current methods on transformation robustness lack.

% \textcolor{red}{\textbf{Analysis for improvement of TSCL with translation}}

% % \begin{figure*}
% % \begin{center}
% % % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
% % %   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
% % \includegraphics[width=0.9\textwidth]{latex/figs/exp5.png}
% % \end{center}
% %   \caption{accuracy on clean Office-Home data}
% % \label{fig:exp5}
% % \end{figure*}
% \input{latex/tabs/acc_rawOfficeHome}

%-----------------------------------------------------------------------------------
\subsection{Empirical analysis}
\label{sec:empirical}

\paragraph{Ablation.}
\input{latex/tabs/mCE_Ablation-delta}

In Section~\ref{sec:theory}, we theoretically show only considering the edge points on the $\delta$ cycle is enough for DDG, which is realized by setting stride $\eta > 2\delta$ in Algorithm \ref{algorithm-DDG}. Table \ref{tab:Ablation-delta} reports the mCE under CRDA with different strides $\eta$. Results show that the setting $\eta > 2\delta$, which results in only considering the edge points, gains best performance. We conclude the reason why settings $\eta \ll \delta$ perform relatively poorer is that they may wander in the $\delta$ cycle instead of reaching the large-shift points on the edge, which causes a lack of consideration on large-shift corruptions like contrast and blurs. Table \ref{tab:Ablation-delta} also shows that only 2 update steps is enough for DDG to gain corruption robustness.
More ablation results can be seen in Appendix.
\input{latex/imgs/ObservationsOfOrder}

\paragraph{Teacher-student warm-up scheme.} 
In this section, we aim to evaluate the effectiveness of the teacher-student warm-up scheme. To compare with simply augmenting samples with testing corruptions, we replace DDG-generated samples in Algorithm \ref{algorithm-DDG} with corresponding testing corruptions. Table \ref{tab:err_TSCL_home} precisely reports the error rate on original data and corruptions with the most severe severity.  Results show that our warm-up scheme can significantly improve the model’s robustness against a specific corruption. Furthermore, our scheme can further improves the model’s original performance instead of negative effect brought by pure data augmentation. In another word, the teacher-student warm-up scheme does not conduct trade-off over robustness and accuracy. 
\input{latex/tabs/err_TSCL_OfficeHome_full}

\paragraph{Order-invariant representations of corruptions.}
We empirically observe that the distance between the corrupted versions and the corresponding clean image in feature space (\textbf{feature distance} for precise) is always positively correlated to the severity of corruptions. Training details are shown in the supplementary material. Fig.~\ref{fig:order} shows that even only trained on clean and corrupted samples with a single severity (Clean + Level 5), models still learn the positive correlation instead of relatively nearer feature distance on a specific severity. In a word, networks always learn order-invariant representations in feature space for different levels of severity, which contributes to Assumption~\ref{assum:assum2} in Section~\ref{sec:wc}.

% \input{latex/tabs/acc_rawOffice}


==> CRDA (TOMM)/latex/sections/Introduction_v4.tex <==
\section{Introduction}
% In the study of visual generalization, researchers mainly focus on robustness on domain shift and common corruptions. Domain shift is mainly studied by domain adaptation (DA) \cite{pan2009survey,long2018conditional,wang2019transferable,Li20DCAN,liang2020shot} and domain generalization (DG) \cite{volpi2018generalizing,dg_mmld,huang2020self} based on the scenario where labeled source domain samples (and unlabeled target domain samples for DA) are available while training to perform classification on target domain. Contributions to corruption robustness focus on the performance of the corrupted testing data (\eg, noise and blur) \cite{hendrycks2019benchmarking,hendrycks2019augmix,sun19ttt,hendrycks2019using}. However, researchers of DA or DG mainly consider domain shift on clean data, while current corruption robustness works focus on corruptions without domain shift. In a word, these two studies with a common goal for generalization \textcolor{red}{deliberately} ignored each other. Thus, there is a question to which both of them must face up: 
% 
% \textit{How to achieve both domain invariance and corruption robustness in a more generalized way?}
% 
\input{latex/imgs/illustration}
Domain adaptation (DA)~\cite{pan2009survey} is a promising technique to transfer knowledge from well-labeled source domain to assist unlabeled target domain learning  with domain shift. Tremendous efforts on domain adaptation~\cite{Li20DCAN,liang2020shot,wang2019TransNorm,long2018conditional} and domain generalization (DG)~\cite{huang2020self,dg_mmld,volpi2018generalizing} indicate the significant progress on domain shift. Besides domain shift, given unseen corruptions (\eg, noise and blur) in real data, domain adaptation methods are increasingly required to be corruption robust on target domain (see Figure~\ref{fig:illustration}). However, most DA or DG works only consider domain shift on clean data, while corruption robustness works~\cite{hendrycks2019benchmarking,hendrycks2019using,hendrycks2019augmix,sun19ttt} usually focus on corruptions without domain shift. Thus, there is a question worth considering: 
\textit{How to build domain invariance with corruption robustness in a more generalized way?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \input{latex/tabs/differentDAsettings}

%Taking into consideration this question, we investigate a more realistic new task,
According to this question, we propose a new task: \textbf{Corruption Robust Domain Adaptation (CRDA)}, \ie, DA models are required to achieve high performance not only on clean target domain that reflects domain invariance, but also be robust against \textbf{unseen} corruptions that are unavailable for training.
%Popular methods of domain adaptation and corruption robustness, even their combinations, 
Popular DA methods, even combining with corruption robustness modules, will get sub-optimal results (Figure~\ref{fig:illustration}) because they cannot handle well two challenges of CRDA: 
%(1) Trade-off between domain invariance and corruption robustness. These two properties may conflict to each other due to \textcolor{red}{different optimization directions.}
(1) trade-off between domain invariance and corruption robustness, which may conflict to each other due to different optimization directions;
(2) generalization to unseen corruptions via domain information. 
% reasonable utilization of domain information helps improving generalization to unseen corruptions. 
It is still rarely investigated that how to take reasonable utilization of domain information for generalization to unseen corruptions.
Meanwhile, data augmentation may have no sense because it only encourages networks to memorize the specific corruptions seen during training and leaves models unable to generalize to new corruptions~\cite{geirhos2018generalisation,hendrycks2019augmix,vasiljevic2016examining}.
To our knowledge, our work is among the first attempt to unify robustness on domain shift and common corruptions.

To address the above challenges, we propose a novel mechanism towards corruption robust domain adaptation.
%Considering the above two key problems, our attempts are as following:
For the first challenge, instead of gaining domain invariance and corruption robustness simultaneously, we propose a Teacher-Student scheme via Contrastive Loss (TSCL) to obtain these two properties step by step. Specifically, a teacher model is first pre-trained to learn domain-invariant representations and then a student model further distills from the teacher model to learn robustness against a specific known corruption via contrastive loss drawn from contrastive learning~\cite{chen2020simple}.
%For the second challenge, based on several assumptions (detailedly discussed in Section~\ref{sec:wc}), \textbf{worst-corruption samples} which most enlarge domain discrepancy are generated to represent unseen corruptions.
% More specifically, instead of minimizing, we construct worst-corruption samples based on the idea of inverting domain discrepancy, which inversely adds the gradients of domain discrepancy loss to the clean inputs by Project Gradient Descent (PGD)~\cite{madry2017PGD}.
For the second challenge, based on several assumptions (see Section~\ref{sec:wc}), we mimic unseen corruptions via worst-corruption (WC) sample generation.
Specifically, instead of minimizing the domain discrepancy, we construct worst-corruption samples by inversely adding the gradients of domain discrepancy loss to the clean inputs by Project Gradient Descent (PGD)~\cite{madry2017PGD}.
Thus, by replacing samples augmented by a specific known corruption in TSCL with WC samples, the proposed \textit{TSCL-WC} method effectively handles the two challenges and achieve better CRDA results.
%Thus, by replacing samples augmented by a specific known corruption in TSCL with Worst-Corruption (WC) samples, we present \textbf{TSCL-WC} for CRDA, which can handle both challenges introduced above.

Our work makes the following contributions:
\begin{itemize}
    \item We investigate a new scenario called corruption robust domain adaptation (CRDA) to equip domain adaptation models with corruption robustness.
    
    \item We propose a novel method for corruption robustness that mimic unseen corruptions via information of domain discrepancy.
    
    \item Experiments demonstrate that our method not only significantly improves corruption robustness for DA models but also maintains or improves classification results on clean target domain.
\end{itemize}

==> CRDA (TOMM)/latex/sections/Introduction_v5.tex <==
\section{Introduction}
% In the study of visual generalization, researchers mainly focus on robustness on domain shift and common corruptions. Domain shift is mainly studied by domain adaptation (DA) \cite{pan2009survey,long2018conditional,wang2019transferable,Li20DCAN,liang2020shot} and domain generalization (DG) \cite{volpi2018generalizing,dg_mmld,huang2020self} based on the scenario where labeled source domain samples (and unlabeled target domain samples for DA) are available while training to perform classification on target domain. Contributions to corruption robustness focus on the performance of the corrupted testing data (\eg, noise and blur) \cite{hendrycks2019benchmarking,hendrycks2019augmix,sun19ttt,hendrycks2019using}. However, researchers of DA or DG mainly consider domain shift on clean data, while current corruption robustness works focus on corruptions without domain shift. In a word, these two studies with a common goal for generalization \textcolor{red}{deliberately} ignored each other. Thus, there is a question to which both of them must face up: 
% 
% \textit{How to achieve both domain invariance and corruption robustness in a more generalized way?}
% 
\input{latex/imgs/illustration}
Domain adaptation (DA)~\cite{pan2009survey} is a promising technique to transfer knowledge from well-labeled source domain to assist unlabeled target domain learning  with domain shift. Tremendous efforts on domain adaptation~\cite{Li20DCAN,liang2020shot,wang2019TransNorm,long2018conditional} and domain generalization (DG)~\cite{huang2020self,dg_mmld,volpi2018generalizing} indicate the significant progress on domain shift. Besides domain shift, given unpredictable corruptions (\eg, noise and blur) in real data, domain adaptation methods are increasingly required to be corruption robust on target domain (see Fig.~\ref{fig:illustration}). However, most DA or DG works only consider transferring source domain knowledge to some specific target datasets, while corruption robustness works~\cite{hendrycks2019benchmarking,hendrycks2019using,hendrycks2019augmix,sun19ttt} usually focus on corruptions without domain shift. Thus, there is a question worth considering: 
\textit{how to conduct robustness against unpredictable corruptions in cross domain scenarios?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \input{latex/tabs/differentDAsettings}

%Taking into consideration this question, we investigate a more realistic new task,
According to this question,  we propose a new task: \textbf{Corruption-agnostic Robust Domain Adaptation (CRDA)}, \ie, DA models are required to not only achieve high performance on original target domains, but also be robust against common corruptions that are \textbf{unavailable for training}.
%Popular methods of domain adaptation and corruption robustness, even their combinations, 
Popular DA methods, even combining with existing corruption robustness modules, will get sub-optimal results (see Fig.~\ref{fig:illustration}) because they cannot handle well two challenges of CRDA: 
%(1) Trade-off between domain invariance and corruption robustness. These two properties may conflict to each other due to \textcolor{red}{different optimization directions.}
(1) unpredictable corruptions with large domain discrepancy;
(2) weak constraints for robustness on unlabeled target domains. More specifically, previous augmentation robustness methods~\cite{hendrycks2019augmix,zhang2017mixup} for corruption-agnostic robustness are always conducted in supervised scenarios with strong classification loss, which may lose effectiveness with domain discrepancy loss on target domains. 
% reasonable utilization of domain information helps improving generalization to unseen corruptions. 
We first show that after taking into domain information, we can construct more generalized augmentation in cross-domain scenarios.
% Meanwhile, data augmentation may have no sense because it only encourages networks to memorize the specific corruptions seen during training and leaves models unable to generalize to new corruptions~\cite{geirhos2018generalisation,hendrycks2019augmix,vasiljevic2016examining}.
To our knowledge, our work is among the first attempt to unify robustness on domain shift and common corruptions.

To address the above challenges, we propose a novel mechanism towards corruption-agnostic robust domain adaptation called Domain Discrepancy Generator (DDG). Specifically, DDG generates augmentation samples that most enlarge domain discrepancy. Based on several assumptions (detailedly discussed in Section~\ref{sec:wc}),  these generated samples are proved to be able to represent unpredictable corruptions. Besides, to enhance the constraints on target domains and tackle with unstable features in the early training stage, we  propose a teacher-student warm-up scheme via contrastive loss. Specifically, a teacher model is first pre-trained to learn the original representations and then a student model further distills from the teacher model to learn robustness against samlpes generated by DDG via contrastive loss drawn from contrastive learning~\cite{chen2020simple}. Our code is available at \url{https://github.com/Mike9674/CRDA}.


Our work makes the following contributions:
\begin{itemize}
    \item We investigate a new scenario called corruption-agnostic robust domain adaptation (CRDA) to equip domain adaptation models with corruption robustness.
    
    \item We take use of information of domain discrepancy to propose a novel module Domain Discrepancy Generator (DDG) for corruption robustness that mimic unpredictable corruptions.
    
    \item Experiments demonstrate that our method not only significantly improves corruption robustness for DA models but also maintains or even improves classification results on original target domains.
    % \eg, the SOTA model DCAN achieves better performance with DDG.
\end{itemize}

==> CRDA (TOMM)/latex/sections/Methodology_v4.tex <==
% 1. TSCL
%     分析挑战(1) --> 以往方法不好的原因之一是同时训练时会冲突 --> 在这样的情况下很难handle trade-off。
%     抛弃同时训练，我们一步一步来 --> TSCL

% 2. worst-corruption samples via inverting domain discrepancy
%     TSCL的问题：只能用data augmentation 处理已知的corruption。 + 通常Data Augmentation不适用于unseen corruption. 
%     --> 利用DA特有的domain信息来构造可以模拟unseen corruption的样本。
    
%     --> Adv

% 3. TSCL-WC
%     总体描述 + 只要handle最严重的corruption就可以了

% 4. Theoretical Explanation

% 5. Metrics
\section{Methodology}
% In this paper, our attempts are made through two key problems of CRDA: 1) trade-off between domain invariance and corruption robustness; 2) generalization to unseen corruptions via domain information. we first propose a simple but effective teacher-student scheme (TSCL) for the first problem. As for the second problem, we further construct worst-corruption samples to mimic unseen corruptions via inversely enlarging domain discrepancy. Putting them together, we derive \textbf{TSCL-WC} as illustrated in Figure \ref{fig:AdvTL}. In addition, we theoretically show that only considering the most severe level of corruptions is  enough for our frameworks to handle all levels of severity.

%----------------------------------------------------------------------------------------------------------
\subsection{Teacher-Student Scheme via Contrastive Loss}
Due to different optimization directions, it is hard to handle domain invariance and corruption robustness at the same time, which results in sub-optimal performance of direct combinations of current works on domain adaptation and corruption robustness. Thus, instead of simultaneous training, we propose a Teacher-Student scheme via Contrastive Loss (TSCL) inspired by contrastive learning~\cite{chen2020simple} to learn these two properties step by step. 

We first assume testing corruptions are available while training so that models only need to learn robustness against a specific known corruption. Algorithm~\ref{algorithm-TSCL} shows the overall process of TSCL. We first gain domain-invariant representations by a pre-trained teacher model based on the traditional DA setting. During the training of the student model, together with random data augmentation, features of the augmented data are aligned with corresponding clean features of the teacher model by contrastive loss introduced below.

\input{latex/algorithm/algorithm-TSCL_v2}

Given a batch of samples ${\{x_i\}}_1^N$, we use feature extractor $f^{(tea)}$ and $f^{(stu)}$ introduced in Algorithm \ref{algorithm-TSCL} to get $2N$ representation feature vectors:
\begin{equation}
    \begin{split}
        Z^{(tea)}={\left\{z_{i}^{(tea)}|z_{i}^{(tea)}=f^{(tea)}(x_i)\right\}}_1^N,\\
        Z^{(stu)}={\left\{z_{i}^{(stu)}|z_{i}^{(stu)}=f^{(stu)}(x_i)\right\}}_1^N,
    \end{split}
\end{equation}
% $Z^{(tea)}={\{z_{i}^{(tea)}|z_{i}^{(tea)}=f^{(tea)}(x_i)\}}_1^N$ and $Z^{(stu)}={\{z_{i}^{(stu)}|z_{i}^{(stu)}=f^{stu}(x_i)\}}_1^N$. 
where we define $Z=Z^{(tea)}\cup Z^{(stu)}={\{z_i\}}_1^{2N}$. The similarity loss of each two features can be calculated by:
%
\begin{equation}
    \ell_{sim}\left(z_{i}, z_{j}\right)=-\log \frac{\exp \left(sim\left(z_{i}, z_{j}\right) / \tau\right)}{\sum_{z_{k} \in Z, z_{k} \neq z_{i}} \exp \left(sim\left(z_{i}, z_{k}\right) / \tau\right)},
    \label{similarity}
\end{equation}
%
where $\tau=0.2$ is a temperature controller to control the similarity extent, and $sim\left(z_i,z_j\right)={z_i}^T z_j/z_i z_j$ is cosine distance between two vectors. 
% which is $sim\left(z_i,z_j\right)={z_i}^T z_j/z_i z_j$. 
Note that Equation (\ref{similarity}) is asymmetric between $z_i, z_j$. The final contrastive loss is defined by:
%
\begin{equation}
    \begin{split}
    \ell_{con}\left(Z^{(stu)}, Z^{(tea)}\right)
    = \frac{1}{2 N} \sum_{i=1}^{N} \left[\ell_{sim}\left(z_{i}^{(stu)}, z_{i}^{(tea)}\right)+ \ell_{sim}\left(z_{i}^{(tea)}, z_{i}^{(stu)}\right)\right],
    \end{split}
    \label{CL}
\end{equation}
%
where the goal is to minimize the distance between feature representations $z_{i}^{(stu)}$ and $z_{i}^{(tea)}$ of a same sample $x_i$. The other kinds of losses defined by the original DA models $\ell_{ori}$ also need to be calculated.

% The overall process of TSCL is shown in \textcolor{red}{Algorithm \ref{algorithm-TSCL}}. 
It is worthy of noting that only the most severe level of corruption $T$ ($t_{5}$ in Algorithm \ref{algorithm-TSCL}) is considered to achieve robustness on all severity levels. The theoretical explanation is described in Section~\ref{sec:theory}. In fact, contrastive loss does not make $Z^{(stu)}$ definitely same as $Z^{(tea)}$. And thanks to corruptions, the final feature representation $Z^{(stu)}$ has a further distillation on the basis of the teacher model, which may lead to not only improvement on robustness but also better performance on domain invariance.

%------------------------------------------------------------------------------------------
\subsection{Worst-Corruption Sample}
\label{sec:wc}

In TSCL, there exists a strong assumption that testing corruptions are available during training. Besides, data augmentation in TSCL only encourages networks to memorize the specific corruptions seen during training and leaves models unable to generalize to new corruptions~\cite{geirhos2018generalisation,vasiljevic2016examining}. 
Thus, we further propose worst-corruption samples most enlarging domain discrepancy to mimic unseen corruptions.

We first assume that corrupted target domain samples hold larger domain discrepancy to source domain than corresponding clean ones, which is empirically proved in SM. 
In domain adaptation, the domain discrepancy is always measured by transfer loss, which is commonly realized by Maximum Mean Discrepancy (MMD) \cite{borgwardt2006integrating,Li20DCAN,long2015DAN,pan2010TCA} or adversarial methods \cite{ganin2016DANN,long2018conditional}. 
Thus, our core idea is to find the points near the original images in sample space that most increase the transfer loss (\textbf{worst-corruption samples} for precise) to represent the most severe corruptions. 

The followings are three basic assumptions for our method, where distance $d_{*}(t(x),x)$ denotes distance between the corrupted images and corresponding clean images:
\begin{assumption}
\label{assum:assum1}
The corrupted versions are within the $\delta$-range neighborhood of the original clean image in sample space ($\boldsymbol{\delta}$ \textbf{cycle} for precise) and distance in sample space $d_{s}(t(x),x)$ becomes larger with increase of the severity level of corruption $T$.
\end{assumption}
\begin{assumption}
\label{assum:assum2}
Within the $\delta$ cycle, the severity level $t$ of a corruption  $T$ is positively correlated to distance in feature space  $d_{f}(f(t(x)) ,f(x))$.
\end{assumption}
\begin{assumption}
\label{assum:assum3}
Within the $\delta$ cycle, the severity level $t$ of a corruption $T$ is positively correlated to the value of transfer loss $\ell_{trans}(t(x))$.
\end{assumption}

The empirical proof can be seen in SM. Assumption~\ref{assum:assum2}  is drawn from an interesting finding in Section~\ref{sec:empirical} that networks always learn order-invariant representations for different severity levels of corruptions.

Based on the above assumptions, we can construct the worst-corruption sample. Given an input target domain data $x_{t}$, source domain $D_{s}$, transfer loss $\ell_{trans}$ and a corruption set $T$ ($t \in T$) whose corresponding corrupted data $t(x_{t})$ is within the $\delta$ cycle of $x_{t}$, we get
\begin{equation}
    \begin{split}
    x_{t}^{(wc)}&=\mathop{\arg\max}_{\left\|x_{t}^{(wc)}-x_{t}\right\| \leq \delta} \ell_{trans}\left(f(x_{t}^{(wc)}), f(D_{s})\right)
    \\&\Rightarrow \mathop{\arg\max}_{t \in T} \ell_{trans}\left(f(t\left(x_{t})\right), f(D_{s})\right)=t_{\max }(x_{t}),
    \end{split}
    \label{construction_x_adv}
\end{equation}
which means the point $x_{t}^{(wc)}$ near the original target domain sample in sample space that most increases transfer loss (\textbf{worst-corruption sample} for precise) can represent the most severe corruption. The idea behind $x_{t}^{(wc)}$ is: instead of minimizing, we mimic unseen corruptions via inversely enlarging domain discrepancy. The proof of Equation (\ref{construction_x_adv}) can be seen in SM.
In practice, worst-corruption samples are constructed by Project Gradient Descent (PGD)~\cite{madry2017PGD} in Algorithm \ref{algorithm-PGD}.
\input{latex/algorithm/algorithm-PGD}
\input{latex/imgs/StructureOfAdvTLe}

\textcolor{red}{It is worthy noting that the worst-corruption samples looks similar to adversarial samples~\cite{madry2017PGD}. However, there exists few evidence that adversarial training contributes a lot to corruption robustness in previous study. We first show that it significantly improves corruption robustness on the basis of the bridge between corruption and domain discrepancy constructed by Assumption \ref{assum:assum3}. Meanwhile, worst-corruption samples are constructed in a unsupervised way while common adversarial training always needs groundtruth labels.}

%----------------------------------------------------------------------------------
\subsection{TSCL-WC}
\label{sec:tscl-wc}

Replacing the random corrupted samples $t(x)$ in Algorithm \ref{algorithm-TSCL} of TSCL with Worst-Corruption samples $x_{t}^{(wc)}$, we derive the final framework \textbf{TSCL-WC} shown in Figure \ref{fig:AdvTL}.

By minimizing distance between worst-corruption samples $x_{t}^{(wc)}$ and original clean samples $x_{t}$ in feature space iteratively, features of the most severely corrupted images come closer to original clean ones, as:
\begin{equation}
    \min d_{f}\left(f(x_{t}^{(wc)}), f(x_{t})\right) \Rightarrow \min d_{f}\left(f(t_{max}(x_{t})), f(x_{t})\right),
    \label{illustration1}
\end{equation}
which leads to better performance on robustness against unseen corruptions. In practice, we realized Equation (\ref{illustration1}) by contrastive loss defined in Equation (\ref{CL}):
\begin{equation}
    \ell_{con}^{(wc)}\left(x_{t}^{(wc)},x_{t}\right)=\ell_{con}\left(f^{(stu)}(x_{t}^{(wc)}),f^{(tea)}(x_{t})\right)
    \label{CL-AdvTL},
\end{equation}
where $f^{(stu)}$ denotes a student model with the same structure as the original DA model to learn corruption robustness and $f^{(tea)}$ is a fixed teacher model trained by the setting of the original DA model. Together with the loss defined by the original DA model $\ell_{ori}$, which commonly contains classifier loss on source domain and transfer loss as illustrated in Figure \ref{fig:AdvTL}, the final total loss is:
\begin{equation}
    \ell_{total}=\ell_{ori}(x_{s},x_{t},y_{s})+\lambda \ell_{con}^{(wc)}(x_{t}^{(wc)},x_{t}).
    \label{total_loss}
\end{equation}

Note that the worst-corruption samples are only constructed on target domain and only processed by contrastive loss. As shown in Algorithm \ref{algorithm-AdvTL}, the overall procedure of TSCL-WC is an extended version of TSCL, which replaces the random corrupted samples $t(x)$ in Algorithm \ref{algorithm-TSCL} with worst-corruption samples $x_{t}^{(wc)}$ to generalize to unseen corruptions.

\input{latex/algorithm/algorithm-AdvTL_v2}

%-----------------------------------------------------------------------------------------
\subsection{Theoretical explanation}
\label{sec:theory}
\textcolor{red}{Intuively, worst-corruption samples should loop many times like $n=10$ in PGD, which is time-consuming. In this section, we theoretically show that we only need to consider the edge point so that by setting $n=2$ is enough, which effectively reduces the time consumption. We begin with the following two propositions, respectively for TSCL and TSCL-WC:} 

\begin{theorem}
Only aligning the most severe level of a corruption is enough to gain robustness under TSCL.
\label{pro1}
\end{theorem}
\begin{theorem}
Only aligning the edge points in the $\delta$ cycle $\{x_{t}^{(wc)}|\|x_{t}^{(wc)}-x_{t}\|=\delta\}$ is enough to gain corruption robustness under TSCL-WC framework.
\label{pro2}
\end{theorem}

Intuitively, aligning all points in the $\delta$ cycle $\{x_{t}^{(wc)}|\|x_{t}^{(wc)}-x_{t}\| \leq \delta\}$ in Equation (\ref{construction_x_adv}) by setting $\eta \ll \delta$ in Algorithm \ref{algorithm-PGD} seems like a reasonable setting, however, we theoretically and empirically show that only aligning the edge points $\{x_{t}^{(wc)}|\|x_{t}^{(wc)}-x_{t}\|=\delta\}$ is enough for TSCL-WC based on Assumption~\ref{assum:assum2}. We first prove Proposition \ref{pro1} for TSCL, then further extend to Proposition \ref{pro2} for TSCL-WC. The theoretical explanations are as followed. 
 
\subsubsection{Proposition 1 for TSCL}
Given input data $x$, a feature extractor $f$ and a corruption $T$ with continuous severity, we denote the distance in feature space $d_{f}(f(T(x)),f(x))$ as $d(T)$. Then Assumption~\ref{assum:assum2}  can be explained as  $T$ is positively correlated with $d(T)$. Due to the properties of monotonic function, the upper bound of $d(T)$ is $d(T_{max})$:
 \begin{equation}
    0 \leq d(T) \leq d(T_{max}) = d_{max},
    \label{max-dT}
\end{equation}
where $T_{max}$ denotes the most severe level of corruption $T$.
By limiting $d_{max}$ to $0$, we get:
\begin{equation}
    \lim_{d_{max} \rightarrow 0} {d(T)}= \lim_{d_{max} \rightarrow 0} {d_{f}(f(T(x)),f(x))}=0,
\label{limit}
\end{equation}
which means for all severity levels of corruption $T$, features of corrupted data $T(x)$ and clean data $x$ are the same when $d_{max} \rightarrow 0$. Thus robustness against a specific corruption is achieved.

Now the last issue is how to limit $d_{max}$ to 0. Note that:
\begin{equation}
    d_{max}=d(T_{max})=d_{f}(f(T_{max}(x)),f(x)).
    \label{dmax}
\end{equation}
Thus, by aligning features of the most severely corrupted samples $T_{max}(x)$ with original features $x$, we get $d_{max}\rightarrow0$. Proposition \ref{pro1} for TSCL is derived.

\subsubsection{Proposition 2 for TSCL-WC}
Considering Assumption~\ref{assum:assum1}, the shift in sample space increases as the increase of the severity level of a corruption $T$. Thus, the most severe corruption $T_{max}(x)$ is always achieved on the edge points of $\delta$ cycle. Then we can use $\{x_{t}^{(wc)}|\|x_{t}^{(wc)}-x_{t}\|=\delta\}$ to implicitly represent $T_{max}(x)$ due to the conclusion in Equation (\ref{construction_x_adv}).  By aligning features of these edge points with the original features via minimizing the contrastive loss defined in Equation (\ref{CL-AdvTL}), corruption robustness is achieved under TSCL-WC as :
\begin{equation}
    \lim_{\ell_{con}^{(wc)} \rightarrow 0} {d(T)}= \lim_{\ell_{con}^{(wc)} \rightarrow 0} {d_{f}(f(T(x)),f(x))}=0.
    \label{limit_xadv}
\end{equation}
Proposition \ref{pro2} for TSCL-WC is derived.

In practice, setting $\eta>2\delta$ in Algorithm \ref{algorithm-PGD} and \ref{algorithm-AdvTL} with only step $n=2$ gains enough good performance.
% In practice, results shows that 
% \textcolor{red}{Based on Assumption 2, we conclude the result that } 
% In practice, we \textcolor{red}{are surprised to} find that only aligning the edge points $\{x_{t}^{(wc)}|\|x_{t}^{(wc)}-x_{t}\|=\delta\}$ in TSCL-WC gets best performance, which is realized by setting $\eta > 2\delta$ in \textcolor{red}{Algorithm}. Intuitively, the setting with $\eta \ll \delta$ seems like a more reasonable setting but gets poorer performance on large shift transformations like contrast. 

%-----------------------------------------------------------------------------------------
\subsection{Metrics for corruption robustness}
The commonly used standardized aggregate performance measure is the Corruption Error (CE) \cite{hendrycks2019benchmarking}, which can be computed by:
\begin{equation}
    \mathrm{CE}_{T}^{f}=\left(\sum_{t=1}^{5} E_{t, T}^{f}\right) \bigg/\left(\sum_{t=1}^{5} E_{t, T}^{ AlexNet}\right),
    \label{CE}
\end{equation}
where $E_{t, T}^{f}$ denotes the error rate of model $f$  on target domain data transformed by corruption $T$ with severity $t$. The $AlexNet$ is trained on clean source domain and tested on corrupted target domain.

The corruption robustness of model $f$ is summarized by averaging Corruption Error values of 15 corruptions introduced in Section~\ref{sec:definition_robustness}: 
$\mathrm{CE}_{\text{Gaussian Noise}}^{f}, \dots , \mathrm{CE}_{\text{Glass Blur}}^{f}$. The results in the mean CE or mCE~\cite{hendrycks2019benchmarking} for short. mCE is calculated by only one setting (\eg, the Ar:Rw setting in Office-Home). For average performance of corruption robustness on the whole dataset (\eg, Office-Home), we need to average mCE values of all settings. 







==> CRDA (TOMM)/latex/sections/Methodology_v5.tex <==
% 1. Domain Discrepancy Generator

% 2. Overall learning framework
% 补充一个公式：l_ori包括分类损失和迁移损失。
% 3. Further explanation

% 4. Metrics
% 要突出我们自己发布了生成函数（类似Benchmark），并附图


\section{Methodology}
% In this paper, our attempts are made through two key problems of CRDA: 1) trade-off between domain invariance and corruption robustness; 2) generalization to unseen corruptions via domain information. we first propose a simple but effective teacher-student scheme (TSCL) for the first problem. As for the second problem, we further construct worst-corruption samples to mimic unseen corruptions via inversely enlarging domain discrepancy. Putting them together, we derive \textbf{TSCL-WC} as illustrated in Figure \ref{fig:AdvTL}. In addition, we theoretically show that only considering the most severe level of corruptions is  enough for our frameworks to handle all levels of severity.

%----------------------------------------------------------------------------------------------------------
\subsection{Domain Discrepancy Generator}
\label{sec:wc}


In CRDA setting, the key challenge is that testing corruptions are unavailable during training. Besides, previous data augmentation only encourages networks to memorize the specific corruptions seen during training and leaves models unable to generalize to new corruptions~\cite{geirhos2018generalisation,vasiljevic2016examining}. In this section, we attempt to utilize domain information given by domain adaptation to solve this challenge.
Thus, Domain Discrepancy Generator (DDG) is proposed to generate samples that most enlarge domain discrepancy to mimic unpredictable corruptions. Fig.~\ref{fig:AdvTL} illustrated the overall mechanism of DDG. The following is reasonable derivation.
\input{latex/imgs/StructureOfAdvTLe}

We first assume that corrupted target domain samples hold larger domain discrepancy to source domain than corresponding original target domain samples, which is empirically proved in the supplementary material. 
Thus, our core idea is to find the points near the original images in sample space that most increase domain discrepancy to represent the most severe corruptions. 
In domain adaptation, the domain discrepancy is always measured by transfer loss, which is commonly realized by Maximum Mean Discrepancy (MMD)~\cite{borgwardt2006integrating,Li20DCAN,long2015DAN,pan2010TCA} or adversarial methods \cite{ganin2016DANN,long2018conditional}. 

The followings are three basic assumptions for our method, where distance $d_{*}(t(x),x)$ denotes distance between the corrupted images and corresponding original images:
\begin{assumption}
\label{assum:assum1}
The corrupted versions are within the $\delta$-range neighborhood of the original image in sample space ($\boldsymbol{\delta}$ \textbf{neighborhood} for precise) and distance in sample space $d_{s}(t(x),x)$ becomes larger with increase of the severity level of corruption $t$.
\end{assumption}
\begin{assumption}
\label{assum:assum2}
Within the $\delta$ neighborhood, the severity level $t$ of a corruption  $T$ is positively correlated to distance in feature space  $d_{f}(f(t(x)) ,f(x))$.
\end{assumption}
\begin{assumption}
\label{assum:assum3}
Within the $\delta$ neighborhood, the severity level $t$ of a corruption $T$ is positively correlated to the value of transfer loss $\ell_{trans}(t(x))$.
\end{assumption}

The empirical proof can be seen in supplementary material. Assumption~\ref{assum:assum2}  is drawn from an interesting finding in Section~\ref{sec:empirical} that networks always learn order-invariant representations for different severity levels of corruptions.

Based on the above assumptions, we can construct the bridge between domain discrepancy and unpredictable corruptions. Given an input target domain data $x_{t}$, source domain $D_{s}$, transfer loss $\ell_{trans}$ and a corruption set $T$ ($t \in T$) whose corresponding corrupted data $t(x_{t})$ is within the $\delta$ neighborhood of $x_{t}$, DDG generates
\begin{equation}
    \begin{split}
    x_{t}^{(DDG)}&=\mathop{\arg\max}_{\left\|x_{t}^{(DDG)}-x_{t}\right\| \leq \delta} \ell_{trans}\left(f(x_{t}^{(DDG)}), f(D_{s})\right)
    \\&\Rightarrow \mathop{\arg\max}_{t \in T} \ell_{trans}\left(f(t\left(x_{t})\right), f(D_{s})\right)=t_{\max }(x_{t}),
    \end{split}
    \label{construction_x_adv}
\end{equation}
which means the point $x_{t}^{(DDG)}$ near the original target domain sample in sample space that most increases transfer loss (denoting domain discrepancy) can represent the most severe corruption. The proof of Equation (\ref{construction_x_adv}) can be seen in the supplementary material.
In practice, Domain Discrepancy Generator generates such samples via Project Gradient Descent (PGD)~\cite{madry2017PGD} in Algorithm \ref{algorithm-PGD}.
\input{latex/algorithm/algorithm-PGD}

It is worthy noting that the generated samples look similar to adversarial samples~\cite{madry2017PGD}. However, there exists few evidence that domain discrepancy could help corruption robustness in cross domain scenarios like domain adaptation ever before. We first show that it significantly improves corruption robustness on the basis of the bridge between corruptions and domain discrepancy constructed by Equation (\ref{construction_x_adv}). Meanwhile, DDG works in an unsupervised way while common adversarial training always needs ground-truth labels.

\subsection{Overall Learning Framework} 
The last question is how to learn robustness in unlabeled target domains. Since there is no strong constraints like classification loss in target domains, simply merging samples generated by DDG with the original data may lose the effectiveness. Thus, we utilize contrastive loss~\cite{chen2020simple} to enhance the constraints on target domains. The core idea is simple, \ie, minimizing the feature distance between corrupted samples with their original versions. Besides, to tackle with the unstable features in the early training stage, we further propose a warm-up scheme like teacher-student framework. The teacher model is first trained to extract the original features, while the student model then extracts corrupted features to minimize the distance to corresponding original features. Algorithm~\ref{algorithm-DDG} shows the overall process of DDG. The proposed contrastive loss is introduced as followed.

% \input{latex/algorithm/algorithm-TSCL_v2}
\input{latex/algorithm/algorithm-DDG}

Given a batch of samples ${\{x_i\}}_1^N$, we use feature extractor $f^{(tea)}$ and $f^{(stu)}$ introduced in Algorithm \ref{algorithm-DDG} to get $2N$ representation feature vectors:
\begin{equation}
    \begin{split}
        Z^{(tea)}={\left\{z_{i}^{(tea)}|z_{i}^{(tea)}=f^{(tea)}(x_i)\right\}}_1^N,\\
        Z^{(stu)}={\left\{z_{i}^{(stu)}|z_{i}^{(stu)}=f^{(stu)}(x_i)\right\}}_1^N,
    \end{split}
\end{equation}
% $Z^{(tea)}={\{z_{i}^{(tea)}|z_{i}^{(tea)}=f^{(tea)}(x_i)\}}_1^N$ and $Z^{(stu)}={\{z_{i}^{(stu)}|z_{i}^{(stu)}=f^{stu}(x_i)\}}_1^N$. 
where we define $Z=Z^{(tea)}\cup Z^{(stu)}={\{z_i\}}_1^{2N}$. The similarity loss of each two features can be calculated by:
%
\begin{equation}
    \ell_{sim}\left(z_{i}, z_{j}\right)=-\log \frac{\exp \left(sim\left(z_{i}, z_{j}\right) / \tau\right)}{\sum_{z_{k} \in Z, z_{k} \neq z_{i}} \exp \left(sim\left(z_{i}, z_{k}\right) / \tau\right)},
    \label{similarity}
\end{equation}
%
where $\tau=0.2$ is a temperature controller to control the similarity extent, and $sim\left(z_i,z_j\right)={z_i}^T z_j/z_i z_j$ is cosine distance between two vectors. 
% which is $sim\left(z_i,z_j\right)={z_i}^T z_j/z_i z_j$. 
Note that Equation (\ref{similarity}) is asymmetric between $z_i, z_j$. The final contrastive loss is defined by:
%
\begin{equation}
    \begin{split}
    \ell_{con}\left(Z^{(stu)}, Z^{(tea)}\right)
    = \frac{1}{2 N} \sum_{i=1}^{N} \left[\ell_{sim}\left(z_{i}^{(stu)}, z_{i}^{(tea)}\right)+ \ell_{sim}\left(z_{i}^{(tea)}, z_{i}^{(stu)}\right)\right],
    \end{split}
    \label{CL}
\end{equation}
%
where the goal is to minimize the distance between feature representations $z_{i}^{(stu)}$ and $z_{i}^{(tea)}$ of a same sample $x_i$. The other kinds of losses defined by the original DA models $\ell_{ori}$, usually containing source domain classification loss $\ell_{cls}$ and transfer loss $\ell_{trans}$in Equation (\ref{ori_loss}),  also need to be calculated:
%
\begin{equation}
\label{ori_loss}
    \ell_{ori}(x_{s},x_{t},y_{s})=\ell_{cls}(x_{s},y_{s})+\ell_{trans}(x_{s},x_{t}).
\end{equation}

In fact, contrastive loss does not make $Z^{(stu)}$ definitely same as $Z^{(tea)}$. And thanks to corruptions, the final feature representation $Z^{(stu)}$ has a further distillation on the basis of the teacher model, which may lead to not only improvement on robustness but also better performance on domain invariance.

By utilizing the contrastive loss in Equation (\ref{CL}), we can minimize feature distance between samples $x_{t}^{(DDG)}$ generated by DDG and original samples $x_{t}$ in the target domain iteratively, which leads to features of the most severely corrupted images come closer to original ones, as:
\begin{equation}
    \min d_{f}\left(f(x_{t}^{(DDG)}), f(x_{t})\right) \Rightarrow \min d_{f}\left(f(t_{max}(x_{t})), f(x_{t})\right).
    \label{illustration1}
\end{equation}
%
In practice, Equation (\ref{illustration1}) is realized by minimizing:
%
\begin{equation}
    \ell_{con}^{(DDG)}\left(x_{t}^{(DDG)},x_{t}\right)=\ell_{con}\left(f^{(stu)}(x_{t}^{(DDG)}),f^{(tea)}(x_{t})\right)
    \label{CL-AdvTL},
\end{equation}
Together with the loss defined by the original DA model $\ell_{ori}$ illustrated in Equation (\ref{ori_loss}) and Fig.~\ref{fig:AdvTL}, the final total loss is:
\begin{equation}
    \ell_{total}=\ell_{ori}(x_{s},x_{t},y_{s})+\lambda \ell_{con}^{(DDG)}(x_{t}^{(DDG)},x_{t}).
    \label{total_loss}
\end{equation}

Note that DDG only generated samples on target domains and the generated samples are only processed by contrastive loss.

%-----------------------------------------------------------------------------------------
\subsection{Further Explanation}
\label{sec:theory}
Intuitively, DDG should loop many times like $n=10$ in PGD to generates an augmented sample, which is time-consuming. In this section, we theoretically show that we only need to consider the edge point so that by setting $n=2$ is enough, which effectively reduces the time consumption. We begin with the following proposition.


\begin{theorem}
Only aligning the edge points $\{x_{t}^{(DDG)}|\|x_{t}^{(DDG)}-x_{t}\|=\delta\}$ around the $\delta$ neighborhood in Equation (\ref{construction_x_adv}) is enough to gain corruption robustness under the DDG framework.
\label{pro2}
\end{theorem}
 
Given input data $x$, a feature extractor $f$ and a corruption $T$ with continuous severity, we denote the distance in feature space $d_{f}(f(T(x)),f(x))$ as $d(T)$. Then Assumption~\ref{assum:assum2}  can be explained as  $T$ is positively correlated with $d(T)$. Due to the properties of monotonic function, the upper bound of $d(T)$ is $d(T_{max})$:
 \begin{equation}
    0 \leq d(T) \leq d(T_{max}) = d_{max},
    \label{max-dT}
\end{equation}
where $T_{max}$ denotes the most severe level of corruption $T$.
By limiting $d_{max}$ to $0$, we get:
\begin{equation}
    \lim_{d_{max} \rightarrow 0} {d(T)}= \lim_{d_{max} \rightarrow 0} {d_{f}(f(T(x)),f(x))}=0,
\label{limit}
\end{equation}
which means for all severity levels of corruption $T$, features of corrupted data $T(x)$ and clean data $x$ are the same when $d_{max} \rightarrow 0$. Thus, robustness against a specific corruption is achieved.

Now the last issue is how to limit $d_{max}$ to 0. Note that:
\begin{equation}
    d_{max}=d(T_{max})=d_{f}(f(T_{max}(x)),f(x)).
    \label{dmax}
\end{equation}
Thus, by aligning features of the most severely corrupted samples $T_{max}(x)$ with original features $x$, we get $d_{max}\rightarrow0$. 

Considering Assumption~\ref{assum:assum1}, the shift in sample space increases as the increase of the severity level of a corruption $T$. Thus, the most severe corruption $T_{max}(x)$ is always achieved on the edge points of $\delta$ cycle. Then we can use $\{x_{t}^{(DDG)}|\|x_{t}^{(DDG)}-x_{t}\|=\delta\}$ to implicitly represent $T_{max}(x)$ due to the conclusion in Equation (\ref{construction_x_adv}).  By aligning features of these edge points with the original features via minimizing the contrastive loss defined in Equation (\ref{CL-AdvTL}), corruption robustness is achieved under DDG as :
\begin{equation}
    \lim_{\ell_{con}^{(DDG)} \rightarrow 0} {d(T)}= \lim_{\ell_{con}^{(DDG)} \rightarrow 0} {d_{f}(f(T(x)),f(x))}=0.
    \label{limit_xadv}
\end{equation}
Proposition \ref{pro2} is derived.

Thus, by setting stride $\eta$ bigger than range $2\delta$, we can reach the edge point in one step. In practice, only step $n=2$ gains enough good performance.
% In practice, results shows that 
% \textcolor{red}{Based on Assumption 2, we conclude the result that } 
% In practice, we \textcolor{red}{are surprised to} find that only aligning the edge points $\{x_{t}^{(wc)}|\|x_{t}^{(wc)}-x_{t}\|=\delta\}$ in TSCL-WC gets best performance, which is realized by setting $\eta > 2\delta$ in \textcolor{red}{Algorithm}. Intuitively, the setting with $\eta \ll \delta$ seems like a more reasonable setting but gets poorer performance on large shift transformations like contrast. 

%-----------------------------------------------------------------------------------------
\subsection{Metrics for corruption robustness}
The commonly used standardized aggregate performance measure is the Corruption Error (CE) \cite{hendrycks2019benchmarking}, which can be computed by:
\begin{equation}
    \mathrm{CE}_{T}^{f}=\left(\sum_{t=1}^{5} E_{t, T}^{f}\right) \bigg/\left(\sum_{t=1}^{5} E_{t, T}^{ AlexNet}\right),
    \label{CE}
\end{equation}
where $E_{t, T}^{f}$ denotes the error rate of model $f$  on target domain data transformed by corruption $T$ with severity $t$. The $AlexNet$ is trained on clean source domain and tested on corrupted target domain.

The corruption robustness of model $f$ is summarized by averaging Corruption Error values of 15 corruptions introduced in Section~\ref{sec:definition_robustness}: 
$\mathrm{CE}_{\text{Gaussian Noise}}^{f}, \dots , \mathrm{CE}_{\text{Glass Blur}}^{f}$. The results in the mean CE or mCE~\cite{hendrycks2019benchmarking} for short. mCE is calculated by only one setting (\eg, the Ar:Rw setting in Office-Home). For average performance of corruption robustness on the whole dataset (\eg, Office-Home), we need to average mCE values of all settings. 







==> CRDA (TOMM)/latex/sections/Outline.tex <==
Abstract
    1. DA 目前的发展（套话）
    
    2. 更真实且通用的场景——Corruption Robust Domain Adaptation (CRDA): 定义
    
    3. 目前方法直接组合在CRDA上效果不好
    
    4. 我们的思考：CRDA问题可以分解为两个子问题：
        (1) Domain-invariance 和 Corruption 之间的协调 <-- 以往方法组合不好的原因
        
        (2) 如何考虑unseen corruption的问题 
        
    5. 由此，我们提出了 xxxxx 的方法：
        (1) 针对问题(1), 我们先不考虑unseen corruption的问题，假设可以得到测试corruption，基于已有DA模型框架，提出TSCL --> 一个基础框架
        
        (2) 针对问题(2), 我们采用基于inverting domain discrepency的方式构造worst-corruption sample 来隐式地表示unseen corruption; 并且将TSCL中的随机数据增广替换成worst-corruption sample。
        
    6. 实验上看，我们的方法优于现有解决方案
    
    7. 有趣的一点是：我们理论证明了只需要考虑最严重的severity就可以handle所有level severity，提升了方法效果和效率。
    
Introduction
    DA现状，Robustness现状-->这两个方向seperately 考虑问题，那么就引出思考：
         How to achieve both domain invariance and corruptionrobustness in a more generalized way?
         
    提出Corruption Robust Domain Adaptation (CRDA)，进一步描述。 用Figure1说明目前方法不行-->原因是他们或多或少fail in two-fold chanllenges in CRDA:
        1) Domain-invariance 和 Corruption 之间的协调
            
        2) General robustness to unseen corruptions via domain information.
    在对CRDA的考虑上，我们分解成了两个子问题：
        ( <-- 以往方法组合不好的原因
        
        ( 
        
    基于这两个问题，我们提出了 xxxxx 的方法:
        首先单独考虑问题(1)，那么我们可以假设corruption是可知的，提出TSCL，指出先考虑Domain-Invariance，再考虑Corruption Robustness，而不是同时一起考虑。
        
        再考虑问题(2), 我们采用inverting domain discrepency的方式构造worst-corruption sample 来隐式地表示unseen corruption
        
        结合两个问题的解决方法，我们将TSCL中对样本基于已知corruption做增广替换成造worst-corruption sample，完成了我们的方法
        
    除此之外，我们还理论上说明了只考虑最严重的severity就足够了
    
    简单描述实验结论，总结。
        
Methodology
    简述：我们对CRDA的考虑：
    (1) Domain-invariance 和 Corruption 之间的协调 --> TSCL
    (2) 如何考虑unseen corruption的问题 --> Augmentation via inverting domain discripancy
        
    1. TSCL
    
    2. Augmentation via inverting domain discripancy
    
    3. Overall Framework
    
    4. Theoretical Explanation

Experiments
    1. 验证TSCL框架的有效性
        与直接同时考虑 Data Augmentation 和 DA的想法对比，说明分阶段考虑更优
        
    2. 我们的方法再CRDA这个setting下的效果
        Office-Home、Office
        
    3. Ablation
        (没办法把TSCL和Augmentation via inverting domain discripancy拆开，因为这两个合起来才能再CRDA下进行，分开setting都不适用)
        保持现有的不变
        
    4. Order-invariant representations of corruptions
        说只考虑最严重的severity就足够这件事情的实验依据


遗留问题：
    我们的方法 (原来的TSCL-Adv) 起个什么名字好？

==> CRDA (TOMM)/latex/sections/Outline_v2.tex <==
Abstract
1. (目前DA在理想情况下做的已经不错了，可以研究更实际的情况了）
2. 一个实际的系统要求同时Domain-invariant and Corruption Robustness
3. 我们提出了一个更实际的task，CRDA：进一步描述
4. 以往方法在这个task下不好，原因是下面两个挑战
5. 两个挑战：(1) DI和CR之间的trade-off 或balance；(2) 利用DA的特性来进一步优化对unseen corruption的鲁棒性
6. 我们的方法
7. 实验结果

Introduction
1. 目前研究现状, 引出问题：我们需要同时考虑DI和CR了
2. 提出一个新的task CRDA：描述
3. 以往方法不好-->两个挑战: ：(1) DI和CR之间的trade-off 或balance；(2) 利用DA的特性来进一步优化对unseen corruption的鲁棒性
4. 基于两个挑战，分别提出我们的方法：
    挑战(1) --> TSCL
    挑战(2) --> construct worst-corruption samples via inverting domain discrepancy
5. 总结
    
Methodology
1. TSCL
    分析挑战(1) --> 以往方法不好的原因之一是同时训练时会冲突 --> 在这样的情况下很难handle trade-off。
    抛弃同时训练，我们一步一步来 --> TSCL

2. worst-corruption samples via inverting domain discrepancy
    TSCL的问题：只能用data augmentation 处理已知的corruption。 + 通常Data Augmentation不适用于unseen corruption. 
    --> 利用DA特有的domain信息来构造可以模拟unseen corruption的样本。
    
    --> Adv

3. TSCL-inverse
    总体描述 + 只要handle最严重的corruption就可以了

4. Theoretical Explanation

5. Metrics
    
Experiments

% 实验上需要也展示 clean target domain 上的分类性能.

==> CRDA (TOMM)/latex/sections/Preliminaries_v2.tex <==
\section{Preliminaries}

%------------------------------------------------------------------------
\subsection{Problem definition for CRDA}
In this paper, we investigate CRDA in the scope  of unsupervised domain adaptation for classification. Given labeled source domain $\mathcal{D}_s = {\{\left(\mathcal{X}_{s},\mathcal{Y}_{s}\right)\}}$, unlabeled target domain $\mathcal{D}_t = {\{\mathcal{X}_{t}\}}$ ($\mathcal{Y}_{t}$ is unavailable while training), models are required to be robust on corrupted target domain samples $T(\mathcal{X}_{t})$ while maintaining the performance on original target domain, where $T$ denotes a corruption set \textbf{unavailable for training}. Note that $\mathcal{Y}_{s}=\mathcal{Y}_{t}=\{1,\ldots,S\}$ and $P\left(\mathcal{D}_s\right)\neq P\left(\mathcal{D}_t\right)$.

% \input{latex/tabs/frequent_notations}
%------------------------------------------------------------------------
\subsection{Definition of corruption robustness}
\label{sec:definition_robustness}
The concept of corruption robustness is drawn from \cite{hendrycks2019benchmarking} with slight modification. Given an input sample set $\mathcal{X}$ with the corresponding label set $\mathcal{Y}$, a corruption set $T$ and a model $m=f \circ c$, where $f$ and $c$ respectively denote a feature extractor and a classifier, the corruption robustness is measured by:
\begin{equation}
\mathbb{E}_{t \sim T}\left[\mathbb{P}_{(x, y) \sim (\mathcal{X},\mathcal{Y})}(m(t(x))=y)\right],
% \forall (x,y) \in (X,Y), t \in T: m(t(x))=m(x)=y
\label{ideal_transforamtion_definition}
\end{equation}
% In practice, if \textcolor{red}{identity transformation} lies in corruption set $T$, Equation (\ref{ideal_transforamtion_definition}) is always achieved by:
% \begin{equation}
% \min _{\theta} E_{t \in T}\left[E_{(x,y) \in (X,Y)} \ell(t(x),y, \theta)\right]
% \end{equation}
% where $\ell$ denotes an \textcolor{red}{effective} loss function.
%
%In this paper, we derive Equation (\ref{ideal_transforamtion_definition}) by aligning features:
% In this paper, we derive the robustness defined in Equation (\ref{ideal_transforamtion_definition}) by aligning features, which is shown in Equation (\ref{ideal_transforamtion_definition}).
where we can derive the robustness by aligning features as:
\begin{equation}
\max \left\{\mathbb{E}_{t \sim T}\left[\mathbb{P}_{x \sim \mathcal{X}}(f(t(x))=f(x))\right]\right\}.
% \forall x \in X, t \in T: f(t(x))=f(x)
\label{practice_transforamtion_definition}
\end{equation}
Here $T$ denotes corruptions derived from \cite{hendrycks2019benchmarking}, which contains 15 kinds of corruptions for $T$ and 5 severities $t$ for each kind (see Fig.~\ref{fig:15corruption1}).
% The total  15 kinds of corruptions include: Gaussian Noise, Shot Noise, Impulse Noise, Defocus Blur, Motion Blur, Zoom Blur, Fog, Frost, Snow, Elastic Transform, Contrast, Brightness, JPEG Compression, Pixelate and Glass Blur.
% Some corruption examples are shown in Figure \ref{fig:illustration}, details of all kinds of corruptions and severities are shown in SM.
\input{latex/imgs/15corruptions}
% Consider Spatial Transformation Later


==> CRDA (TOMM)/latex/sections/Related_Work.tex <==
\section{Related Work}
\input{latex/tabs/differentDAsettings}

\paragraph{Unsupervised Domain Adaptation.} 
% conclude mainstreams
% discuss and point out the differences of our paper
Tremendous DA methods have made progress in cross-domain applications like recognition~\cite{gopalan2011domain}, object detection~\cite{chen2018domain}, and semantic segmentation~\cite{tsai2018learning}. The core idea is to seek domain-invariant features among source and target domains~\cite{pan2009survey}. A mainstream methodology is distribution alignment, which is mainly based on Maximum Mean Discrepancy (MMD)~\cite{borgwardt2006integrating,chen2019joint,Li20DCAN,long2015DAN,pan2010TCA} or adversarial methods~\cite{ganin2016DANN,goodfellow2014GAN,long2018conditional,zhang2018collaborative,zhang2019domain}. Besides, some works further make improvement by pseudo-labeling~\cite{saito2017asymmetric}, co-training~\cite{zhang2018collaborative}, entropy regularization~\cite{shu2018dirt}, and evolutionary-based architecture design~\cite{sheng2021evolving}.
Recently, increasing researchers focus on more realistic scenarios: considering user privacy, \cite{li2020model,liang2020shot} investigate the scenario where only source domain models instead of data available while training. Label corruptions in source domain~\cite{han2020towards} is proposed to address the low quality labeling problem in DA. Besides, domain generalization~\cite{huang2020self,dg_mmld,volpi2018generalizing} aims to learn domain-invariant representations for unseen target domains.
Different from existing literature (see Table \ref{tab:DifferentDA}), we propose a new and realistic topic: corruption-agnostic robust domain adaptation, which investigates corruption robustness in domain adaptation.

% \vspace{-3mm}
\paragraph{Corruption Robustness.}
% conclude mainstreams
% \input{latex/tabs/differentDAsettings}
% discuss and point out the differences of our paper
Convolutional networks are proved fragile to simple corruptions by several studies~\cite{dodge2017study,hosseini2017google}. Assuming corruptions are known beforehand, Quality Resilient DNN~\cite{dodge2017quality} learns robustness against specific corruptions via a mixture of corruption-specific experts. 
% Zheng \textcolor{red}{et.al} aligns prediction of noisy images and clean ones to tackle underfitting on noise corruptions. 
Instead of knowing testing corruptions beforehand, we propose CRDA to learn general robustness against unseen corruptions. In recent years, increasing works begin to focus on robustness against unseen corruptions. \cite{vasiljevic2016examining} shows that fine-tuning on blurred images fails to generalize to unseen blurs. Several benchmarks~\cite{hendrycks2020many,hendrycks2019benchmarking,hendrycks2019nae,kang2019testing} are constructed to measure generalization to unseen corruptions. Self-supervised learning is found beneficial to corruption robustness~\cite{chen2020adversarial,hendrycks2019using}. CutMix~\cite{yun2019cutmix}, Mixup~\cite{zhang2017mixup}, Patch Gaussian~\cite{lopes2019improving}, Randaugment~\cite{cubuk2020randaugment} and AugMix~\cite{hendrycks2019augmix} are under the mainstream that aggregates several general transformations to implicitly represent unseen corruptions. However, current benchmarks and mainstream methods all take it for granted that training and testing data are from the same domain distribution, while CRDA also requires consideration of domain shift, as illustrated in Table \ref{tab:DifferentDA}. Furthermore, instead of aggregating transformations, we propose a new idea that utilize domain discrepancy information to mimic unseen corruptions.

% \paragraph{Adversarial Training}
% conclude mainstreams

% discuss and point out the differences of our paper

==> CRDA (TOMM)/latex/sections/Supplementary_Outline.tex <==
Supplementary Material 内容
1.	15 种corruptions 的图示和描述 y
2.	3个Assumption的可靠性说明 y
3.	公式（6）的推导 y
4.	完整的TSCL结果 y
5.	AugMix的Implement Detail  x
6.	Lower bound 的具体求法，实现细节 x
8.	5.4节Order-invariant representations of corruptions的训练细节 y
9.	Training Loss的曲线 x
10.	Ablation：
    a)	超参数的影响 y
11.	解释性实验
    a)	展示并分析worst-corruption sample的图像 y
    b)	之前方法简单结合没处理好trade-off的量化指标证明
12.	为什么要选AugMix作为baseline对比 x
13. 之前基于特征的AdvTL-feature的尝试：结果及原因分析 x
14. 对于一些没有直接定义Transfer Loss 的DA x 模型，一种替代方法：训练一个鉴别器来生成Transfer Loss
    a)  出发点
    b)  方法描述
    b)  结果展示
15. AlexNet 的error rate结果 (计算mCE时用的) x
16. 其他DA模型的鲁棒性测试，说明DCAN鲁棒性相对好只是个例 x
17. 说明表3中的CLean的结果是所有鲁棒性的实验取的平均值 y


==> CRDA (TOMM)/latex/sections/Todo_list.tex <==
Theoretical Explanation 是否严谨？是否必要？待商榷。
想想有没有更好的名字代替TSCL-Inverse
在实验中加原始精度比较
Introduction 部分是否要去掉combination，再考虑一下
想办法把Abstract里的Teacher-Student scheme (TSCL) 补全成 Teacher-Student scheme via Contrastive Loss (TSCL)。但是补全就会跨列
是否要把图1放在第一页？放在第二页会和表格冲突

==> CRDA (TOMM)/latex/tabs/Rebuttle_TTT.tex <==
\begin{table}[h]
    \centering
    \caption{Accuracy ($\%$) of TTT under Ar$\to$Cl}
    \label{tab:acc_TTT}
    \setlength{\tabcolsep}{1.2mm}{
    \small{
    \begin{tabular}{c|c|c}
        \toprule
        \multirow{2}{*}{TTT} & \multicolumn{2}{c}{CDAN+TN}\\
        \cline{2-3}
         & - & TSCL-WC\\
        \hline
        33.4 & 54.1 & 57.1\\
        \bottomrule
    \end{tabular}
    }
    }
    \vspace{-1.5mm}
\end{table}

==> CRDA (TOMM)/latex/tabs/Rebuttle_clean2corrupted.tex <==
\begin{table}[h]
\linespread{1}
    \centering
    \vspace{-3mm}
    \caption{Accuracy ($\%$) on different corruption level of gaussian noise under Ar$\to$Cl.}
    \vspace{-3mm}
    \label{tab:clean2corrupted}
    \small{
    \setlength{\tabcolsep}{1.0mm}{
    \begin{tabular}{l|cccccc|c}
        
        \toprule
        Method & clean & 1 & 2 & 3 & 4 & 5 & Avg ($\uparrow$)\\
        \hline
        CDAN+TN & 54.1 & 49.2 & 45.9 & 41.3 & 34.4 & 25.9 & 41.8\\ 
        Yours & 53.6  & 51.3  & 50.5  & 49.9 & 48.0 & 44.5 & 49.6\\
        TSCL-WC & 57.1 & 55.5 & 54.5 & 52.0 & 48.4 & 39.8 & 51.2\\
        \bottomrule
    \end{tabular}
    }
    }
    \vspace{-4mm}
\end{table}



==> CRDA (TOMM)/latex/tabs/acc_rawOffice.tex <==
\begin{table}
    \centering
    \caption{Accuracy ($\%$) on clean Office-31 data (ResNet-50).}
    \label{tab:acc_Office}
    \setlength{\tabcolsep}{1.15mm}{
    \small{
    \begin{tabular}{c|ccc|ccc}
        \toprule
        \multirow{2}{*}{Settings} & \multicolumn{3}{c|}{CDAN+TN} &\multicolumn{3}{c}{DCAN} \\
        \cline{2-7}
         & - & AugMix & Ours & - & AugMix & Ours\\
        \hline
        A$\to$D & 92.2 & 85.9 & 92.2 & 93.4 & 92.8 & 90.8\\
        A$\to$W & 93.2 & 75.6 & 93.3 & 94.3 & 94.3 & 95.0\\
        D$\to$A & 74.7 & 64.6 & 73.9 & 76.6 & 74.3 & 76.2\\
        D$\to$W & 98.5 & 98.9 & 98.6 & 97.0 & 97.6 & 96.7\\
        W$\to$A & 74.6 & 62.0 & 75.2 & 72.4 & 71.9 & 72.9\\
        W$\to$D & 100.0 & 100.0 & 100.0 & 99.6 & 99.8 & 100.0\\
        \hline
        Avg ($\downarrow$) & 88.9 & 81.2 & 88.9 & 88.9 & 88.5 & 88.6\\
        \bottomrule
    \end{tabular}
    }
    }
    \vspace{-3mm}
\end{table}

==> CRDA (TOMM)/latex/tabs/acc_rawOfficeHome.tex <==
% \begin{table*}
%     \centering
%     \caption{Accuracy ($\%$) on clean Office-Home data.}
%     \label{tab:acc_OfficeHome}
%     \small{
%     \setlength{\tabcolsep}{1.0mm}{
%     \begin{tabular}{l|cccccccccccc|c}
%         \toprule
%         Method & Ar$\to$Cl & Ar$\to$Pr & Ar$\to$Rw & Cl$\to$Ar & Cl$\to$Pr & Cl$\to$Rw & Pr$\to$Ar & Pr$\to$Cl & Pr$\to$Rw & Rw$\to$Ar & Rw$\to$Cl & Rw$\to$Pr & Avg \\
%         \hline
%         CDAN+TN &54.1 & 70.3 & 77.9 & 62.2 & 74.4 & 73.7 & 62.4 & 53.1 & 81.0 & 72.8 & 56.9 & 82.5 & 68.4\\
%         DCAN & 57.8 & 76.3 & 82.9 & 68.5 & 72.7 & 76.7 & 68.0 & 56.5 & 82.1 & 73.5 & 60.8 & 83.3 & 71.6\\
%         SHOT & 57.8 & 78.8 & 82.0 & 67.7 & 78.8 & 77.0 & 67.1 & 54.6 & 82.1 & 73.1 & 58.2 & 84.1 & 71.8\\
%         AdvTL & 57.1 & 74.4 & 79.4 & 63.5 & 75.9 & 75.3 & 63.2 & 54.9 & 81.9 & 73.1 & 58.8 & 84.2 & 70.1\\
%         DCAN+AdvTL & 58.1 & 75.2 & 82.9 & 68.7 & 75.0 & 77.6 & 68.1 & 56.6 & 81.8 & 73.9 & 60.6 & 83.1 & 71.8\\
%         TSCL & 55.6 & 71.0 & 79.2 & 63.3 & 75.5 & 75.2 & 62.6 & 54.1 & 81.6 & 73.1 & 57.8 & 83.3 & 69.3\\
%         DCAN+TSCL & 58.1 & 75.6 & 82.8 & 69.0 & 74.7 & 77.0 & 68.4 & 57.2 & 82.3 & 74.2 & 61.2 & 83.4 & 72.0\\
%         SHOT+TSCL & 58.0 & 79.0 & 82.4 & 68.2 & 79.9 & 78.4 & 67.1 & 55.0 & 81.7 & 73.4 & 58.1 & 84.5 & 72.1\\
%         \bottomrule
%     \end{tabular}
%     }
%     }
% \end{table*}
\begin{table*}
    \centering
    \caption{Accuracy ($\%$) on clean Office-Home data (ResNet-50).}
    \label{tab:acc_OfficeHome}
    \resizebox{140mm}{!}{%\small{
    \setlength{\tabcolsep}{0.8mm}{
    \begin{tabular}{l|cccccccccccc|c}
        \toprule
        Method & Ar$\to$Cl & Ar$\to$Pr & Ar$\to$Rw & Cl$\to$Ar & Cl$\to$Pr & Cl$\to$Rw & Pr$\to$Ar & Pr$\to$Cl & Pr$\to$Rw & Rw$\to$Ar & Rw$\to$Cl & Rw$\to$Pr & Avg ($\uparrow$) \\
        \hline
        ResNet & 34.9 & 50.0 & 58.0 & 37.4 & 41.9 & 46.2 & 38.5 & 31.2 & 60.4 & 53.9 & 41.2 & 59.9 & 46.1\\
        DAN & 43.6 & 57.0 & 67.9 & 45.8 & 56.5 & 60.4 & 44.0 & 43.6 & 67.7 & 63.1 & 51.5 & 74.3 & 56.3\\
        DANN & 45.6 & 59.3 & 70.1 & 47.0 & 58.5 & 60.9 & 46.1 & 43.7 & 68.5 & 63.2 & 51.8 & 76.8 & 57.6\\
        JAN & 45.9 & 61.2 & 68.9 & 50.4 & 59.7 & 61.0 & 45.8 & 43.4 & 70.3 & 63.9 & 52.4 & 76.8 & 58.3\\
        DWT & 50.3 & 72.1 & 77.0 & 59.6 & 69.3 & 70.2 & 58.3 & 48.1 & 77.3 & 69.3 & 53.6 & 82.0 & 65.6\\
        CDAN & 50.7 & 70.6 & 76.0 & 57.6 & 70.0 & 70.0 & 57.4 & 50.9 & 77.3 & 70.9 & 56.7 & 81.6 & 65.8\\
        TADA & 53.1 & 72.3 & 77.2 & 59.1 & 71.2 & 72.1 & 59.7 & 53.1 & 78.4 & 72.4 & 60.0 & 82.9 & 67.6\\
        SymNets & 47.7 & 72.9 & 78.5 & 64.2 & 71.3 & 74.2 & 64.2 & 48.8 & 79.5 & 74.5 & 52.6 & 82.7 & 67.6\\
        MDD & 54.9 & 73.7 & 77.8 & 60.0 & 71.4 & 71.8 & 61.2 & 53.6 & 78.1 & 72.5 & 60.2 & 82.3 & 68.1\\
        \hline
        CDAN+TN & 54.1 & 70.3 & 77.9 & 62.2 & 74.4 & 73.7 & 62.4 & 53.1 & 81.0 & 72.8 & 56.9 & 82.5 & 68.4\\
        +AugMix & 50.5 & 70.1 & 74.9 & 56.7 & 69.6 & 68.7 & 53.9 & 50.4 & 75.9 & 67.9 & 58.2 & 80.6 & 64.8\\
        % +TSCL & 55.6 & 71.0 & 79.2 & 63.3 & 75.5 & 75.2 & 62.6 & 54.1 & 81.6 & 73.1 & 57.8 & 83.3 & 69.3\\
        \textbf{+DDG} & 57.1 & 74.4 & 79.4 & 63.5 & 75.9 & 75.3 & 63.2 & 54.9 & 81.9 & 73.1 & 58.8 & 84.2 & \textbf{70.1}\\
        \hline
        DCAN & 57.8 & \textbf{76.3} & 82.9 & 68.5 & 72.7 & 76.7 & 68.0 & 56.5 & 82.1 & 73.5 & \textbf{60.8} & \textbf{83.3} & 71.6\\
        +AugMix & 55.8 & 74.8 & 82.5 & 67.6 & 72.1 & 76.1 & 67.5 & 55.0 & \textbf{82.5} & 73.4 & 59.0 & 82.5 & 70.7\\
        % +TSCL & 58.1 & 75.6 & 82.8 & 69.0 & 74.7 & 77.0 & 68.4 & 57.2 & 82.3 & 74.2 & 61.2 & 83.4 & 72.0\\
        \textbf{+DDG} & \textbf{58.1} & 75.2 & \textbf{82.9} & \textbf{68.7} & \textbf{75.0} & \textbf{77.6} & \textbf{68.1} & \textbf{56.6} & 81.8 & \textbf{73.9} & 60.6 & 83.1 & \textbf{71.8}\\
        % \hline
        % SHOT & 57.8 & 78.8 & 82.0 & 67.7 & 78.8 & 77.0 & 67.1 & 54.6 & 82.1 & 73.1 & 58.2 & 84.1 & 71.8\\
        % +TSCL & 58.0 & 79.0 & 82.4 & 68.2 & 79.9 & 78.4 & 67.1 & 55.0 & 81.7 & 73.4 & 58.1 & 84.5 & 72.1\\
        \bottomrule
    \end{tabular}
    }
    }
    \vspace{-1.5mm}
\end{table*}


==> CRDA (TOMM)/latex/tabs/differentDAsettings.tex <==
% \begin{table*}
%     \centering
%     \caption{Comparison of related research topics.}
%     \label{tab:DifferentDA}
%     \begin{tabular}{l|c|c|c}
%         \toprule
%         \textbf{Setting} & Domain Shift & Target Domain Available & Visual Corruption \\
%         \hline
%         Unsupervised Domain Adaptation & \checkmark & \checkmark &  \\
%         \hline
%         Domain Generalization & \checkmark &  &  \\
%         \hline
%         Corruption Robustness &  &  & \checkmark \\
%         \hline
%         Corruption Robust Domain Adaptation & \checkmark & \checkmark & \checkmark \\
%         \bottomrule
%     \end{tabular}
% \end{table*}

\begin{table*}
    \centering
    \caption{Comparison of related research topics.}
    \label{tab:DifferentDA}
    \resizebox{140mm}{!}{
    \begin{tabular}{l|c|c|c}
        \toprule
        \multicolumn{1}{c|}{\textbf{Setting}} & Domain Shift & Target Domain Available & Visual Corruption \\
        \hline
        Unsupervised Domain Adaptation~\cite{Li20DCAN,long2018conditional,pan2009survey} & \checkmark & \checkmark &  \\
        \hline
        Domain Generalization~\cite{huang2020self,dg_mmld,volpi2018generalizing} & \checkmark &  &  \\
        \hline
        Corruption Robustness~\cite{hendrycks2019benchmarking,hendrycks2019using,hendrycks2019augmix,shorten2019survey} &  &  & \checkmark \\
        \hline
        \textbf{Corruption-Agnostic Robust Domain Adaptation} & \checkmark & \checkmark & \checkmark \\
        \bottomrule
    \end{tabular}
    }
    \vspace{-3mm}
\end{table*}

==> CRDA (TOMM)/latex/tabs/err_TSCL_OfficeHome.tex <==
\begin{table}
    \centering
    \caption{Error rate ($\%$) under a specific known corruption on the Ar$\to$Rw setting of Office-Home dataset for teacher-student warm-up shceme.}
    \label{tab:err_TSCL_home}
    \setlength{\tabcolsep}{1.6mm}{
    \small{
    \begin{tabular}{c|ccc}
        \toprule
        \multirow{2}{*}{Corruption} & \multicolumn{3}{c}{CDAN+TN} \\
        \cline{2-4}
         & -  & DataAug & Ours \\
        \hline
        Clean & 22.1 & 24.6 & 21.2\\
        Gaussian Noise & 78.4 & 33.4 & 27.8\\
        Defocus Blur & 70.4 & 35.0 & 26.7\\
        Fog & 47.3 & 24.6 & 23.6\\
        Contrast & 66.4 & 24.6 & 23.0\\
        \bottomrule
    \end{tabular}
    }
    }
    \vspace{-1.5mm}
\end{table}

==> CRDA (TOMM)/latex/tabs/err_TSCL_OfficeHome_full.tex <==
\begin{table}
    \centering
    \caption{Error rate ($\%$) under a specific known corruption on the Ar$\to$Rw setting of Office-Home dataset for teacher-student warm-up shceme.}
    \label{tab:err_TSCL_home}
    \setlength{\tabcolsep}{1.6mm}{
    \small{
    \begin{tabular}{c|ccc|c|ccc}
        \toprule
        \multirow{2}{*}{Corruption} & \multicolumn{3}{c|}{CDAN+TN} &\multirow{2}{*}{Corruption} & \multicolumn{3}{c}{CDAN+TN} \\
        \cline{2-4}
        \cline{6-8}
         & -  & DataAug & Ours  & & - & DataAug & Ours\\
        \hline
        Clean & 22.1 & 24.6 & 21.2 & Frost & 55.7 & 30.6 & 25.5\\
        Gaussian Noise & 78.4 & 33.4 & 27.8 & Snow & 60.0 & 31.2 & 23.9\\
        Shot Noise & 78.3 & 34.9 & 26.9 & Elastic Transform & 84.2 & 30.0 & 23.3\\
        Impulse Noise & 83.4 & 33.4 & 24.4 & Contrast & 66.4 & 24.6 & 23.0\\
        Defocus Blur & 70.4 & 34.9 & 26.7 & Brightness & 29.7 & 26.5 & 23.6\\
        Motion Blur & 69.5 & 28.4 & 24.3 & JPEG Compression & 37.6 & 29.0 & 23.2\\
        Zoom Blur & 53.6 & 29.4 & 23.1 & Pixelate & 45.7 & 26.9 & 22.6\\
        Fog & 47.3 & 24.6 & 23.6 & Glass Blur & 86.4 & 37.0 & 27.8\\
        \bottomrule
    \end{tabular}
    }
    }
    \vspace{-1.5mm}
\end{table}

==> CRDA (TOMM)/latex/tabs/frequent_notations.tex <==
\begin{table}[t]
    \centering
    \caption{Notations and descriptions used in this paper}
    \label{tab:frequent_notation}
    \small{
    \setlength{\tabcolsep}{1.1mm}{
    \begin{tabular}{c|c}
        \toprule
        Notation&Description\\
        \hline
        $f$ & feature extractor \\
        % ($\Leftrightarrowf_{1}\circf_{2}$)
        % $f_{1}$ & feature extractor without the last layer\\
        % $f_{2}$ & the last layer of feature extractor\\
        $c$ & classifier\\
        $TL$ & transfer loss\\
        $x$ & input data\\
        % $f$ & interval feature ($\Leftrightarrowf_{1}(x)$)\\
        $z$ & final feature ($\Leftrightarrow f(x)$)\\
        $*^{(stu)}$ & * of the student model (\textcolor{red}{e.g.} $f^{(stu)}$)\\
        $*^{(tea)}$ & * of the teacher model\\
        $x_{t}^{(adv)}$ & worst-transformation-case sample\\
        \bottomrule
    \end{tabular}
    }
    }
\end{table}

==> CRDA (TOMM)/latex/tabs/mCE_Ablation-delta.tex <==
\begin{table}[t]
    \centering
    \caption{mCE ($\%$) on Ar$\to$Rw for different updata strides $\eta$ in DDG}
    \label{tab:Ablation-delta}
    \small{
    \setlength{\tabcolsep}{5mm}{
    \begin{tabular}{ccc|c}
        \toprule
        $\delta$&$\eta$&$n$&mCE ($\downarrow$)\\
        \hline
        $60/255$ & $> 2\delta$ & 2 & 48.0\\ 
        $60/255$ & $> 2\delta$ & 10 & 49.6\\ 
        $60/255$ & $15/255$ & 10 & 51.6\\ 
        $60/255$ & $6/255$ & 10 & 52.8\\ 
        \bottomrule
    \end{tabular}
    }
    }
    \vspace{-3mm}
\end{table}

==> CRDA (TOMM)/latex/tabs/mCE_Office.tex <==
% \begin{table}
%     \centering
%     \caption{mCE ($\%$) on all cross-domain settings of Office-31 dataset under CRDA.}
%     \label{tab:mCE_Office}
%     \setlength{\tabcolsep}{2.4mm}{
%     \small{
%     \begin{tabular}{c|ccc|c}
%         \toprule
%         \multirow{2}{*}{Settings} & \multicolumn{3}{c|}{CDAN+TN} & Lower \\
%         \cline{2-4}
%          & - & AugMix & Ours & Bould \\
%         \hline
%         A$\to$D & 60.3 & 46.0 & 48.9 & 12.3\\
%         A$\to$W & 59.6 & 65.2 & 46.9 & 10.1\\
%         D$\to$A & 64.1 & 66.0 & 62.4 & 33.8\\
%         D$\to$W & 83.5 & 59.9 & 69.7 & 4.6\\
%         W$\to$A & 64.7 & 67.9 & 60.1 & 36.4\\
%         W$\to$D & 120.2 & 64.3 & 70.9 & 0.7\\
%         \hline
%         Avg ($\downarrow$) & 75.4 & 61.6 & \textbf{59.8} & 16.3\\
%         \bottomrule
%     \end{tabular}
%     }
%     }
% \end{table}
\begin{table}
    \centering
    \caption{mCE ($\%$) on all cross-domain settings of Office-31 dataset under CRDA (ResNet-50).}
    \label{tab:mCE_Office}
    \setlength{\tabcolsep}{1.15mm}{
    \small{
    \begin{tabular}{c|ccc|ccc|c}
        \toprule
        \multirow{2}{*}{Settings} & \multicolumn{3}{c|}{CDAN+TN} &\multicolumn{3}{c|}{DCAN} & Lower \\
        \cline{2-7}
         & - & AugMix & Ours & - & AugMix & Ours & Bound \\
        \hline
        A$\to$D & 60.3 & 46.0 & 48.9 & 42.3 & 40.5 & 36.9 & 12.3\\
        A$\to$W & 59.6 & 65.2 & 46.9 & 40.0 & 32.4 & 28.6 & 10.1\\
        D$\to$A & 64.1 & 66.0 & 62.4 & 50.3 & 53.0 & 46.6 & 33.8\\
        D$\to$W & 83.5 & 59.9 & 69.7 & 45.2 & 48.1 & 35.9 & 4.6\\
        W$\to$A & 64.7 & 67.9 & 60.1 & 60.1 & 59.8 & 55.0 & 36.4\\
        W$\to$D & 120.2 & 64.3 & 70.9 & 46.6 & 54.6 & 44.5 & 0.7\\
        \hline
        Avg ($\downarrow$) & 75.4 & 61.6 & \textbf{59.8} & 47.4 & 48.1 & \textbf{41.3} & 16.3 \\
        \bottomrule
    \end{tabular}
    }
    }
    \vspace{-3mm}
\end{table}

==> CRDA (TOMM)/latex/tabs/mCE_OfficeHome.tex <==
% \begin{table*}
%     \centering
%     \caption{mCE on all settings of Office-Home dataset for stage2-(b).}
%     \label{tab:mCE_OfficeHome}
%     \small{
%     \setlength{\tabcolsep}{1.1mm}{
%     \begin{tabular}{l|cccccccccccc|c}
%         \toprule
%         Method & Ar$\to$Cl & Ar$\to$Pr & Ar$\to$Rw & Cl$\to$Ar & Cl$\to$Pr & Cl$\to$Rw & Pr$\to$Ar & Pr$\to$Cl & Pr$\to$Rw & Rw$\to$Ar & Rw$\to$Cl & Rw$\to$Pr & Avg \\
%         \hline
%         Ori & 68.6 & 60.5 & 57.2 & 64.1 & 57.4 & 56.2 & 64.0 & 69.8 & 52.8 & 61.3 & 69.5 & 58.2 &  \\
%         Ori+AugMix & 71.9 & 65.9 & 61.7 & 74.0 & 68.4 & 66.7 & 75.0 & 78.0 & 64.1 & 68.5 & 73.8 & 64.2 &  \\
%         Ori+AdvTL & 60.1 & 51.5 & 51.1 & 65.0 & 60.1 & 57.2 & 60.5 & 63.3 & 51.9 & 61.7 & 66.2 & 50.0 &  \\
%         \bottomrule
%     \end{tabular}
%     }
%     }
% \end{table*}

\begin{table}
    \centering
    \caption{mCE ($\%$) on all cross-domain settings of Office-Home dataset under CRDA (ResNet-50).}
    \label{tab:mCE_OfficeHome}
    \setlength{\tabcolsep}{1.2mm}{
    \small{
    \begin{tabular}{c|ccc|ccc|c}
        \toprule
        \multirow{2}{*}{Settings} & \multicolumn{3}{c|}{CDAN+TN} &\multicolumn{3}{c|}{DCAN} & Lower \\
        \cline{2-7}
         & - & AugMix & Ours & - & AugMix & Ours & Bound \\
        \hline
        Ar$\to$Cl & 69.7 & 69.3 & 59.8 & 61.4 & 63.2 & 58.3 & 52.2 \\
        Ar$\to$Pr & 62.2 & 52.8 & 52.2 & 51.0 & 49.3 & 48.0 & 37.7 \\
        Ar$\to$Rw & 59.2 & 56.0 & 48.0 & 47.9 & 46.0 & 44.6 & 30.8 \\
        Cl$\to$Ar & 65.4 & 73.7 & 66.0 & 58.6 & 57.4 & 55.2 & 45.8 \\
        Cl$\to$Pr & 58.7 & 56.6 & 51.9 & 58.0 & 57.3 & 51.6 & 34.6 \\
        Cl$\to$Rw & 57.6 & 61.3 & 56.2 & 52.0 & 53.8 & 47.5 & 34.7 \\
        Pr$\to$Ar & 65.5 & 72.2 & 63.6 & 61.1 & 58.9 & 55.1 & 44.7 \\
        Pr$\to$Cl & 70.9 & 71.4 & 63.6 & 66.2 & 65.3 & 62.2 & 54.9 \\
        Pr$\to$Rw & 55.0 & 55.3 & 48.8 & 53.7 & 48.5 & 49.4 & 25.7 \\
        Rw$\to$Ar & 63.2 & 62.4 & 57.8 & 63.0 & 59.2 & 57.7 & 36.0 \\
        Rw$\to$Cl & 70.4 & 61.4 & 64.4 & 64.0 & 64.2 & 59.9 & 52.9 \\
        Rw$\to$Pr & 60.9 & 52.6 & 47.9 & 58.4 & 52.5 & 52.6 & 26.8 \\
        \hline
        Avg ($\downarrow$) & 63.2 & 62.1 & \textbf{56.7} & 57.9 & 56.3 & \textbf{53.5} & 39.7 \\
        \bottomrule
    \end{tabular}
    }
    }
    \vspace{-1.5mm}
\end{table}
 	 	 	 	 	 	 	 		 	 	 	 
 	 	 	 	 	 	 	 	 	 	 	 	


 	  	 	 	 	 	 	 	 	 	 	 	 	 
	 	 	 	 	 	 	 	 	 	 	 


==> CRDA (TOMM)/latex/tabs/stage.tex <==
\begin{table}
    \renewcommand\arraystretch{1.1}
    \centering
    \caption{Different stages based on information available while training. Note that labels of the target domain are unavailable while training.}
    \label{tab:stage}
    \setlength{\tabcolsep}{1.7mm}{
    \small{
    \begin{tabular}{c|c|ccc|c}
        \toprule
        \multicolumn{2}{c}{\multirow{2}*{Stage}} & \multicolumn{3}{|c|}{Training} & Testing\\
        \cline{3-5}
        \multicolumn{2}{c|}{}& Source & Target$^*$ & Corruption & (corrupted)\\
        \hline
        Mostly &1-(a) & \checkmark &   & \checkmark & Source\\
        studied & 1-(b) & \checkmark &   &   & Source\\
        \hline
        \multirow{2}*{\textbf{Ours}}&\textbf{2-(a)} & \checkmark & \checkmark & \checkmark & \textbf{Target}\\
        &\textbf{2-(b)} & \checkmark & \checkmark &  & \textbf{Target}\\
        \cline{1-2}
        Future & 2-(c) & \checkmark &   & \checkmark & Target\\
        work & 2-(d) & \checkmark &   &  & Target\\
        
        \bottomrule
    \end{tabular}
    }
    }
\end{table}

% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline

% \multicolumn{2}{|c|}{ \multirow{2}*{$S_i$} }& \multicolumn{4}{c|}{sj} &\multirow{2}*{max}\\
% \cline{3-6}
% \multicolumn{2}{|c|}{}&50&100&150&200&\\
% \hline
% \multirow{4}*{cl}&50&0&100&200&300&300\\
% \cline{2-7}
% &100&100&0&100&200&200\\
% \cline{2-7}
% &150&200&100&0&100&200\\
% \cline{2-7}
% &200&300&200&100&0&300\\
% \hline
% \end{tabular}
% \end{table}

        % \multirow{2}{*}{Settings} & \multicolumn{3}{c|}{CDAN+TN} & Lower \\
        %  & - & +AugMix & +Ours & Bound \\
        % \hline
        % Ar$\to$Cl & 69.7 & 73.2 & 59.8 & 52.4 \\
        % Ar$\to$Pr & 62.2 & 67.4 & 52.2 & 37.8 \\
        % Ar$\to$Rw & 59.2 & 63.9 & 48.0 & 30.9 \\
        % Cl$\to$Ar & 65.4 & 74.9 & 66.0 & 45.7 \\
        % Cl$\to$Pr & 58.7 & 69.3 & 51.9 & 34.8 \\
        % Cl$\to$Rw & 57.6 & 67.8 & 56.2 & 34.9 \\
        % Pr$\to$Ar & 65.5 & 76.4 & 63.6 & 44.7 \\
        % Pr$\to$Cl & 70.9 & 79.1 & 63.6 & 55.1 \\
        % Pr$\to$Rw & 55.0 & 66.0 & 48.8 & 25.8 \\
        % Rw$\to$Ar & 63.2 & 70.3 & 57.8 & 35.8 \\
        % Rw$\to$Cl & 70.4  & 75.1 & 64.4 & 53.2 \\
        % Rw$\to$Pr & 60.9 & 66.2 & 47.9 & 27.0 \\
        % \hline
        % Avg ($\downarrow$) & 63.2 & 70.8 & 56.7  & 39.8 \\

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle


==> latex/Supplementary_Section/Full_TSCL_results.tex <==
\section{Full results for trade-off in TSCL}
\label{sec:full_TSCL_result}
\input{latex/Supplementary_Section/tabs/err_TSCL}
Table~\ref{tab:err_TSCL_full} reports the full results (mCE) of methods on each type of visual corruption.

==> latex/Supplementary_Section/Worst-Corruption_Sample.tex <==
\section{Instance of worst-corruption sample}
\label{sec:wc_sample}
% \input{latex/Supplementary_Section/imgs/wc_sample}
We show several examples of worse-corruption sample generated by our method, as well as its corresponding clean image, in Figure \ref{fig:wc_sample}.

==> latex/Supplementary_Section/imgs/mCE_office-sup.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.45\textwidth]{latex/figs/mCE-office-supplementary.pdf}
    \caption{mCE ($\%$) on all cross-domain settings of Office-31 under CRDA (ResNet-50).}
    \label{fig:mCE-office-sup}
\end{figure}

==> latex/Supplementary_Section/imgs/mCE_officehome-sup.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.96\textwidth]{latex/figs/mCE-officehome-supplementary.pdf}
    \caption{mCE ($\%$) on all cross-domain settings of Office-Home under CRDA (ResNet-50).}
    \label{fig:mCE-officehome-sup}
\end{figure*}

==> latex/Supplementary_Section/imgs/wc_sample.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=0.88\textwidth]{latex/figs/WC_samplee.pdf}
    \caption{Worst-corruption samples of different iterations.}
    \label{fig:wc_sample}
\end{figure*}

==> latex/Supplementary_Section/tabs/err_TSCL.tex <==
\begin{table}
    \centering
    \caption{Error rate ($\%$) under a specific known corruption on the Ar$\to$Rw setting of Office-Home dataset for teacher-student warm-up shceme.}
    \label{tab:err_TSCL_full}
    \setlength{\tabcolsep}{3mm}{
    % \small{
    \begin{tabular}{c|ccc}
        \toprule
        \multirow{2}{*}{Corruption} & \multicolumn{3}{c}{CDAN+TN} \\
        \cline{2-4}
         & -  & DataAug & Ours \\
        \hline
        Clean & 22.1 & 24.6 & 21.2\\
        Gaussian Noise & 78.4 & 33.4 & 27.8\\
        Shot Noise & 78.3 & 34.9 & 26.9\\
        Impulse Noise & 83.4 & 33.4 & 24.4\\
        Defocus Blur & 70.4 & 34.9 & 26.7\\
        Motion Blur & 69.5 & 28.4 & 24.3\\
        Zoom Blur & 53.6 & 29.4 & 23.1\\
        Fog & 47.3 & 24.6 & 23.6\\
        Frost & 55.7 & 30.6 & 25.5\\
        Snow & 60.0 & 31.2 & 23.9\\
        Elastic Transform & 84.2 & 30.0 & 23.3\\
        Contrast & 66.4 & 24.6 & 23.0\\
        Brightness & 29.7 & 26.5 & 23.6\\
        JPEG Compression & 37.6 & 29.0 & 23.2\\
        Pixelate & 45.7 & 26.9 & 22.6\\
        Glass Blur & 86.4 & 37.0 & 27.8\\
        \bottomrule
    \end{tabular}
    % }
    }
    \vspace{-1.5mm}
\end{table}

==> latex/algorithm/algorithm-AdvTL.tex <==
\begin{algorithm}[t]
\caption{Overall process for AdvTL}
\begin{algorithmic}[1]
\Require The original DA model $f+c$, source and target domain samples $X=X_s\cup X_t$, source domain labels $Y_s$. Parameters for AdvTL: threshold $\delta$, update stride $\eta > 2\delta$ and update steps $n$.
\State Train the original DA model as the teacher model $f^{(tea)}+c^{(tea)}$. Fix the parameters.
\State 	Construct a student network $f^{(stu)}+c^{(stu)}$ with same structure of $f+c$. 
\Repeat :
\State Get a batch of source and target domain samples $x=\{x_{s},x_{t}\}$ from $X$ and the corresponding labels of source domain samples $y_s$.
\State Construct worst-transformation-case samples $x_{t}^{(adv)}$ by Algorithm \ref{algorithm-PGD}:

$x_{t}^{(adv)}=\text{PGD}(x_{t},x_{s},f^{(stu)},\delta, \eta, n)$
\State  Calculate features representations of target domain samples:

$z_{t}^{(adv)}=f^{(stu)}\left(x_{t}^{(adv)}\right)$


$z_{t}^{(stu)}=f^{(stu)}\left(x_{t}\right)$

$z_{t}^{(tea)}=f^{(tea)}\left(x_{t}\right)$

\State  Calculate features representations of source domain samples:

$z_{s}^{(stu)}=f^{(stu)}\left(x_{s}\right)$

$z_{s}^{(tea)}=f^{(tea)}\left(x_{s}\right)$

\State Calculate classification predict result:

$z_{stu}=z_{t}^{(stu)} \cup z_{s}^{(stu)}$

$y_{stu}=c_{stu}\left(z_{stu}\right)$
\State 	Calculate the loss introduced by the original DA model:

$\ell_{ori}\left(z_{stu},\ y_{stu},\ y_s\right)$
\State Calculate the contrastive loss by \textcolor{red}{Equation (\ref{CL-AdvTL})}: 

$\ell_{contrast}^{(adv)}=\ell_{contrast}\left(z_{t}^{(adv)},z_{t}^{(tea)}\right)$
\State Calculate the total loss $\ell_{total}=\ell_{ori}+\lambda\ell_{contrast}^{(adv)}$
\State Backward grad and update parameters of $f_{stu}+c_{stu}$
\Until Converge
\State \Return $f_{stu}+c_{stu}$

\end{algorithmic}
\label{algorithm-AdvTL}
\end{algorithm}

==> latex/algorithm/algorithm-AdvTL_v2.tex <==
\begin{algorithm}[t]
    \caption{Overall process for TSCL-WC}
    \label{algorithm-AdvTL}
    \small{
    \textbf{Input:} 
    \begin{minipage}[t]{0.87\linewidth}
    Data and source labels: $\mathcal{X}_{s}$, $\mathcal{X}_{t}$, $\mathcal{Y}_{s}$; Original DA model $f+c$; Parameters: $\delta=60/255$, $\eta > 2\delta$, $n=2$
    \end{minipage}
    
    \textbf{Output:} 
    \begin{minipage}[t]{0.86\linewidth}
    Robust student model $f^{(stu)}+c^{(stu)}$
    \end{minipage}
    
    \begin{algorithmic}[1]
    \State Train the original model as a teacher model $f^{(tea)}+c^{(tea)}$. Fix the parameters.
    \State 	Construct a student network $f^{(stu)}+c^{(stu)}$ with same structure of $f+c$. 
    \Repeat :
    \State Draw $x_{s}, x_{t}, y_s$ from $\mathcal{X}_{s}, \mathcal{X}_{t}, \mathcal{Y}_{s}$.
    \State 
    \begin{minipage}[t]{0.9\linewidth}
    Construct worst-corruption samples according to Equation (\ref{construction_x_adv}) and Algorithm \ref{algorithm-PGD}:
    
    $\qquad x_{t}^{(wc)}=\text{PGD}\left(x_{t},x_{s},f^{(stu)},\delta, \eta, n\right)$
    \end{minipage}
    
    \State
    Update $f^{(stu)}+c^{(stu)}$ according to Equation (\ref{CL-AdvTL})
    
    and (\ref{total_loss}).
    
    \Until Convergence
    \State \Return $f^{(stu)}+c^{(stu)}$
    
    \end{algorithmic}
    }
\end{algorithm}

==> latex/algorithm/algorithm-TSCL.tex <==
\begin{algorithm}[t]
\caption{Overall process for TSCL}
\begin{algorithmic}[1]
\Require The original DA model $f+c$, source and target domain samples $X=X_s\cup X_t$, source domain labels $Y_s$ and a transformation $T \equiv {\{t_{i}\}}_{0}^{5}$ with six levels of severity during testing ($t_{0}$ denotes clean data).
\State Train the original DA model as the teacher model $f^{(tea)}+c^{(tea)}$. Fix the parameters.
\State 	Construct a student network $f^{(stu)}+c^{(stu)}$ with same structure of $f+c$. 
\Repeat :
\State Get a batch of samples $x$ from $X$ and the corresponding labels of source samples $y_s$.
\State Randomly select a transformation $t$ from $\{t_{0},t_{5}\}$
\State  Calculate features representations:

$z^{(stu)}=f^{(stu)}\left(t(x)\right)$, $z^{(tea)}=f^{(tea)}\left(x\right)$
\State Calculate classification predict result:

$y^{(stu)}=c^{(stu)}\left(z^{(stu)}\right)$
\State 	Calculate the loss introduced by the original DA model:

$\ell_{ori}\left(z^{(stu)},\ y^{(stu)},\ y_s\right)$
\State Calculate the contrastive loss in Equation (\ref{CL}):

$\ell_{contrast}\left(z^{(stu)},z^{(tea)}\right)$
\State Calculate the total loss: $\ell_{total}=\ell_{ori}+\lambda\ell_{contrast}$
\State Backward gradients and update parameters of $f^{(stu)}+c^{(stu)}$
\Until Converge
\State \Return $f^{(stu)}+c^{(stu)}$

\end{algorithmic}
\label{algorithm-TSCL}
\end{algorithm}

==> latex/algorithm/algorithm-TSCL_v2.tex <==
\begin{algorithm}[t]
\caption{Overall process for TSCL}
\textbf{Input:} 
\begin{minipage}[t]{0.87\linewidth}
Data and source labels: $\mathcal{X}_{s}$, $\mathcal{X}_{t}$, $\mathcal{Y}_{s}$; Original DA model $f+c$; A corruption with six levels of severity  $T = {\{t_{i}\}}_{0}^{5}$  ($\mathrm t_{0}$ denotes clean data).
\end{minipage}

\textbf{Output:} 
\begin{minipage}[t]{0.86\linewidth}
Robust student model $f^{(stu)}+c^{(stu)}$
\end{minipage}
\begin{algorithmic}[1]
\State Train the original model as a teacher model $f^{(tea)}+c^{(tea)}$. Fix the parameters.
\State 	Construct a student network $f^{(stu)}+c^{(stu)}$ with same structure of $f+c$. 
\Repeat :
\State Draw $x_{s}, x_{t}, y_s$ from $\mathcal{X}_{s}, \mathcal{X}_{t}, \mathcal{Y}_{s}$. $x=\{x_{s}, x_{t}\}$.
\State Randomly draw a corruption $t$ from $\{t_{0},t_{5}\}$
\State  
\begin{minipage}[t]{0.9\linewidth}
\begin{spacing}{1.4}
Update $f^{(stu)}+c^{(stu)}$ according to (\ref{CL}):

    $\qquad \ell_{ori}\left(t(x_{s}),t(x_{t}),y_{s}\right)$

    $\qquad \ell_{con}\left(f^{(stu)}(t(x)),f^{(tea)}(x)\right)$
\end{spacing}
\begin{spacing}{0.5}
    $\qquad \ell_{total}=\ell_{ori}+\lambda\ell_{con}$
\end{spacing}
\end{minipage}
% \begin{minipage}[t]{0.9\linewidth}
% \begin{spacing}{1.4}
% Update $f^{(stu)}+c^{(stu)}$ according to (\ref{CL}):

%     $\qquad \ell_{ori}\left(x_{s},x_{t},y_{s}\right)$

%     $\qquad \ell_{con}\left(f^{(stu)}(x_{t}^{(wc)}),f^{(tea)}(x_{t})\right)$
% \end{spacing}
% \begin{spacing}{0.5}
%     $\qquad \ell_{total}=\ell_{ori}+\lambda\ell_{con}$
% \end{spacing}
% \end{minipage}
\Until Convergence
\State \Return $f^{(stu)}+c^{(stu)}$

\end{algorithmic}
\label{algorithm-TSCL}
\end{algorithm}

==> latex/imgs/Fig1.tex <==
\begin{figure*}
    \begin{center}
    \includegraphics[width=0.96\textwidth]{latex/figs/figure_stage2be.pdf}
    \end{center}
    \caption{Instances of corruption robust domain adaptation (CRDA).
    %Here labeled clean source domain (art) and unlabeled clean target domain (real world) samples are available while training.
    Existing domain adaptation method (CDAN+TN \cite{wang2019TransNorm}) and corruption robust method (AugMix \cite{hendrycks2019augmix}), even their combination, suffer from unseen corruptions on target domain.}
    \label{fig:illustration}
    \vspace{-3mm}
\end{figure*}

==> latex/sections/Abstract_v6.tex <==
\begin{abstract}
% 1. DA 目前的发展（套话）
% 2. 更真实且通用的场景——Corruption Robust Domain Adaptation (CRDA): 定义
% 3. 目前方法直接组合在CRDA上效果不好
% 4. 我们的思考：CRDA问题可以分解为两个子问题：
%     (1) domain invariance 和 Corruption 之间的协调 <-- 以往方法组合不好的原因
%     (2) 如何考虑unseen corruption的问题 
% 5. 由此，我们提出了 xxxxx 的方法：
%     (1) 针对问题(1), 我们先不考虑unseen corruption的问题，假设可以得到测试corruption，基于已有DA模型框架，提出TSCL --> 一个基础框架
%     (2) 针对问题(2), 我们采用基于inverting domain discrepency的方式构造worst-corruption sample 来隐式地表示unseen corruption; 并且将TSCL中的随机数据增广替换成worst-corruption sample。
% 6. 实验上看，我们的方法优于现有解决方案
% 7. 有趣的一点是：我们理论证明了只需要考虑最严重的severity就可以handle所有level severity，提升了方法效果和效率。
Big progress has been achieved in domain adaptation in decades. Given unseen corruptions (\eg, noise and blur) in real data, domain adaptation methods are increasingly required to be corruption robust on target domain.
In this paper, we investigate a new task, corruption robust domain adaptation (CRDA): 
% models are required 
to be accurate on clean data and robust against unseen corruptions on target domain.
We observe that popular methods of domain adaptation, corruption robustness, and their combinations, have sub-optimal CRDA results.
% The challenges are two-fold: 1) trade-off between domain invariance and corruption robustness; 2) data augmentation for robustness contributes little to domain adaptation.
The challenges are two-fold: 1) trade-off between domain invariance and corruption robustness; 2) generalization to unseen corruptions via domain information.
% For better results, we present TSCL-WP.
For better results, we present TSCL-WC.
Specifically, we propose a simple but effective teacher-student scheme (TSCL) to balance domain invariance and corruption robustness. %suitable to most DA models on the basis of random data augmentation.
% Besides, we generate worse perturbation (WP) by inverting domain discrepancy to mimic unseen corruptions.
Besides, we generate worst-corruption (WC) samples that most enlarge domain discrepancy to mimic unseen corruptions.
Experiments verify that TSCL-WC keeps performance on clean data and achieves better corruption robustness than baselines.
% Interestingly, \textcolor{red}{we empirically find that networks always learn order-invariant representations for different severity levels of corruptions.} Based on this finding, we theoretically show only considering the most severe corruptions is enough for our framework to gain robustness on all levels of severity.
\end{abstract}

==> latex/sections/Conclusion_Future_Work_v2.tex <==
\section{Conclusion}
% In this paper, we propose TSCL-WC to investigate a more realistic new task, corruption robustness domain adaptation (CRDA) in the aspect of two key challenges: 1) trade-off between domain invariance and corruption robustness; 2) generalization to unseen domains via domain information. For the first challenge, we propose a Teacher-Student scheme via Contrastive Loss (TSCL) to show that it is better to consider domain invariance and corruption robustness step by step instead of simultaneous training. For the second challenge, taking the particularity of DA into consideration, we present a new idea for corruption robustness that mimic unseen corruptions via worst-corruption samples most enlarging domain discrepancy. Empirical results justify that TSCL-WC outperforms existing baselines on domain invariance and achieves better corruption robustness.
% 
% Future work include a more general scenario, where target domains are unavailable while training. This is in the category of domain generalization. 
In this paper, we propose TSCL-WC to investigate a more realistic new task, corruption robust domain adaptation (CRDA). We propose a Teacher-Student scheme via Contrastive Loss (TSCL) to show that it is better to consider domain invariance and corruption robustness step by step rather than simultaneous learning. Besides, taking domain information into consideration, we present a new idea for corruption robustness that mimic unseen corruptions via worst-corruption samples most enlarging domain discrepancy. Empirical results justify that TSCL-WC outperforms existing baselines on domain invariance and achieves better corruption robustness.

==> latex/sections/Experiments_v3.tex <==
\section{Experiments}
%------------------------------------------------------------------------------------
\subsection{Setups}
\paragraph{Datasets.} Office-Home and Office-31 are two benchmark datasets widely adopted for visual domain adaptation algorithms. Experiments are mainly conducted on Office-Home, a relatively challenging dataset. 
% Office is an easier dataset to validate generalization of our methods. 
\textit{Office-Home}~\cite{venkateswara2017officehome} is a challenging medium sized benchmark, which contains 15588 images from 4 domains (Artistic images (Ar), Clip Art (Cl), Product images (Pr), and Real-World images (Rw)). Each domain consists of 65 object classes under daily life environment.
\textit{Office-31}~\cite{saenko2010office31} is a standard benchmark with 4110 images and 31 classes under office environment. There are totally three domains: Amazon (A), Webcam (W) and DSLR (D).

\paragraph{Corruption.} To check the corruption robust of one given DA model, we create the corrupted version of Office-31 and Office-Home by using the corruption types defined by ImageNet-C \cite{hendrycks2019benchmarking}, a widely used benchmark for corruption robustness. For each image, there exists $15$ corruption types with $5$ levels of severity as partially illustrated in Figure\ref{fig:illustration} and detailed described in SM. 
% We further test on these two datasets with spatial transformation and the implementation details can be seen in corresponding experiments.

%------------------------------------------------------------------------------------
\paragraph{Baselines} To illustrate the improvement on CRDA, we apply our method on \textbf{CDAN+TN} \cite{long2018conditional,wang2019TransNorm}, a classic baseline model for domain adaptation. We further apply our method to a SOTA DA model \textbf{DCAN} \cite{Li20DCAN}. 
% In addition, our methods can further maintain or improve models' original accuracy. To validate this, another SOTA model \textbf{SHOT} \cite{liang2020shot} is adopted together with CDAN+TN and DCAN.
Note that the domain discrepancies of CDAN+TN and DCAN are respectively measured by adversarial methods~\cite{goodfellow2014GAN} and MMD~\cite{borgwardt2006integrating}. 
We compare our TSCL-WC method with \textbf{AugMix} \cite{hendrycks2019augmix}, a SOTA method for corruption robustness, which aggregates several general transformations such as contrast, equalization and posterization for data augmentation. 
 
 %-----------------------------------------------------------------------------------
 \paragraph{Implementation details}
 For contrastive loss in Equations (\ref{CL}) and (\ref{CL-AdvTL}), the trade-off $\lambda$ is set to $0.5$. For TSCL-WC, we conduct Algorithm \ref{algorithm-DDG} with $\delta=60/255$, $\eta=6$, $n=2$. Network structures and other hyper-parameters are the same as the original DA models. The structure and parameter details of CDAN+TN and DCAN can be seen in SM. 
 
 %-----------------------------------------------------------------------------------
\subsection{Experiments of Trade-off in TSCL}
\input{latex/tabs/acc_rawOfficeHome}
% In this section, we evaluate our TSCL framework method for stage 2-(a). Table \ref{tab:err_TSCL_home} precisely reports the error rate on clean data and some corruptions with the most severe severity. The full results can be seen in SM. Results show that our TSCL can significantly improve the model’s robustness against a specific corruption. Furthermore, TSCL can further improves the model’s original performance instead of negative effect brought by pure data augmentation. In another word, TSCL does not conduct trade-off over robustness and accuracy. 
Assuming testing corruptions available while training, we precisely report the error rate of TSCL on clean data and some corruptions with the most severe severity in Table \ref{tab:err_TSCL_home}. The full results can be seen in SM. Results show that our TSCL can significantly improve the model’s robustness against a specific known corruption. Furthermore, instead of the negative effect brought by simultaneous learning of pure data augmentation, TSCL further improves the model’s average clean accuracy that reflects domain invariance. In another word, the step-by-step learning scheme of TSCL balances the trade-off between domain invariance and corruption robustness well. 

\input{latex/tabs/err_TSCL_OfficeHome_full}

\input{latex/imgs/Error_MostLevel_stage2b_A2R}

%-----------------------------------------------------------------------------------
\subsection{Experiments in CRDA}
We compare TSCL-WC with AugMix and the original DA models on both corruption robustness and original performance which reflects domain invariance. In addition, we further set an empirical lower bound for CRDA calculated by mCE of TSCL applied on CDAN+TN, which assumes testing corruptions are available while training. Models that reach the lower bound can be robust against unseen corruptions as if they are already known beforehand.
 
Figure \ref{fig:exp3} shows the error rate on clean data and 15 different corruptions with the most severe severity in a single setting. It is reported that TSCL-WC achieves improvement over most kinds of corruptions with about 10 percentages in average than the original model and 3 percentages than AugMix.  We observe that AugMix only achieves relatively high robustness on several corruptions such as Fog and Contrast. The reason possibly is that these corruptions can be implied by the aggregation of the general transformations defined by AugMix, however, corruptions like Pixelate may lie out of the implied set. Instead, our TSCL-WC achieves a much more generalizable implied set thanks to reasonable utilization of domain discrepancy information. It is worthy of noting that same like TSCL, TSCL-WC can also improve the original accuracy which reflects domain invariance.

\input{latex/tabs/mCE_OfficeHome}
\input{latex/tabs/mCE_Office}
 
Figure \ref{fig:exp3} also shows that TSCL-WC gains no improvement over the Contrast corruption. We argue the reason probably is that this corruption conducts too much shift in sample space which goes beyond the scope of Assumption~\ref{assum:assum1}. Possible solutions include loosening the constraint in Assumption~\ref{assum:assum1} and considering the invariant order of pixel values (Contrast does not change the order of pixel values). We leave them for future work.

We report the overall robustness under the whole Office-Home and Office-31 datasets in Table \ref{tab:mCE_OfficeHome} and Table \ref{tab:mCE_Office} with the standard robustness metric mCE. Results show that even the SOTA model AugMix has sub-optimal results or even worse  performance in some settings, which indicates the challenge of CRDA. Despite the challenging task, TSCL-WC still gains improvement with obvious margins. Meanwhile, there is still a long way for further study to reach the lower bound in CRDA.
Besides robustness, TSCL-WC also maintains or improves the original accuracy of DA models. Results are shown in Table \ref{tab:acc_OfficeHome}. 

%-----------------------------------------------------------------------------------
% \subsection{Improvement on original accuracy}

% In \textcolor{red}{Experiments xxx}, both TSCL and TSCL-Adv are found beneficial to the original performance. In this section, we respectively apply our methods on \textcolor{red}{classic} model CDAN+TN and two SOTA model DCAN and SHOT. \textcolor{red}{For TSCL, it is found that replacing the random data augmentation with random translation gains stable improvement over all kinds of methods. Random translation randomly translate the input images with at most 1/4 of the image width, which is realized by affine transformation \cite{jaderberg2015STN,shen2016TICNN}. Details about Random Translation and affine transformation can be seen in Appendix. }. \textcolor{red}{Table \ref{tab:acc_OfficeHome}} shows that our methods achieve improvement over all three kinds of DA models. Results shows that SHOT with TSCL-translation can overperform the current SOTA. In summary, TSCL and TSCL-Adv gains improve over both robustness and accuracy \textcolor{red}{instead of trade-off}, which is what most current methods on transformation robustness lack.

% \textcolor{red}{\textbf{Analysis for improvement of TSCL with translation}}

% % \begin{figure*}
% % \begin{center}
% % % \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
% % %   %\includegraphics[width=0.8\linewidth]{egfigure.eps}
% % \includegraphics[width=0.9\textwidth]{latex/figs/exp5.png}
% % \end{center}
% %   \caption{accuracy on clean Office-Home data}
% % \label{fig:exp5}
% % \end{figure*}
% \input{latex/tabs/acc_rawOfficeHome}

%-----------------------------------------------------------------------------------
\subsection{Empirical analysis}
\label{sec:empirical}

\paragraph{Ablation.}
\input{latex/tabs/mCE_Ablation-delta}

In Section~\ref{sec:theory}, we theoretically show only considering the edge points on the $\delta$ cycle is enough for TSCL-WC, which is realized by setting stride $\eta > 2\delta$ in Algorithm \ref{algorithm-DDG}. Table \ref{tab:Ablation-delta} reports the mCE under CRDA with different strides $\eta$. Results show that the setting $\eta > 2\delta$, which results in only considering the edge points, gains best performance. We conclude the reason why settings $\eta \ll \delta$ perform relatively poorer is that they may wander in the $\delta$ cycle instead of reaching the large-shift points on the edge, which causes a lack of consideration on large-shift corruptions like contrast and blurs. Table \ref{tab:Ablation-delta} also shows that only 2 update steps is enough for TSCL-WC to gain corruption robustness.
More ablation results can be seen in SM.
\input{latex/imgs/ObservationsOfOrder}

\paragraph{Order-invariant representations of corruptions.}
We empirically observe that the distance between the corrupted versions and the corresponding clean image in feature space (\textbf{feature distance} for precise) is always positively correlated to the severity of corruptions. Training details are shown in SM. Figure \ref{fig:order} shows that even only trained on clean and corrupted samples with a single severity, models still learn the positive correlation instead of relatively nearer feature distance on a specific severity. In a word, networks always learn order-invariant representations in feature space for different levels of severity, which contributes to Assumption~\ref{assum:assum2} in Section~\ref{sec:wc}.


==> latex/sections/Introduction_v4.tex <==
\section{Introduction}
% In the study of visual generalization, researchers mainly focus on robustness on domain shift and common corruptions. Domain shift is mainly studied by domain adaptation (DA) \cite{pan2009survey,long2018conditional,wang2019transferable,Li20DCAN,liang2020shot} and domain generalization (DG) \cite{volpi2018generalizing,dg_mmld,huang2020self} based on the scenario where labeled source domain samples (and unlabeled target domain samples for DA) are available while training to perform classification on target domain. Contributions to corruption robustness focus on the performance of the corrupted testing data (\eg, noise and blur) \cite{hendrycks2019benchmarking,hendrycks2019augmix,sun19ttt,hendrycks2019using}. However, researchers of DA or DG mainly consider domain shift on clean data, while current corruption robustness works focus on corruptions without domain shift. In a word, these two studies with a common goal for generalization \textcolor{red}{deliberately} ignored each other. Thus, there is a question to which both of them must face up: 
% 
% \textit{How to achieve both domain invariance and corruption robustness in a more generalized way?}
% 
\input{latex/imgs/illustration}
Domain adaptation (DA)~\cite{pan2009survey} is a promising technique to transfer knowledge from well-labeled source domain to assist unlabeled target domain learning  with domain shift. Tremendous efforts on domain adaptation~\cite{Li20DCAN,liang2020shot,wang2019TransNorm,long2018conditional} and domain generalization (DG)~\cite{huang2020self,dg_mmld,volpi2018generalizing} indicate the significant progress on domain shift. Besides domain shift, given unseen corruptions (\eg, noise and blur) in real data, domain adaptation methods are increasingly required to be corruption robust on target domain (see Figure~\ref{fig:illustration}). However, most DA or DG works only consider domain shift on clean data, while corruption robustness works~\cite{hendrycks2019benchmarking,hendrycks2019using,hendrycks2019augmix,sun19ttt} usually focus on corruptions without domain shift. Thus, there is a question worth considering: 
\textit{How to build domain invariance with corruption robustness in a more generalized way?}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \input{latex/tabs/differentDAsettings}

%Taking into consideration this question, we investigate a more realistic new task,
According to this question, we propose a new task: \textbf{Corruption Robust Domain Adaptation (CRDA)}, \ie, DA models are required to achieve high performance not only on clean target domain that reflects domain invariance, but also be robust against \textbf{unseen} corruptions that are unavailable for training.
%Popular methods of domain adaptation and corruption robustness, even their combinations, 
Popular DA methods, even combining with corruption robustness modules, will get sub-optimal results (Figure~\ref{fig:illustration}) because they cannot handle well two challenges of CRDA: 
%(1) Trade-off between domain invariance and corruption robustness. These two properties may conflict to each other due to \textcolor{red}{different optimization directions.}
(1) trade-off between domain invariance and corruption robustness, which may conflict to each other due to different optimization directions;
(2) generalization to unseen corruptions via domain information. 
% reasonable utilization of domain information helps improving generalization to unseen corruptions. 
It is still rarely investigated that how to take reasonable utilization of domain information for generalization to unseen corruptions.
Meanwhile, data augmentation may have no sense because it only encourages networks to memorize the specific corruptions seen during training and leaves models unable to generalize to new corruptions~\cite{geirhos2018generalisation,hendrycks2019augmix,vasiljevic2016examining}.
To our knowledge, our work is among the first attempt to unify robustness on domain shift and common corruptions.

To address the above challenges, we propose a novel mechanism towards corruption robust domain adaptation.
%Considering the above two key problems, our attempts are as following:
For the first challenge, instead of gaining domain invariance and corruption robustness simultaneously, we propose a Teacher-Student scheme via Contrastive Loss (TSCL) to obtain these two properties step by step. Specifically, a teacher model is first pre-trained to learn domain-invariant representations and then a student model further distills from the teacher model to learn robustness against a specific known corruption via contrastive loss drawn from contrastive learning~\cite{chen2020simple}.
%For the second challenge, based on several assumptions (detailedly discussed in Section~\ref{sec:wc}), \textbf{worst-corruption samples} which most enlarge domain discrepancy are generated to represent unseen corruptions.
% More specifically, instead of minimizing, we construct worst-corruption samples based on the idea of inverting domain discrepancy, which inversely adds the gradients of domain discrepancy loss to the clean inputs by Project Gradient Descent (PGD)~\cite{madry2017PGD}.
For the second challenge, based on several assumptions (see Section~\ref{sec:wc}), we mimic unseen corruptions via worst-corruption (WC) sample generation.
Specifically, instead of minimizing the domain discrepancy, we construct worst-corruption samples by inversely adding the gradients of domain discrepancy loss to the clean inputs by Project Gradient Descent (PGD)~\cite{madry2017PGD}.
Thus, by replacing samples augmented by a specific known corruption in TSCL with WC samples, the proposed \textit{TSCL-WC} method effectively handles the two challenges and achieve better CRDA results.
%Thus, by replacing samples augmented by a specific known corruption in TSCL with Worst-Corruption (WC) samples, we present \textbf{TSCL-WC} for CRDA, which can handle both challenges introduced above.

Our work makes the following contributions:
\begin{itemize}
    \item We investigate a new scenario called corruption robust domain adaptation (CRDA) to equip domain adaptation models with corruption robustness.
    
    \item We propose a novel method for corruption robustness that mimic unseen corruptions via information of domain discrepancy.
    
    \item Experiments demonstrate that our method not only significantly improves corruption robustness for DA models but also maintains or improves classification results on clean target domain.
\end{itemize}

==> latex/sections/Methodology_v4.tex <==
% 1. TSCL
%     分析挑战(1) --> 以往方法不好的原因之一是同时训练时会冲突 --> 在这样的情况下很难handle trade-off。
%     抛弃同时训练，我们一步一步来 --> TSCL

% 2. worst-corruption samples via inverting domain discrepancy
%     TSCL的问题：只能用data augmentation 处理已知的corruption。 + 通常Data Augmentation不适用于unseen corruption. 
%     --> 利用DA特有的domain信息来构造可以模拟unseen corruption的样本。
    
%     --> Adv

% 3. TSCL-WC
%     总体描述 + 只要handle最严重的corruption就可以了

% 4. Theoretical Explanation

% 5. Metrics
\section{Methodology}
% In this paper, our attempts are made through two key problems of CRDA: 1) trade-off between domain invariance and corruption robustness; 2) generalization to unseen corruptions via domain information. we first propose a simple but effective teacher-student scheme (TSCL) for the first problem. As for the second problem, we further construct worst-corruption samples to mimic unseen corruptions via inversely enlarging domain discrepancy. Putting them together, we derive \textbf{TSCL-WC} as illustrated in Figure \ref{fig:AdvTL}. In addition, we theoretically show that only considering the most severe level of corruptions is  enough for our frameworks to handle all levels of severity.

%----------------------------------------------------------------------------------------------------------
\subsection{Teacher-Student Scheme via Contrastive Loss}
Due to different optimization directions, it is hard to handle domain invariance and corruption robustness at the same time, which results in sub-optimal performance of direct combinations of current works on domain adaptation and corruption robustness. Thus, instead of simultaneous training, we propose a Teacher-Student scheme via Contrastive Loss (TSCL) inspired by contrastive learning~\cite{chen2020simple} to learn these two properties step by step. 

We first assume testing corruptions are available while training so that models only need to learn robustness against a specific known corruption. Algorithm~\ref{algorithm-TSCL} shows the overall process of TSCL. We first gain domain-invariant representations by a pre-trained teacher model based on the traditional DA setting. During the training of the student model, together with random data augmentation, features of the augmented data are aligned with corresponding clean features of the teacher model by contrastive loss introduced below.

\input{latex/algorithm/algorithm-TSCL_v2}

Given a batch of samples ${\{x_i\}}_1^N$, we use feature extractor $f^{(tea)}$ and $f^{(stu)}$ introduced in Algorithm \ref{algorithm-TSCL} to get $2N$ representation feature vectors:
\begin{equation}
    \begin{split}
        Z^{(tea)}={\left\{z_{i}^{(tea)}|z_{i}^{(tea)}=f^{(tea)}(x_i)\right\}}_1^N,\\
        Z^{(stu)}={\left\{z_{i}^{(stu)}|z_{i}^{(stu)}=f^{(stu)}(x_i)\right\}}_1^N,
    \end{split}
\end{equation}
% $Z^{(tea)}={\{z_{i}^{(tea)}|z_{i}^{(tea)}=f^{(tea)}(x_i)\}}_1^N$ and $Z^{(stu)}={\{z_{i}^{(stu)}|z_{i}^{(stu)}=f^{stu}(x_i)\}}_1^N$. 
where we define $Z=Z^{(tea)}\cup Z^{(stu)}={\{z_i\}}_1^{2N}$. The similarity loss of each two features can be calculated by:
%
\begin{equation}
    \ell_{sim}\left(z_{i}, z_{j}\right)=-\log \frac{\exp \left(sim\left(z_{i}, z_{j}\right) / \tau\right)}{\sum_{z_{k} \in Z, z_{k} \neq z_{i}} \exp \left(sim\left(z_{i}, z_{k}\right) / \tau\right)},
    \label{similarity}
\end{equation}
%
where $\tau=0.2$ is a temperature controller to control the similarity extent, and $sim\left(z_i,z_j\right)={z_i}^T z_j/z_i z_j$ is cosine distance between two vectors. 
% which is $sim\left(z_i,z_j\right)={z_i}^T z_j/z_i z_j$. 
Note that Equation (\ref{similarity}) is asymmetric between $z_i, z_j$. The final contrastive loss is defined by:
%
\begin{equation}
    \begin{split}
    \ell_{con}\left(Z^{(stu)}, Z^{(tea)}\right)
    = \frac{1}{2 N} \sum_{i=1}^{N} \left[\ell_{sim}\left(z_{i}^{(stu)}, z_{i}^{(tea)}\right)+ \ell_{sim}\left(z_{i}^{(tea)}, z_{i}^{(stu)}\right)\right],
    \end{split}
    \label{CL}
\end{equation}
%
where the goal is to minimize the distance between feature representations $z_{i}^{(stu)}$ and $z_{i}^{(tea)}$ of a same sample $x_i$. The other kinds of losses defined by the original DA models $\ell_{ori}$ also need to be calculated.

% The overall process of TSCL is shown in \textcolor{red}{Algorithm \ref{algorithm-TSCL}}. 
It is worthy of noting that only the most severe level of corruption $T$ ($t_{5}$ in Algorithm \ref{algorithm-TSCL}) is considered to achieve robustness on all severity levels. The theoretical explanation is described in Section~\ref{sec:theory}. In fact, contrastive loss does not make $Z^{(stu)}$ definitely same as $Z^{(tea)}$. And thanks to corruptions, the final feature representation $Z^{(stu)}$ has a further distillation on the basis of the teacher model, which may lead to not only improvement on robustness but also better performance on domain invariance.

%------------------------------------------------------------------------------------------
\subsection{Worst-Corruption Sample}
\label{sec:wc}

In TSCL, there exists a strong assumption that testing corruptions are available during training. Besides, data augmentation in TSCL only encourages networks to memorize the specific corruptions seen during training and leaves models unable to generalize to new corruptions~\cite{geirhos2018generalisation,vasiljevic2016examining}. 
Thus, we further propose worst-corruption samples most enlarging domain discrepancy to mimic unseen corruptions.

We first assume that corrupted target domain samples hold larger domain discrepancy to source domain than corresponding clean ones, which is empirically proved in SM. 
In domain adaptation, the domain discrepancy is always measured by transfer loss, which is commonly realized by Maximum Mean Discrepancy (MMD) \cite{borgwardt2006integrating,Li20DCAN,long2015DAN,pan2010TCA} or adversarial methods \cite{ganin2016DANN,long2018conditional}. 
Thus, our core idea is to find the points near the original images in sample space that most increase the transfer loss (\textbf{worst-corruption samples} for precise) to represent the most severe corruptions. 

The followings are three basic assumptions for our method, where distance $d_{*}(t(x),x)$ denotes distance between the corrupted images and corresponding clean images:
\begin{assumption}
\label{assum:assum1}
The corrupted versions are within the $\delta$-range neighborhood of the original clean image in sample space ($\boldsymbol{\delta}$ \textbf{cycle} for precise) and distance in sample space $d_{s}(t(x),x)$ becomes larger with increase of the severity level of corruption $T$.
\end{assumption}
\begin{assumption}
\label{assum:assum2}
Within the $\delta$ cycle, the severity level $t$ of a corruption  $T$ is positively correlated to distance in feature space  $d_{f}(f(t(x)) ,f(x))$.
\end{assumption}
\begin{assumption}
\label{assum:assum3}
Within the $\delta$ cycle, the severity level $t$ of a corruption $T$ is positively correlated to the value of transfer loss $\ell_{trans}(t(x))$.
\end{assumption}

The empirical proof can be seen in SM. Assumption~\ref{assum:assum2}  is drawn from an interesting finding in Section~\ref{sec:empirical} that networks always learn order-invariant representations for different severity levels of corruptions.

Based on the above assumptions, we can construct the worst-corruption sample. Given an input target domain data $x_{t}$, source domain $D_{s}$, transfer loss $\ell_{trans}$ and a corruption set $T$ ($t \in T$) whose corresponding corrupted data $t(x_{t})$ is within the $\delta$ cycle of $x_{t}$, we get
\begin{equation}
    \begin{split}
    x_{t}^{(wc)}&=\mathop{\arg\max}_{\left\|x_{t}^{(wc)}-x_{t}\right\| \leq \delta} \ell_{trans}\left(f(x_{t}^{(wc)}), f(D_{s})\right)
    \\&\Rightarrow \mathop{\arg\max}_{t \in T} \ell_{trans}\left(f(t\left(x_{t})\right), f(D_{s})\right)=t_{\max }(x_{t}),
    \end{split}
    \label{construction_x_adv}
\end{equation}
which means the point $x_{t}^{(wc)}$ near the original target domain sample in sample space that most increases transfer loss (\textbf{worst-corruption sample} for precise) can represent the most severe corruption. The idea behind $x_{t}^{(wc)}$ is: instead of minimizing, we mimic unseen corruptions via inversely enlarging domain discrepancy. The proof of Equation (\ref{construction_x_adv}) can be seen in SM.
In practice, worst-corruption samples are constructed by Project Gradient Descent (PGD)~\cite{madry2017PGD} in Algorithm \ref{algorithm-PGD}.
\input{latex/algorithm/algorithm-PGD}
\input{latex/imgs/StructureOfAdvTLe}

\textcolor{red}{It is worthy noting that the worst-corruption samples looks similar to adversarial samples~\cite{madry2017PGD}. However, there exists few evidence that adversarial training contributes a lot to corruption robustness in previous study. We first show that it significantly improves corruption robustness on the basis of the bridge between corruption and domain discrepancy constructed by Assumption \ref{assum:assum3}. Meanwhile, worst-corruption samples are constructed in a unsupervised way while common adversarial training always needs groundtruth labels.}

%----------------------------------------------------------------------------------
\subsection{TSCL-WC}
\label{sec:tscl-wc}

Replacing the random corrupted samples $t(x)$ in Algorithm \ref{algorithm-TSCL} of TSCL with Worst-Corruption samples $x_{t}^{(wc)}$, we derive the final framework \textbf{TSCL-WC} shown in Figure \ref{fig:AdvTL}.

By minimizing distance between worst-corruption samples $x_{t}^{(wc)}$ and original clean samples $x_{t}$ in feature space iteratively, features of the most severely corrupted images come closer to original clean ones, as:
\begin{equation}
    \min d_{f}\left(f(x_{t}^{(wc)}), f(x_{t})\right) \Rightarrow \min d_{f}\left(f(t_{max}(x_{t})), f(x_{t})\right),
    \label{illustration1}
\end{equation}
which leads to better performance on robustness against unseen corruptions. In practice, we realized Equation (\ref{illustration1}) by contrastive loss defined in Equation (\ref{CL}):
\begin{equation}
    \ell_{con}^{(wc)}\left(x_{t}^{(wc)},x_{t}\right)=\ell_{con}\left(f^{(stu)}(x_{t}^{(wc)}),f^{(tea)}(x_{t})\right)
    \label{CL-AdvTL},
\end{equation}
where $f^{(stu)}$ denotes a student model with the same structure as the original DA model to learn corruption robustness and $f^{(tea)}$ is a fixed teacher model trained by the setting of the original DA model. Together with the loss defined by the original DA model $\ell_{ori}$, which commonly contains classifier loss on source domain and transfer loss as illustrated in Figure \ref{fig:AdvTL}, the final total loss is:
\begin{equation}
    \ell_{total}=\ell_{ori}(x_{s},x_{t},y_{s})+\lambda \ell_{con}^{(wc)}(x_{t}^{(wc)},x_{t}).
    \label{total_loss}
\end{equation}

Note that the worst-corruption samples are only constructed on target domain and only processed by contrastive loss. As shown in Algorithm \ref{algorithm-AdvTL}, the overall procedure of TSCL-WC is an extended version of TSCL, which replaces the random corrupted samples $t(x)$ in Algorithm \ref{algorithm-TSCL} with worst-corruption samples $x_{t}^{(wc)}$ to generalize to unseen corruptions.

\input{latex/algorithm/algorithm-AdvTL_v2}

%-----------------------------------------------------------------------------------------
\subsection{Theoretical explanation}
\label{sec:theory}
\textcolor{red}{Intuively, worst-corruption samples should loop many times like $n=10$ in PGD, which is time-consuming. In this section, we theoretically show that we only need to consider the edge point so that by setting $n=2$ is enough, which effectively reduces the time consumption. We begin with the following two propositions, respectively for TSCL and TSCL-WC:} 

\begin{theorem}
Only aligning the most severe level of a corruption is enough to gain robustness under TSCL.
\label{pro1}
\end{theorem}
\begin{theorem}
Only aligning the edge points in the $\delta$ cycle $\{x_{t}^{(wc)}|\|x_{t}^{(wc)}-x_{t}\|=\delta\}$ is enough to gain corruption robustness under TSCL-WC framework.
\label{pro2}
\end{theorem}

Intuitively, aligning all points in the $\delta$ cycle $\{x_{t}^{(wc)}|\|x_{t}^{(wc)}-x_{t}\| \leq \delta\}$ in Equation (\ref{construction_x_adv}) by setting $\eta \ll \delta$ in Algorithm \ref{algorithm-PGD} seems like a reasonable setting, however, we theoretically and empirically show that only aligning the edge points $\{x_{t}^{(wc)}|\|x_{t}^{(wc)}-x_{t}\|=\delta\}$ is enough for TSCL-WC based on Assumption~\ref{assum:assum2}. We first prove Proposition \ref{pro1} for TSCL, then further extend to Proposition \ref{pro2} for TSCL-WC. The theoretical explanations are as followed. 
 
\subsubsection{Proposition 1 for TSCL}
Given input data $x$, a feature extractor $f$ and a corruption $T$ with continuous severity, we denote the distance in feature space $d_{f}(f(T(x)),f(x))$ as $d(T)$. Then Assumption~\ref{assum:assum2}  can be explained as  $T$ is positively correlated with $d(T)$. Due to the properties of monotonic function, the upper bound of $d(T)$ is $d(T_{max})$:
 \begin{equation}
    0 \leq d(T) \leq d(T_{max}) = d_{max},
    \label{max-dT}
\end{equation}
where $T_{max}$ denotes the most severe level of corruption $T$.
By limiting $d_{max}$ to $0$, we get:
\begin{equation}
    \lim_{d_{max} \rightarrow 0} {d(T)}= \lim_{d_{max} \rightarrow 0} {d_{f}(f(T(x)),f(x))}=0,
\label{limit}
\end{equation}
which means for all severity levels of corruption $T$, features of corrupted data $T(x)$ and clean data $x$ are the same when $d_{max} \rightarrow 0$. Thus robustness against a specific corruption is achieved.

Now the last issue is how to limit $d_{max}$ to 0. Note that:
\begin{equation}
    d_{max}=d(T_{max})=d_{f}(f(T_{max}(x)),f(x)).
    \label{dmax}
\end{equation}
Thus, by aligning features of the most severely corrupted samples $T_{max}(x)$ with original features $x$, we get $d_{max}\rightarrow0$. Proposition \ref{pro1} for TSCL is derived.

\subsubsection{Proposition 2 for TSCL-WC}
Considering Assumption~\ref{assum:assum1}, the shift in sample space increases as the increase of the severity level of a corruption $T$. Thus, the most severe corruption $T_{max}(x)$ is always achieved on the edge points of $\delta$ cycle. Then we can use $\{x_{t}^{(wc)}|\|x_{t}^{(wc)}-x_{t}\|=\delta\}$ to implicitly represent $T_{max}(x)$ due to the conclusion in Equation (\ref{construction_x_adv}).  By aligning features of these edge points with the original features via minimizing the contrastive loss defined in Equation (\ref{CL-AdvTL}), corruption robustness is achieved under TSCL-WC as :
\begin{equation}
    \lim_{\ell_{con}^{(wc)} \rightarrow 0} {d(T)}= \lim_{\ell_{con}^{(wc)} \rightarrow 0} {d_{f}(f(T(x)),f(x))}=0.
    \label{limit_xadv}
\end{equation}
Proposition \ref{pro2} for TSCL-WC is derived.

In practice, setting $\eta>2\delta$ in Algorithm \ref{algorithm-PGD} and \ref{algorithm-AdvTL} with only step $n=2$ gains enough good performance.
% In practice, results shows that 
% \textcolor{red}{Based on Assumption 2, we conclude the result that } 
% In practice, we \textcolor{red}{are surprised to} find that only aligning the edge points $\{x_{t}^{(wc)}|\|x_{t}^{(wc)}-x_{t}\|=\delta\}$ in TSCL-WC gets best performance, which is realized by setting $\eta > 2\delta$ in \textcolor{red}{Algorithm}. Intuitively, the setting with $\eta \ll \delta$ seems like a more reasonable setting but gets poorer performance on large shift transformations like contrast. 

%-----------------------------------------------------------------------------------------
\subsection{Metrics for corruption robustness}
The commonly used standardized aggregate performance measure is the Corruption Error (CE) \cite{hendrycks2019benchmarking}, which can be computed by:
\begin{equation}
    \mathrm{CE}_{T}^{f}=\left(\sum_{t=1}^{5} E_{t, T}^{f}\right) \bigg/\left(\sum_{t=1}^{5} E_{t, T}^{ AlexNet}\right),
    \label{CE}
\end{equation}
where $E_{t, T}^{f}$ denotes the error rate of model $f$  on target domain data transformed by corruption $T$ with severity $t$. The $AlexNet$ is trained on clean source domain and tested on corrupted target domain.

The corruption robustness of model $f$ is summarized by averaging Corruption Error values of 15 corruptions introduced in Section~\ref{sec:definition_robustness}: 
$\mathrm{CE}_{\text{Gaussian Noise}}^{f}, \dots , \mathrm{CE}_{\text{Glass Blur}}^{f}$. The results in the mean CE or mCE~\cite{hendrycks2019benchmarking} for short. mCE is calculated by only one setting (\eg, the Ar:Rw setting in Office-Home). For average performance of corruption robustness on the whole dataset (\eg, Office-Home), we need to average mCE values of all settings. 







==> latex/sections/Outline.tex <==
Abstract
    1. DA 目前的发展（套话）
    
    2. 更真实且通用的场景——Corruption Robust Domain Adaptation (CRDA): 定义
    
    3. 目前方法直接组合在CRDA上效果不好
    
    4. 我们的思考：CRDA问题可以分解为两个子问题：
        (1) Domain-invariance 和 Corruption 之间的协调 <-- 以往方法组合不好的原因
        
        (2) 如何考虑unseen corruption的问题 
        
    5. 由此，我们提出了 xxxxx 的方法：
        (1) 针对问题(1), 我们先不考虑unseen corruption的问题，假设可以得到测试corruption，基于已有DA模型框架，提出TSCL --> 一个基础框架
        
        (2) 针对问题(2), 我们采用基于inverting domain discrepency的方式构造worst-corruption sample 来隐式地表示unseen corruption; 并且将TSCL中的随机数据增广替换成worst-corruption sample。
        
    6. 实验上看，我们的方法优于现有解决方案
    
    7. 有趣的一点是：我们理论证明了只需要考虑最严重的severity就可以handle所有level severity，提升了方法效果和效率。
    
Introduction
    DA现状，Robustness现状-->这两个方向seperately 考虑问题，那么就引出思考：
         How to achieve both domain invariance and corruptionrobustness in a more generalized way?
         
    提出Corruption Robust Domain Adaptation (CRDA)，进一步描述。 用Figure1说明目前方法不行-->原因是他们或多或少fail in two-fold chanllenges in CRDA:
        1) Domain-invariance 和 Corruption 之间的协调
            
        2) General robustness to unseen corruptions via domain information.
    在对CRDA的考虑上，我们分解成了两个子问题：
        ( <-- 以往方法组合不好的原因
        
        ( 
        
    基于这两个问题，我们提出了 xxxxx 的方法:
        首先单独考虑问题(1)，那么我们可以假设corruption是可知的，提出TSCL，指出先考虑Domain-Invariance，再考虑Corruption Robustness，而不是同时一起考虑。
        
        再考虑问题(2), 我们采用inverting domain discrepency的方式构造worst-corruption sample 来隐式地表示unseen corruption
        
        结合两个问题的解决方法，我们将TSCL中对样本基于已知corruption做增广替换成造worst-corruption sample，完成了我们的方法
        
    除此之外，我们还理论上说明了只考虑最严重的severity就足够了
    
    简单描述实验结论，总结。
        
Methodology
    简述：我们对CRDA的考虑：
    (1) Domain-invariance 和 Corruption 之间的协调 --> TSCL
    (2) 如何考虑unseen corruption的问题 --> Augmentation via inverting domain discripancy
        
    1. TSCL
    
    2. Augmentation via inverting domain discripancy
    
    3. Overall Framework
    
    4. Theoretical Explanation

Experiments
    1. 验证TSCL框架的有效性
        与直接同时考虑 Data Augmentation 和 DA的想法对比，说明分阶段考虑更优
        
    2. 我们的方法再CRDA这个setting下的效果
        Office-Home、Office
        
    3. Ablation
        (没办法把TSCL和Augmentation via inverting domain discripancy拆开，因为这两个合起来才能再CRDA下进行，分开setting都不适用)
        保持现有的不变
        
    4. Order-invariant representations of corruptions
        说只考虑最严重的severity就足够这件事情的实验依据


遗留问题：
    我们的方法 (原来的TSCL-Adv) 起个什么名字好？

==> latex/sections/Outline_v2.tex <==
Abstract
1. (目前DA在理想情况下做的已经不错了，可以研究更实际的情况了）
2. 一个实际的系统要求同时Domain-invariant and Corruption Robustness
3. 我们提出了一个更实际的task，CRDA：进一步描述
4. 以往方法在这个task下不好，原因是下面两个挑战
5. 两个挑战：(1) DI和CR之间的trade-off 或balance；(2) 利用DA的特性来进一步优化对unseen corruption的鲁棒性
6. 我们的方法
7. 实验结果

Introduction
1. 目前研究现状, 引出问题：我们需要同时考虑DI和CR了
2. 提出一个新的task CRDA：描述
3. 以往方法不好-->两个挑战: ：(1) DI和CR之间的trade-off 或balance；(2) 利用DA的特性来进一步优化对unseen corruption的鲁棒性
4. 基于两个挑战，分别提出我们的方法：
    挑战(1) --> TSCL
    挑战(2) --> construct worst-corruption samples via inverting domain discrepancy
5. 总结
    
Methodology
1. TSCL
    分析挑战(1) --> 以往方法不好的原因之一是同时训练时会冲突 --> 在这样的情况下很难handle trade-off。
    抛弃同时训练，我们一步一步来 --> TSCL

2. worst-corruption samples via inverting domain discrepancy
    TSCL的问题：只能用data augmentation 处理已知的corruption。 + 通常Data Augmentation不适用于unseen corruption. 
    --> 利用DA特有的domain信息来构造可以模拟unseen corruption的样本。
    
    --> Adv

3. TSCL-inverse
    总体描述 + 只要handle最严重的corruption就可以了

4. Theoretical Explanation

5. Metrics
    
Experiments

% 实验上需要也展示 clean target domain 上的分类性能.

==> latex/sections/Supplementary_Outline.tex <==
Supplementary Material 内容
1.	15 种corruptions 的图示和描述 y
2.	3个Assumption的可靠性说明 y
3.	公式（6）的推导 y
4.	完整的TSCL结果 y
5.	AugMix的Implement Detail  x
6.	Lower bound 的具体求法，实现细节 x
8.	5.4节Order-invariant representations of corruptions的训练细节 y
9.	Training Loss的曲线 x
10.	Ablation：
    a)	超参数的影响 y
11.	解释性实验
    a)	展示并分析worst-corruption sample的图像 y
    b)	之前方法简单结合没处理好trade-off的量化指标证明
12.	为什么要选AugMix作为baseline对比 x
13. 之前基于特征的AdvTL-feature的尝试：结果及原因分析 x
14. 对于一些没有直接定义Transfer Loss 的DA x 模型，一种替代方法：训练一个鉴别器来生成Transfer Loss
    a)  出发点
    b)  方法描述
    b)  结果展示
15. AlexNet 的error rate结果 (计算mCE时用的) x
16. 其他DA模型的鲁棒性测试，说明DCAN鲁棒性相对好只是个例 x
17. 说明表3中的CLean的结果是所有鲁棒性的实验取的平均值 y


==> latex/sections/Todo_list.tex <==
Theoretical Explanation 是否严谨？是否必要？待商榷。
想想有没有更好的名字代替TSCL-Inverse
在实验中加原始精度比较
Introduction 部分是否要去掉combination，再考虑一下
想办法把Abstract里的Teacher-Student scheme (TSCL) 补全成 Teacher-Student scheme via Contrastive Loss (TSCL)。但是补全就会跨列
是否要把图1放在第一页？放在第二页会和表格冲突

==> latex/tabs/Rebuttle_TTT.tex <==
\begin{table}[h]
    \centering
    \caption{Accuracy ($\%$) of TTT under Ar$\to$Cl}
    \label{tab:acc_TTT}
    \setlength{\tabcolsep}{1.2mm}{
    \small{
    \begin{tabular}{c|c|c}
        \toprule
        \multirow{2}{*}{TTT} & \multicolumn{2}{c}{CDAN+TN}\\
        \cline{2-3}
         & - & TSCL-WC\\
        \hline
        33.4 & 54.1 & 57.1\\
        \bottomrule
    \end{tabular}
    }
    }
    \vspace{-1.5mm}
\end{table}

==> latex/tabs/Rebuttle_clean2corrupted.tex <==
\begin{table}[h]
\linespread{1}
    \centering
    \vspace{-3mm}
    \caption{Accuracy ($\%$) on different corruption level of gaussian noise under Ar$\to$Cl.}
    \vspace{-3mm}
    \label{tab:clean2corrupted}
    \small{
    \setlength{\tabcolsep}{1.0mm}{
    \begin{tabular}{l|cccccc|c}
        
        \toprule
        Method & clean & 1 & 2 & 3 & 4 & 5 & Avg ($\uparrow$)\\
        \hline
        CDAN+TN & 54.1 & 49.2 & 45.9 & 41.3 & 34.4 & 25.9 & 41.8\\ 
        Yours & 53.6  & 51.3  & 50.5  & 49.9 & 48.0 & 44.5 & 49.6\\
        TSCL-WC & 57.1 & 55.5 & 54.5 & 52.0 & 48.4 & 39.8 & 51.2\\
        \bottomrule
    \end{tabular}
    }
    }
    \vspace{-4mm}
\end{table}



==> latex/tabs/acc_rawOffice.tex <==
\begin{table}
    \centering
    \caption{Accuracy ($\%$) on clean Office-31 data (ResNet-50).}
    \label{tab:acc_Office}
    \setlength{\tabcolsep}{1.15mm}{
    \small{
    \begin{tabular}{c|ccc|ccc}
        \toprule
        \multirow{2}{*}{Settings} & \multicolumn{3}{c|}{CDAN+TN} &\multicolumn{3}{c}{DCAN} \\
        \cline{2-7}
         & - & AugMix & Ours & - & AugMix & Ours\\
        \hline
        A$\to$D & 92.2 & 85.9 & 92.2 & 93.4 & 92.8 & 90.8\\
        A$\to$W & 93.2 & 75.6 & 93.3 & 94.3 & 94.3 & 95.0\\
        D$\to$A & 74.7 & 64.6 & 73.9 & 76.6 & 74.3 & 76.2\\
        D$\to$W & 98.5 & 98.9 & 98.6 & 97.0 & 97.6 & 96.7\\
        W$\to$A & 74.6 & 62.0 & 75.2 & 72.4 & 71.9 & 72.9\\
        W$\to$D & 100.0 & 100.0 & 100.0 & 99.6 & 99.8 & 100.0\\
        \hline
        Avg ($\downarrow$) & 88.9 & 81.2 & 88.9 & 88.9 & 88.5 & 88.6\\
        \bottomrule
    \end{tabular}
    }
    }
    \vspace{-3mm}
\end{table}

==> latex/tabs/err_TSCL_OfficeHome.tex <==
\begin{table}
    \centering
    \caption{Error rate ($\%$) under a specific known corruption on the Ar$\to$Rw setting of Office-Home dataset for teacher-student warm-up shceme.}
    \label{tab:err_TSCL_home}
    \setlength{\tabcolsep}{1.6mm}{
    \small{
    \begin{tabular}{c|ccc}
        \toprule
        \multirow{2}{*}{Corruption} & \multicolumn{3}{c}{CDAN+TN} \\
        \cline{2-4}
         & -  & DataAug & Ours \\
        \hline
        Clean & 22.1 & 24.6 & 21.2\\
        Gaussian Noise & 78.4 & 33.4 & 27.8\\
        Defocus Blur & 70.4 & 35.0 & 26.7\\
        Fog & 47.3 & 24.6 & 23.6\\
        Contrast & 66.4 & 24.6 & 23.0\\
        \bottomrule
    \end{tabular}
    }
    }
    \vspace{-1.5mm}
\end{table}

==> latex/tabs/frequent_notations.tex <==
\begin{table}[t]
    \centering
    \caption{Notations and descriptions used in this paper}
    \label{tab:frequent_notation}
    \small{
    \setlength{\tabcolsep}{1.1mm}{
    \begin{tabular}{c|c}
        \toprule
        Notation&Description\\
        \hline
        $f$ & feature extractor \\
        % ($\Leftrightarrowf_{1}\circf_{2}$)
        % $f_{1}$ & feature extractor without the last layer\\
        % $f_{2}$ & the last layer of feature extractor\\
        $c$ & classifier\\
        $TL$ & transfer loss\\
        $x$ & input data\\
        % $f$ & interval feature ($\Leftrightarrowf_{1}(x)$)\\
        $z$ & final feature ($\Leftrightarrow f(x)$)\\
        $*^{(stu)}$ & * of the student model (\textcolor{red}{e.g.} $f^{(stu)}$)\\
        $*^{(tea)}$ & * of the teacher model\\
        $x_{t}^{(adv)}$ & worst-transformation-case sample\\
        \bottomrule
    \end{tabular}
    }
    }
\end{table}

==> latex/tabs/stage.tex <==
\begin{table}
    \renewcommand\arraystretch{1.1}
    \centering
    \caption{Different stages based on information available while training. Note that labels of the target domain are unavailable while training.}
    \label{tab:stage}
    \setlength{\tabcolsep}{1.7mm}{
    \small{
    \begin{tabular}{c|c|ccc|c}
        \toprule
        \multicolumn{2}{c}{\multirow{2}*{Stage}} & \multicolumn{3}{|c|}{Training} & Testing\\
        \cline{3-5}
        \multicolumn{2}{c|}{}& Source & Target$^*$ & Corruption & (corrupted)\\
        \hline
        Mostly &1-(a) & \checkmark &   & \checkmark & Source\\
        studied & 1-(b) & \checkmark &   &   & Source\\
        \hline
        \multirow{2}*{\textbf{Ours}}&\textbf{2-(a)} & \checkmark & \checkmark & \checkmark & \textbf{Target}\\
        &\textbf{2-(b)} & \checkmark & \checkmark &  & \textbf{Target}\\
        \cline{1-2}
        Future & 2-(c) & \checkmark &   & \checkmark & Target\\
        work & 2-(d) & \checkmark &   &  & Target\\
        
        \bottomrule
    \end{tabular}
    }
    }
\end{table}

% \begin{table}[!htbp]
% \centering
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline

% \multicolumn{2}{|c|}{ \multirow{2}*{$S_i$} }& \multicolumn{4}{c|}{sj} &\multirow{2}*{max}\\
% \cline{3-6}
% \multicolumn{2}{|c|}{}&50&100&150&200&\\
% \hline
% \multirow{4}*{cl}&50&0&100&200&300&300\\
% \cline{2-7}
% &100&100&0&100&200&200\\
% \cline{2-7}
% &150&200&100&0&100&200\\
% \cline{2-7}
% &200&300&200&100&0&300\\
% \hline
% \end{tabular}
% \end{table}

        % \multirow{2}{*}{Settings} & \multicolumn{3}{c|}{CDAN+TN} & Lower \\
        %  & - & +AugMix & +Ours & Bound \\
        % \hline
        % Ar$\to$Cl & 69.7 & 73.2 & 59.8 & 52.4 \\
        % Ar$\to$Pr & 62.2 & 67.4 & 52.2 & 37.8 \\
        % Ar$\to$Rw & 59.2 & 63.9 & 48.0 & 30.9 \\
        % Cl$\to$Ar & 65.4 & 74.9 & 66.0 & 45.7 \\
        % Cl$\to$Pr & 58.7 & 69.3 & 51.9 & 34.8 \\
        % Cl$\to$Rw & 57.6 & 67.8 & 56.2 & 34.9 \\
        % Pr$\to$Ar & 65.5 & 76.4 & 63.6 & 44.7 \\
        % Pr$\to$Cl & 70.9 & 79.1 & 63.6 & 55.1 \\
        % Pr$\to$Rw & 55.0 & 66.0 & 48.8 & 25.8 \\
        % Rw$\to$Ar & 63.2 & 70.3 & 57.8 & 35.8 \\
        % Rw$\to$Cl & 70.4  & 75.1 & 64.4 & 53.2 \\
        % Rw$\to$Pr & 60.9 & 66.2 & 47.9 & 27.0 \\
        % \hline
        % Avg ($\downarrow$) & 63.2 & 70.8 & 56.7  & 39.8 \\
